DFL-TORO: A One-Shot Demonstration Framework for Learning Time-Optimal Robotic Manufacturing Tasks

This paper presents DFL-TORO, a novel Demonstration Framework for Learning Time-Optimal Robotic tasks via One-shot kinesthetic demonstration. It aims at optimizing the process of Learning from Demonstration (LfD), applied in the manufacturing sector. As the effectiveness of LfD is challenged by the quality and efficiency of human demonstrations, our approach offers a streamlined method to intuitively capture task requirements from human teachers, by reducing the need for multiple demonstrations. Furthermore, we propose an optimization-based smoothing algorithm that ensures time-optimal and jerk-regulated demonstration trajectories, while also adhering to the robot's kinematic constraints. The result is a significant reduction in noise, thereby boosting the robot's operation efficiency. Evaluations using a Franka Emika Research 3 (FR3) robot for a variety of tasks further substantiate the efficacy of our framework, highlighting its potential to transform kinesthetic demonstrations in contemporary manufacturing environments. Moreover, we take our proposed framework into a real manufacturing setting operated by an ABB YuMi robot and showcase its positive impact on LfD outcomes by performing a case study via Dynamic Movement Primitives (DMPs).

==> Sections/drafts/fsm.tex <==
In order to overcome this challenge, we propose a programming framework based on Finite-State Machines (FSM), which allows for modular composition of various behaviors/actions. The FSM architecture enables the integration of subtasks learned via Learning from Demonstration (LfD), traditionally programmed modules, and any other arbitrary behavior modules in a cohesive manner.

### Finite-State Machine Architecture

The FSM framework operates by defining a set of states, each representing a specific behavior or action of the robot. Transitions between these states are governed by predefined conditions or triggers, ensuring that the robot can switch from one behavior to another seamlessly based on the context and requirements of the task at hand.

1. **State Definition**:
   - Each state in the FSM corresponds to a distinct subtask or behavior. These states can be learned via LfD, where the robot observes and replicates human demonstrations, or they can be traditionally programmed modules that execute specific functions.
   - For example, a state could represent picking an object (LfD-based), moving to a specific location (traditionally programmed), or interacting with a PLC (arbitrary behavior module).

2. **Transitions and Conditions**:
   - Transitions between states are defined by conditions that must be met for the robot to move from one state to another. These conditions can be based on sensory inputs, completion signals from other modules, or time-based triggers.
   - For instance, a transition from the "pick object" state to the "move to location" state might be triggered by a sensor detecting that the object has been successfully grasped.

3. **Modularity and Scalability**:
   - The modular nature of FSM allows for easy integration of new behaviors or modifications of existing ones without disrupting the overall system. This is particularly advantageous during the transition from mass production to mass customization, as new subtasks can be incorporated incrementally.
   - As new LfD modules are developed, they can be added as new states in the FSM, while maintaining the existing traditionally programmed functionalities.

4. **Interfacing with External Systems**:
   - The FSM framework can interface with external systems such as PLCs, digital I/O devices, and other components of the robotic setup. This is essential for ensuring that traditionally programmed functionalities, such as gripper control or system communications, continue to operate smoothly alongside LfD modules.
   - By defining specific states and transitions for these interactions, the FSM ensures that these critical operations are maintained and seamlessly integrated with new behaviors.

### Practical Implementation

In practice, implementing an FSM architecture involves several steps:

1. **Design the FSM Structure**:
   - Identify and define all the necessary states and transitions based on the task requirements and existing robotic setup.
   - Ensure that each state is well-documented, with clear descriptions of the conditions for entering and exiting the state.

2. **Develop Behavior Modules**:
   - Create LfD-based modules for tasks that benefit from learning from demonstrations.
   - Implement traditionally programmed modules for tasks that require precise control or interaction with external systems.

3. **Integrate and Test**:
   - Integrate the behavior modules into the FSM framework, ensuring that transitions are correctly defined and tested.
   - Conduct thorough testing to verify that the system operates as expected and that transitions between states are smooth and reliable.

4. **Continuous Improvement**:
   - As new subtasks or improvements are identified, update the FSM structure and behavior modules accordingly.
   - Leverage the modularity of the FSM to add, remove, or modify states without significant disruptions to the overall system.

By adopting a Finite-State Machine architecture, we can achieve a flexible and robust framework that supports the coexistence of LfD-based modules and traditionally programmed functionalities. This approach facilitates a smooth transition towards more adaptive and customized robotic operations, ultimately enhancing the efficiency and capability of robotic systems in diverse industrial applications.

==> Sections/drafts/lfd.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Efficiency of Implementation
- According to [], among the demonstration mechanisms, kinesthetic teaching requires the least setup resources to teach robotic tasks, and is a suitable choice for demonstrating to robotic manipulators.
- to minimize the implementation time and effort from humans, we focus on one-shot demonstration
- There is a choice between allowing humans to demonstrate complete tasks at once, compared to demonstrating one subtask at a time and then allowing the teacher to compose the complete task hierarchy via a high-level approach (that does not require robotic expertise)
- The subtask approach allows for a higher efficiency of implementation for a multitude of reasons:
- By breaking the complex operations into smaller modular components, the LfD algorithm can focus on learning each subtask individually, which simplifies the learning process.
- Subtask demonstration reduces the cognitive load on the human teacher as well, making the demonstration process less difficult
- By focusing on one subtask at a time, the errors and inefficiencies can be more easily identified and corrected, leading to higher overall accuracy and reliability.
- subtasks can be reused and recombined for different tasks, increasing the flexibility and scalability of the system. This modular learning strategy accelerates the training process, reduces the need for extensive retraining, and enhances the robot's ability to adapt to new tasks quickly and efficiently.
- Besides the mentioned advantages, demonstrating on subtask level facilitates the integration of already-existing robotic setups throughout the transformation from mass production to mass customization.
- During this transformation, ensuring seamless integration of robotics with existing systems and processes can be complex.
- This is plus the fact that not every traditional functionality can be replaced by LfD-based modules. For example, gripper functionalities or managing Digitial Inputs/outputs to communicate with PLCs or other components are exclusively programmed in the traditional way and via the robot's exclusive platform.
- In order to ensure a seamless integration of LfD components gradually and without complete change of the already-existing setup, it is necessary to come up with an architecture which enables the co-existance of traditionally programmed modules as well as newly-implemented LfD modules.
- This not only reduces the downtime of this transformation, but is a practical way to do gradual transformation with a higher efficiency of implementation
- The last important factor is the composition of this modular architecture into a task hierarchy in a way that non-robotic-experts can seamlessly implement and modify, via high-level intuitive modular programming.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Demonstrating subtasks instead of complete tasks enhances the efficiency of Learning from Demonstration (LfD) implementation by breaking down complex operations into manageable, modular components. This approach allows robots to learn and master each subtask individually, which simplifies the learning process and reduces the cognitive load on the human demonstrator. By focusing on one subtask at a time, errors and inefficiencies can be more easily identified and corrected, leading to higher overall accuracy and reliability. Additionally, subtasks can be reused and recombined for different tasks, increasing the flexibility and scalability of the system. This modular learning strategy accelerates the training process, reduces the need for extensive retraining, and enhances the robot's ability to adapt to new tasks quickly and efficiently.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% Efficiency of Operation
- A direct measure of efficiency of the operation of LfD is the evaluation of task success rate and production throughput
- an ideal situation is a 100 percent success rate and the maximum possible throughput, which leads to the maximum number of products at the end of the day.
- regarding these metrics, there are several key challenges facing when applying LfD in practical settings.
- When capturing demonstrations, there is noise entangled in the recorded data. This noise can be from the error of the joint sensors as well as the hand trembling and shaking while demonstration.
- The negative effect of this noise impacts the efficiency of operation in two manners:
- Accuracy: Accuracy in LfD is determined by a set of task-specific criteria that ensures the success of the task.
- This is similar to optimization-based approaches, where constraints and costs are designed to guide an algorithm toward a successful solution.
- In human demonstrations, these constraints and costs are inherently encoded.
- For instance, in a reaching task, the end-effector must approach the object from a specific direction to avoid collision with surrounding elements, such as a tray, and grasp the object at the correct angle. This precise information is implicitly conveyed through human demonstration.
- However, the presence of noise can obscure these implicit cues, rendering them less effective. This noise can degrade the performance of LfD algorithms, making it more challenging for the system to learn and generalize the intended motion. 
- It is highly probable that the Learning algorithm overfits on the noise and consequently affect the success rate of the task.
- State of the art learning approaches focus on robustifying against noisy demonstrations, while if we can remove the noise beforehand, we can design our learning algorithm to better the learn the noise-free demonstration, rather than dealing with the noise.
- Exisiting approaches rely on multiple demonstrations to filter out the noise from the authentic accurate demonstration, but it comes at the cost of degrading the efficiency of implementation.

- Execution Time: The robotic task execution time is an important factor which directly influences the production throughput.
- For example, assume the current execution time for producing a product is 150s. For a 24-hour plant, it leads to 576 products per day, while reducing the execution time by only 6s will increase the daily production to 600 products per day, a 4 percent increase in the production throughput.
- Human demonstrations are naturally slow. This is mainly due to the cognitive complexity of teaching accurate detailed motions.
- Nonetheless, as minimizing the execution time is a crucial factor, it is essential to obtain the most optimal timing law from the slow demonstration.
- Speeding up slow demonstrations is not straightforward, as it creates two issues:
- As elaborated in [ref], demonstrations cannot usually sped up uniformly, hence a simple uniform scaling of the demonstration is not a feasible solution. It is necessary to allow the humans to also teach the correct timing law
- The presence of noise causes erratic/jerky motion and often creates velocity/acceleration spikes that renders the whole trajectory kinematically infeasible.
- Motion Jerk refers to the rate of change of acceleration over time and indicates the smoothness of the motion and the wear and tear of the robot. Low jerk profiles indicate smooth human-like motion, reducing stress on the mechanical components, while high jerk can lead to increased wear and tear of the robot, raising maintenance costs and energy consumption.
- Therefore, overall, there is a need to eliminate the noise from demonstration, while maintaining the accuracy of demonstration, as well as achieving the most optimal timing law which completes the task with success in the shortest amount of time







%%%%% LfD in Manufacturing
% Now that we have shown that LfD is the choice for mass customization, of course there are challenges to use LfD in manufacturing and maintain the efficiency

% LfD challenges in manufacturing
% While there has been a major focus on enhancing the performance of the learning algorithms, several practical challenges other than the learning method's performance remain to be able to integrate LfD in manufacturing
% Here, we explain in detail, the challenges of LfD in manufacturing with respect to two aspects: the challenges related to the efficiency of implementation, and the challenges related to the efficiency of operation.
- Efficiency of Implementation: When it comes to the implementation of an LfD-based solution, the motivation is to minimize the implementation resources required to teach a robotic task via a non-expert human. The efficiency of implementation is directly related to the setup required for teaching, the difficulty and effort of demonstration, and the time required for successfully and fully demonstrating the task. According to [], among the demonstration mechanisms, kinesthetic teaching requires the least setup resources to teach robotic tasks, and is a suitable choice for demonstrating to robotic manipulators. Moreover, while many LfD approaches rely on capturing multiple demonstrations, we aim for a one-shot demonstration approach in order to minimize the implementation time and effort.

- While capturing a one-shot demonstration via kinesthetic teaching, there is noise entangled in the recorded demonstration data. This noise can be from the error of the joint sensors as well as the hand trembling and shaking while demonstration. The negative effect of this noise directly impacts the efficiency of operation of LfD shows itself in two main aspects:

%% Accuracy
% Measure of accuracy is a set of subjective requirements that ensures the success of the task.
% Similar to optimization-based approaches where constraints and costs are designed so that the algorithm finds the successful solution.
% Such constraints and costs are implicitly encoded in the human demonstration. For example, in a reaching task, in order to  reach for an object, the end-effector has to approach the object from a certain direction, to avoid collision with the tray and successfully grasp the object with correct angle.
% Such information are implicitly encoded in the human demonstration. However, the presence of noise obscures such implicit information and makes it suboptimal for the LfD algorithm to learn and generalize the motion, hence affecting the success rate.

%%%%%%%%
Accuracy in kinesthetic demonstrations is determined by a set of task-specific criteria that ensure the success of the task. This is similar to optimization-based approaches, where constraints and costs are designed to guide an algorithm toward a successful solution. In human demonstrations, these constraints and costs are inherently encoded.

For instance, in a reaching task, the end-effector must approach the object from a specific direction to avoid collision with surrounding elements, such as a tray, and grasp the object at the correct angle. This precise information is implicitly conveyed through human demonstration.

However, the presence of noise can obscure these implicit cues, rendering them less effective. This noise can degrade the performance of LfD algorithms, making it more challenging for the system to learn and generalize the intended motion. Consequently, the success rate of the task is negatively impacted.
%%%%%%%%

%% Cycle time
The execution time refers to the duration it takes for a robotic task to execute. This duration directly contributes to the production throughput, and hence the efficiency of operation.
Human demonstrations are naturally slow. This is mainly due to the cognitive complexity of teaching accurate detailed motions.
Nonetheless, as minimizing the execution time is a crucial factor, it is essential to obtain the most optimal timing law from the slow demonstration. The state-of-the-art approaches mainly address this by letting humans speed up their initial demonstrations throughout the LfD process, overlooking the robot's kinematic limits. 
This amplifies the effect of the present noise and leads to jerky trajectories.
Motion Jerk refers to the rate of change of acceleration over time and indicates the smoothness of the motion and the wear and tear of the robot. Low jerk profiles indicate smooth human-like motion, reducing stress on the mechanical components, while high jerk can lead to increased wear and tear of the robot, raising maintenance costs and energy consumption.
Therefore, it is not straightforward to achieve the optimal timing law in the presence of noise.






- Integration of LfD into already-existing robotic setups: since the transformation from mass production to mass customization is not sudden, and happens gradually over time, the already-existing robotic setups which are traditionally programmed cannot shift to a flexible LfD-based solution all of a sudden. Not only is it impractical, but also it causes a huge downtime even if we attempt to transform the whole setup altogether.
% State machine is Modular
- Accuracy: When it comes to manufacturing, the success rate of the robotic task becomes directly relevant to how accurate the task is being executed. The notion of accuracy is subjective and differs from one task to another, but generally is encoded in the human demonstrations. e.g. in small-part assembly, the success of the task depends on how accurate the robot is, when it comes to manipulating the objects. The accuracy of the LfD outcome mainly relies on the accuracy of the demonstration and how accurately the human operator has provided the demonstration
- cycle time: in order to provide accurate demonstrations, the human will take longer to demonstrate, since it is cognitively demanding to demonstrate with a high accuracy and at a high speed! therefore, since the demonstration is slow, the LfD outcome will naturally be slow
- Noise: During the process of demonstration, noise can occur due to sensors reading the joint values, or hand trembling. The produced noise can make it difficult to detect the demonstration from the noise.



==> Sections/drafts/mass_customization.tex <==
% This is the context, what has happened. there is a shift from mass production to mass customization and these changes have happened in the manufacturing industry

- from fixed limited products to many variants
- from rigid manufacturing to flexible production based on customer (market) demand
- from structured (fixed) robot setup to unstructured (flexible) robot setup
- Challenges related to vision/perception and programming

% Mass Production
- Characterized by dedicated production lines for large volumes of identical products.
- Utilizes basic industrial robots performing repetitive tasks.
- Linear supply chains with limited flexibility

% Mass Customization
- Incorporates Flexible Manufacturing Systems, allowing quick reconfiguration of machinery and production lines to handle varied products without significant downtime.
- Employs advanced robotics with enhanced capabilities such as vision systems, AI-driven decision-making, and greater dexterity, enabling them to handle diverse tasks and adapt to different product designs.
- Integrated, responsive supply chains that utilize real-time data to manage inventory and logistics dynamically, supporting customization.
- Modular design



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The transition from mass production to mass customization in manufacturing has been driven by the increasing demand for personalized products in smaller batch sizes. This shift necessitates adaptable robotic systems that can efficiently handle the variability and complexity associated with customized production (Romiti et al., 2022). Traditional manufacturing methods focused on mass production are no longer sufficient to meet the requirements of mass customization, leading to the need for more flexible and reconfigurable robotic manipulators (Dogra et al., 2020). These manipulators are designed to be custom-tailored for specific tasks in collaborative environments such as manufacturing, maintenance, and services, enabling companies to address the challenges posed by high levels of customization (Arrais et al., 2020).

Robotic manipulation plays a crucial role in enabling the transition to mass customization by automating processes that require precision, repeatability, and flexibility (Eimontaite et al., 2018). The development of collaborative robotic systems that can mimic the motions of skilled technicians is essential for industries aiming to cope with the increasing demand for customized products (Arrais et al., 2020). Additionally, the use of modular and reconfigurable robotic systems allows for effortless creation of safe robots through self-programming and self-verification, facilitating quick adaptation to changing production needs (Althoff et al., 2019).

Furthermore, the integration of robotics in manufacturing processes not only enhances productivity but also reduces labor costs associated with small-scale production of custom-made products (Shauri  Nonami, 2011). The design and manufacturing speed of robots, along with the ease of composing custom designs, have the potential to democratize access to customized robots for various industrial applications (Önal et al., 2015). By leveraging advancements in robotics, companies can streamline their production processes, optimize efficiency, and meet the growing consumer demand for personalized products in the era of mass customization.

% References:
% Althoff, M., Giusti, A., Liu, S., & Pereira, A. (2019). Effortless creation of safe robots from modules through self-programming and self-verification. Science Robotics, 4(31). https://doi.org/10.1126/scirobotics.aaw1924
% Arrais, R., Costa, C., Ribeiro, P., Rocha, L., Silva, M., & Veiga, G. (2020). On the development of a collaborative robotic system for industrial coating cells. The International Journal of Advanced Manufacturing Technology, 115(3), 853-871. https://doi.org/10.1007/s00170-020-06167-z
% Dogra, A., Padhee, S., & Singla, E. (2020). An optimal architectural design for unconventional modular reconfigurable manipulation system. Journal of Mechanical Design, 143(6). https://doi.org/10.1115/1.4048821
% Eimontaite, I., Gwilt, I., Cameron, D., Aitken, J., Rolph, J., Mokaram, S., … & Law, J. (2018). Language-free graphical signage improves human performance and reduces anxiety when working collaboratively with robots. The International Journal of Advanced Manufacturing Technology, 100(1-4), 55-73. https://doi.org/10.1007/s00170-018-2625-2
% Romiti, E., Malzahn, J., Kashiri, N., Iacobelli, F., Ruzzon, M., Laurenzi, A., … & Tsagarakis, N. (2022). Toward a plug-and-work reconfigurable cobot. Ieee/Asme Transactions on Mechatronics, 27(5), 3219-3231. https://doi.org/10.1109/tmech.2021.3106043
% Shauri, R. and Nonami, K. (2011). Assembly manipulation of small objects by dual‐arm manipulator. Assembly Automation, 31(3), 263-274. https://doi.org/10.1108/01445151111150604
% Önal, Ç., Tolley, M., Wood, R., & Rus, D. (2015). Origami-inspired printed robots. Ieee/Asme Transactions on Mechatronics, 20(5), 2214-2221. https://doi.org/10.1109/tmech.2014.2369854
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The transition from mass production to mass customization in the context of robotic manipulation signifies a significant evolution in manufacturing paradigms. Mass production, known for the large-scale production of standardized goods, has historically dominated the industrial landscape (Radder  Louw, 1999). However, the growing consumer demand for personalized and unique items has led to a notable shift towards mass customization, where products are tailored to individual customer preferences (Dogra et al., 2020). This transformation has necessitated adjustments in manufacturing processes, including the adoption of more flexible and adaptable robotic systems to efficiently produce customized goods (Romiti et al., 2022).

Robotic manipulation plays a pivotal role in facilitating the shift from mass production to mass customization. Traditional industrial robots have been crucial in automating manufacturing processes and achieving economies of scale in mass production environments (Faidallah et al., 2022). Nevertheless, as the focus transitions towards producing customized products in smaller batch sizes, the necessity for robotic systems that can swiftly adapt to changing requirements becomes crucial (Romiti et al., 2022). This need for adaptability is further underscored by the imperative to minimize maintenance downtime in highly flexible production settings (Romiti et al., 2022).

The emergence of collaborative robots, or cobots, has significantly contributed to enabling the transition to mass customization (Romiti et al., 2022). These robots are designed to work alongside human operators, fostering a more flexible and agile production process (Villani et al., 2018). The capability of cobots to collaborate with human workers in industrial settings enhances safety and allows for intuitive interaction, making them well-suited for environments with varied and frequently changing tasks (Villani et al., 2018). This collaborative human-robot interaction approach is particularly advantageous in scenarios where customization demands a high level of flexibility and adaptability (Villani et al., 2018).

Additionally, the concept of modular reconfigurable manipulation systems has gained prominence in the realm of mass customization (Dogra et al., 2020). By designing robotic manipulators that can be easily reconfigured or customized to suit specific tasks, manufacturers can achieve enhanced flexibility in their production processes (Dogra et al., 2020). This modularity enables the seamless integration of different end-effectors or tools, allowing the same robotic system to perform a range of tasks without extensive reprogramming or retooling (Dogra et al., 2020).

In the domain of mass customization, the development of self-programming and self-verifying robots has emerged as a promising avenue to streamline the adaptation of robotic systems to evolving production needs (Althoff et al., 2019). These robots can effortlessly create and verify safe behaviors, enabling them to quickly learn and adapt to new tasks without extensive manual programming (Althoff et al., 2019). This autonomous learning capability is particularly valuable in dynamic production environments with evolving requirements (Althoff et al., 2019).

Furthermore, the integration of artificial intelligence and advanced control systems has played a pivotal role in enhancing the capabilities of robotic manipulators for mass customization (Althoff et al., 2019). By leveraging AI algorithms, robots can optimize their movements, adapt to changing environments, and self-diagnose potential issues to ensure continuous operation in customized production settings (Althoff et al., 2019). This level of intelligence and autonomy is essential for meeting the demands of mass customization while upholding efficiency and productivity (Althoff et al., 2019).

The transition towards mass customization has also driven innovations in robotic design and architecture to better support customized production processes (Hassan et al., 2017). For instance, studies on optimal base placements for multiple autonomous robots have been conducted to enhance collaboration and productivity in customized manufacturing environments (Hassan et al., 2017). Through strategic robot deployment and interaction optimization, manufacturers can achieve higher efficiency and customization levels in their production processes (Hassan et al., 2017).

In conclusion, the shift from mass production to mass customization concerning robotic manipulation signifies a fundamental transformation in manufacturing practices. This evolution is fueled by the escalating demand for personalized products and the necessity for flexible production systems that can rapidly adapt to changing requirements. Collaborative robots, modular reconfigurable systems, self-programming capabilities, and advanced AI integration are key facilitators of this transition, enabling manufacturers to efficiently produce customized goods in smaller batch sizes. By embracing these technological advancements and innovative approaches to robotic manipulation, companies can effectively navigate the complexities of mass customization and remain competitive in today's dynamic market landscape.

% References:
% Althoff, M., Giusti, A., Liu, S., & Pereira, A. (2019). Effortless creation of safe robots from modules through self-programming and self-verification. Science Robotics, 4(31). https://doi.org/10.1126/scirobotics.aaw1924
% Dogra, A., Padhee, S., & Singla, E. (2020). An optimal architectural design for unconventional modular reconfigurable manipulation system. Journal of Mechanical Design, 143(6). https://doi.org/10.1115/1.4048821
% Faidallah, E., Maged, S., Alsamanty, M., Hossameldin, Y., & Abdrabbo, S. (2022). Design and control implementation of adaptive soft gripper installed on kuka kr6 r900 robot arm. Engineering Research Journal - Faculty of Engineering (Shoubra), 51(4), 239-248. https://doi.org/10.21608/erjsh.2022.156200.1073
% Hassan, M., Liu, D., & Paul, G. (2017). Collaboration of multiple autonomous industrial robots through optimal base placements. Journal of Intelligent & Robotic Systems, 90(1-2), 113-132. https://doi.org/10.1007/s10846-017-0647-x
% Radder, L. and Louw, L. (1999). Mass customization and mass production. The TQM Journal, 11(1), 35-40. https://doi.org/10.1108/09544789910246615
% Romiti, E., Malzahn, J., Kashiri, N., Iacobelli, F., Ruzzon, M., Laurenzi, A., … & Tsagarakis, N. (2022). Toward a plug-and-work reconfigurable cobot. Ieee/Asme Transactions on Mechatronics, 27(5), 3219-3231. https://doi.org/10.1109/tmech.2021.3106043
% Villani, V., Pini, F., Leali, F., & Secchi, C. (2018). Survey on human–robot collaboration in industrial settings: safety, intuitive interfaces and applications. Mechatronics, 55, 248-266. https://doi.org/10.1016/j.mechatronics.2018.02.009
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The transformation from mass production to mass customization represents a significant shift in manufacturing paradigms, largely driven by advances in robotic manipulation. Traditionally, mass production focused on manufacturing large quantities of standardized products, emphasizing efficiency, cost reduction, and high output. This method relied on standardization, economies of scale, and the use of assembly lines where work was divided into simple, repetitive tasks. Although highly efficient, mass production offered limited flexibility, making changes in design or customization difficult and costly.

In contrast, mass customization combines the efficiencies of mass production with the personalization of custom-made products, allowing for high-volume production of tailored goods. This approach emphasizes personalization, flexibility, and responsive manufacturing, enabling production systems to adapt to varying designs without significant downtime or increased costs. The shift towards mass customization is driven by the need to meet individual customer preferences while maintaining the benefits of large-scale production.

Robotic manipulation plays a crucial role in enabling mass customization. In traditional mass production, robots performed repetitive and precise tasks, improving efficiency and consistency. These robots were typically fixed-programmed for specific tasks, offering little room for variation. However, modern robotics in mass customization features flexible automation, where robots can be quickly reprogrammed to handle different tasks or product variations. Adaptive robots, equipped with advanced sensors and AI, can adjust to different products and processes dynamically.

Collaborative robots, or cobots, are also essential in this transition. Designed to work alongside humans, cobots provide the flexibility and precision needed for customized tasks while humans handle more complex decision-making processes. These robots are safe for human interaction, allowing for more flexible workspaces and production processes. The integration of AI and machine learning further enhances robotic capabilities, with predictive maintenance reducing downtime and AI-driven demand forecasting optimizing customization.

Advanced sensing and vision systems enhance robotic perception, allowing robots to recognize and manipulate various objects, crucial for customized production. These systems also ensure high-quality standards are maintained across varied products. Additive manufacturing, or 3D printing, complements robotic manipulation by enabling the creation of unique parts and products without the need for retooling, facilitating rapid prototyping and efficient customization.

The benefits of robotic manipulation in mass customization are manifold. Robots offer increased flexibility, handling a wide range of tasks and adapting to new products without extensive retooling. They also maintain cost efficiency through automation and efficient material use, while ensuring high-quality standards due to their precision and consistency. Additionally, automation and flexible production systems reduce lead times for customized orders.

Despite these advantages, the transition to mass customization with advanced robotics poses challenges. The initial investment for advanced robotic systems and their integration can be high. Skilled personnel are required to program, maintain, and operate these sophisticated systems. Moreover, ensuring seamless integration of robotics with existing systems and processes can be complex.

In conclusion, the shift from mass production to mass customization, facilitated by advancements in robotic manipulation, marks a major evolution in manufacturing. By leveraging flexible, adaptive, and intelligent robotic systems, manufacturers can efficiently produce customized products at scale, meeting diverse customer demands without sacrificing cost or quality. This transformation is reshaping industries and setting new standards for production efficiency and product personalization.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Sections/drafts/traditional_vs_lfd.tex <==
%%%%% Traditional Programming vs LfD
% Now with the changes happening, the current way of programming is no longer efficient (traditional programming) (why?)
% But LfD is here to rescue, being the suitable option for robot manufacturing in the context of mass customization (why?)

- While traditional programming was good for mass production, it no longer serves the purpose of mass customization
- why is it no longer good for mass customization? (we need to bring arguments for each item mentioned before for mass customization)

- coordinate programming is initially for mass production. the next solution is optimization-based, which is better for mass customization but still not good enough (why?)

- Programming via robot coordinates --> rigid, suitable for structured setups, working with offsets, requires robot expert
- Advanced motion planning and optimization --> smoother, human-like, and optimized motion, but requires modeling of the environment and providing custom-tailored constraints and cost functions to create the desired motion for the task, requires robot expert.
- for any new task or modification, the programming and implementation needs to be performed again, which leads to more production down time

% Manual Programming

% Motion Planning and Optimization

% LfD


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Traditional programming methods, which include hand-coded programs and optimization-based approaches, are increasingly unsuitable for mass customization due to their inherent limitations in flexibility, scalability, and adaptability. Hand-coded programs are highly specific and rigid, designed to perform predefined tasks with little room for variation. This rigidity makes it difficult to adapt to the diverse and dynamic requirements of mass customization. Furthermore, developing and modifying hand-coded programs for different tasks or product variations is time-consuming, leading to increased downtime and reduced productivity. Scaling these programs to accommodate a wide range of customizations is challenging as the complexity of the programming rises exponentially with the number of product variations.

Motion-planning and optimization-based approaches, while effective for specific tasks, present their own set of challenges. These methods involve creating detailed models and algorithms to optimize the robot's movements and actions, requiring significant computational resources and expertise. Although they can handle specific scenarios well, they are limited in adaptability. Adapting these methods to different products or customization requirements involves substantial reprogramming and re-optimization, which is not feasible for the high-mix, low-volume production typical of mass customization. Additionally, the process of motion planning and optimization can be slow, making it difficult to respond quickly to changes in customer demands or product designs.

Learning from Demonstration (LfD), also known as imitation learning, offers a more suitable approach for mass customization due to its flexibility, ease of adaptation, and efficiency in handling diverse tasks and product variations. LfD allows robots to learn new tasks by observing human demonstrations, enabling them to quickly adapt to new products or variations without the need for extensive reprogramming. This dynamic learning capability makes LfD particularly effective for environments where products change frequently and customization is the norm. By observing different demonstrations, robots can learn to handle a wide range of product variations and customization requirements, offering a level of adaptability that traditional programming methods cannot match.

One of the key advantages of LfD is its intuitive programming process. Instead of writing complex code, operators can teach robots through demonstrations, reducing the need for specialized programming skills. This simplification makes it easier to implement robotic systems in mass customization settings and facilitates rapid prototyping of new tasks and processes. By quickly demonstrating a new task, operators can have robots ready to perform customizations with minimal downtime, enhancing productivity and responsiveness. This approach significantly reduces the time required to develop and deploy new tasks, enabling robots to be trained in a fraction of the time it would take to hand-code programs or develop optimization models.

LfD also enables scalable solutions where robots can be easily retrained for new tasks or products, making it feasible to handle a large variety of customizations. This scalability is crucial for maintaining efficiency and meeting customer demands in mass customization environments. Additionally, LfD allows robots to continuously learn and improve from ongoing demonstrations and feedback, ensuring that they remain effective and efficient as customization requirements evolve. The integration of LfD with AI and machine learning techniques enhances the robot's ability to generalize from demonstrations and handle complex tasks with greater autonomy, further supporting the suitability of LfD for dynamic and varied production environments.

In conclusion, traditional programming methods, including hand-coded programs and motion-planning approaches, are limited by their rigidity, complexity, and lack of adaptability, making them unsuitable for the dynamic and diverse requirements of mass customization. Learning from Demonstration (LfD) offers a flexible, intuitive, and efficient approach to programming robots for mass customization. By enabling robots to learn tasks through observation and continuously adapt to new requirements, LfD supports the rapid and scalable production of customized products, meeting the demands of modern manufacturing environments.

==> Sections/fig_opt.tex <==
\begin{figure*}[ht]
    \centering
    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{ccc}
            \begin{subfigure}[b]{0.33\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/opt/joint_1_org.pdf}
                \label{fig:subfig1}
            \end{subfigure} &
            \begin{subfigure}[b]{0.33\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/opt/joint_1_org.pdf}
                \label{fig:subfig2}
            \end{subfigure} &
            \begin{subfigure}[b]{0.33\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/opt/joint_1_org.pdf}
                \label{fig:subfig3}
            \end{subfigure} \\
            
            \begin{subfigure}[b]{0.33\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/opt/joint_1_org.pdf}
                \label{fig:subfig4}
            \end{subfigure} &
            \begin{subfigure}[b]{0.33\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/opt/joint_1_org.pdf}
                \label{fig:subfig5}
            \end{subfigure} &
            \begin{subfigure}[b]{0.33\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/opt/joint_1_org.pdf}
                \label{fig:subfig6}
            \end{subfigure} \\
            
            \begin{subfigure}[b]{0.33\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/opt/joint_1_org.pdf}
                \label{fig:subfig7}
            \end{subfigure} &
            \begin{subfigure}[b]{0.33\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/opt/joint_1_org.pdf}
                \label{fig:subfig8}
            \end{subfigure} &
            \begin{subfigure}[b]{0.33\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/opt/joint_1_org.pdf}
                \label{fig:subfig9}
            \end{subfigure} \\
            
            \begin{subfigure}[b]{0.33\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/opt/joint_1_org.pdf}
                \label{fig:subfig10}
            \end{subfigure} &
            \begin{subfigure}[b]{0.33\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/opt/joint_1_org.pdf}
                \label{fig:subfig11}
            \end{subfigure} &
            \begin{subfigure}[b]{0.33\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/opt/joint_1_org.pdf}
                \label{fig:subfig12}
            \end{subfigure} \\
            
            \begin{subfigure}[b]{0.33\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/opt/joint_1_org.pdf}
                \label{fig:subfig13}
            \end{subfigure} &
            \begin{subfigure}[b]{0.33\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/opt/joint_1_org.pdf}
                \label{fig:subfig14}
            \end{subfigure} &
            \begin{subfigure}[b]{0.33\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/opt/joint_1_org.pdf}
                \label{fig:subfig15}
            \end{subfigure} \\
            
            \begin{subfigure}[b]{0.33\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/opt/joint_1_org.pdf}
                \label{fig:subfig16}
            \end{subfigure} &
            \begin{subfigure}[b]{0.33\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/opt/joint_1_org.pdf}
                \label{fig:subfig17}
            \end{subfigure} &
            \begin{subfigure}[b]{0.33\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/opt/joint_1_org.pdf}
                \label{fig:subfig18}
            \end{subfigure} \\
            
            \begin{subfigure}[b]{0.33\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/opt/joint_1_org.pdf}
                \label{fig:subfig19}
            \end{subfigure} &
            \begin{subfigure}[b]{0.33\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/opt/joint_1_org.pdf}
                \label{fig:subfig20}
            \end{subfigure} &
            \begin{subfigure}[b]{0.33\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/opt/joint_1_org.pdf}
                \label{fig:subfig21}
            \end{subfigure} \\
            
            \begin{subfigure}[b]{0.33\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/opt/joint_1_org.pdf}
                \label{fig:subfig22}
            \end{subfigure} &
            \begin{subfigure}[b]{0.33\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/opt/joint_1_org.pdf}
                \label{fig:subfig23}
            \end{subfigure} &
            \begin{subfigure}[b]{0.33\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/opt/joint_1_org.pdf}
                \label{fig:subfig24}
            \end{subfigure} \\
            
            \begin{subfigure}[b]{0.33\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/opt/joint_1_org.pdf}
                \label{fig:subfig25}
            \end{subfigure} &
            \begin{subfigure}[b]{0.33\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/opt/joint_1_org.pdf}
                \label{fig:subfig26}
            \end{subfigure} &
            \begin{subfigure}[b]{0.33\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/opt/joint_1_org.pdf}
                \label{fig:subfig27}
            \end{subfigure} \\
            
            \begin{subfigure}[b]{0.33\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/opt/joint_1_org.pdf}
                \label{fig:subfig28}
            \end{subfigure} &
            \begin{subfigure}[b]{0.33\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/opt/joint_1_org.pdf}
                \label{fig:subfig29}
            \end{subfigure} &
            \begin{subfigure}[b]{0.33\textwidth}
                \centering
                \includegraphics[width=\linewidth]{Figures/opt/joint_1_org.pdf}

                \label{fig:subfig30}
            \end{subfigure} \\
        \end{tabular}
    \end{minipage}
    \caption{Main Figure Caption}
    \label{fig:main}
\end{figure*}


==> Sections/introduction-draft.tex <==
\section{Introduction}
\label{sec:intro}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% This is the context, what has happened. there is a shift from mass production to mass customization and these changes have happened in the manufacturing industry

% Mass production
In the manufacturing industry, The transition from mass production to mass customization marks a significant evolution in manufacturing paradigms.
Mass production, known for the large-scale production of standardized goods, has historically dominated the industrial landscape \cite{radder1999mass}.
Traditionally, mass production focused on manufacturing large quantities of standardized products, emphasizing efficiency, cost reduction, and high throughput. This method relied on the use of assembly lines where work was divided into fixed, simple and repetitive tasks. Although highly efficient, mass production offered limited flexibility, making changes in design or customization difficult and costly.

% Mass Customization
The growing consumer demand for personalized and unique items has led to a notable shift towards mass customization, where products are tailored to market preferences.
Mass customization combines the efficiencies of mass production with the personalization of custom-made products, allowing for high-volume small-batch production of tailored goods.
The shift towards mass customization is driven by the need to meet customer preferences while maintaining the benefits of large-scale production.
The key idea is to allow a higher degree of flexibility without compromising the efficiency of mass production. (or while competing with the efficiency of mass production)

% Robotic Manipulation in mass production vs mass customization
Robotic manipulation plays a pivotal role in facilitating the shift from mass production to mass customization.
Since mass production is characterized by dedicated production lines for large volumes of identical products, traditional industrial robots were required to perform repetitive tasks in a highly structured production line, where the positions and movements of objects and parts were predetermined and consistent.
In contrast, mass customization requires flexible manufacturing systems that can swiftly reconfigure production lines to accommodate diverse products with minimal downtime. This environment requires advanced robotic systems equipped with vision technologies, AI-driven decision-making, and increased dexterity. These capabilities enable robots to perform a variety of tasks and adapt to different product designs. Consequently, the robots must operate in unstructured and dynamic environments, where the objects and required movements frequently change.

% Collaborative robots
The emergence of collaborative robots, or cobots, has significantly contributed to enabling the transition to mass customization \cite{romiti2021toward}. These robots are designed to work alongside human operators, fostering a more flexible and agile production process \cite{villani2018survey}. The capability of cobots to collaborate with human workers in industrial settings enhances safety and allows for intuitive interaction, making them well-suited for environments with varied and frequently changing tasks \cite{villani2018survey}. This collaborative human-robot interaction approach is particularly advantageous in scenarios where customization demands a high level of flexibility and adaptability \cite{villani2018survey}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Efficiency of Implementation, Efficiency of Operation
With cobots replacing traditional industrial robots for mass customization, it is necessary to rethink the programming methodologies used for deploying these robots in production. An ideal programming approach should not only enable seamless introduction of new tasks to the robotic setup, but also ensure a high throughput throughout the production. These factors can be referred to as "the efficiency of implementation" and "the efficiency of operation", respectively. The efficiency of implementation refers to the effort, time, resources, and costs required to implement a robotic task, and overall the process through which the robotic task turns from concept to operational status. On the other hand, the efficiency of operation focuses on maximizing throughput and success rates during the robot's actual working phase while reducing the operation costs. This involves ensuring that the cobots can perform their tasks accurately and in minimum time,  while minimizing the ongoing costs such as energy consumption and maintenance. 


% Traditional programming
Traditional programming approach involves manually writing coordinate-based scripts for the robot, providing a low-level sequence of behaviors to successfully execute tasks.
Such hand-coded programs are highly specific and rigid, designed to perform predefined tasks with little room for variation. While this approach was suitable for robot programming in mass production, This rigidity makes it difficult to adapt to the diverse and dynamic requirements of mass customization. 
Moreover, cobots are designed to operate in an unstructured and dynamic environment shared with humans. This significantly increases the complexity of programming compared to traditional industrial robots. Scaling these programs to accommodate a wide range of customizations will also exponentially increase the complexity of programming with respect to product variations. The increased complexity compromises the efficacy of the program in terms of optimality and production cycle time, affecting the efficiency of operation.
Therefore, developing and modifying hand-coded programs for different tasks or product variations becomes time-consuming, leading to increased downtime and low efficiency of implementation. Despite these limitations, many industrial cobots still natively support manual programming methods, with some features exclusively accessible via this method, e.g., digital input/output management, gripper functionalities, etc.

% Motion planning and optimization
To overcome some of the limitations of manual programming, methods based on motion planning and optimization have emerged.
These methods enable higher-level programming, avoiding the need to explicitly provide low-level motion coordinates.
Implementing these methods involves creating a model of the robot and its working environment and developing algorithms to optimize the robot's actions based on predefined costs and constraints.
This approach better handles the higher complexity of cobot task implementation by considering the dynamic and unstructured operating environment and adaptively finding the optimal behavior to execute tasks, enhancing the efficiency of operation.
However, these methodologies remain highly task-specific. Each task requires modifying the robot model and devising a set of costs and constraints to ensure successful and optimal solutions. 
Adapting these methods to different products or customization requirements involves substantial reprogramming, which is not efficient for the high-mix, low-volume production typical of mass customization. Additionally, both manual programming and motion planning and optimization require high levels of robotic expertise for implementation. This demands a robot expert to act as an intermediary between the task specialist and the robot, which directly impacts the efficiency of implementation by increasing the costs.

% LfD
The alternative and most recent paradigm for flexible programming of cobots is Learning from Demonstration (LfD). Also known as Imitation Learning (IL), LfD is the paradigm in which robots learn how to perform new tasks by observing and imitating human demonstrations. In contrast to manual programming, LfD does not require a robot expert to provide an explicit motion sequence, and offers an opportunity for non-experts to directly teach complex behaviors to the robot. Moervoer, as opposed to motion planning and optimization approach, LfD does not require modeling of the robot and its operating environment as well as explicit costs and constraints. LfD achieves optimal behavior by learning the implicit task requirements that are encoded in the human demonstration. Naturally, demonstrations dictate the requirements of a "successful" execution, i.e., an implicit representation of the constraints required to ensure optimal and reliable execution. By learning these requirements directly from the demonstration, LfD can reach optimal behavior and maximize the efficiency of operation without the need for a robot expert to model the environment or design individual optimization formulations for each task. Also, these conceptual advantages significantly enhance the efficiency of implementation by allowing non-expert users to directly program cobots in a rapid manner.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

While LfD offers significant conceptual advantages compared to other programming methods, their deployment in practical manufacturing settings requires careful consideration while posing several performance challenges with respect to the efficiency of implementation and the efficiency of operation. 
% Motivated by the challenges of the practical application of LfD in manufacturing, we tailor our design choices as well as our proposed solutions to maximize both the efficiency of implementation and operation.

% Efficiency of Implementation
In order to maximize the efficiency of implementation, it is necessary to consider various factors such as the cost of demonstration setup, as well as the human time and cognitive effort required for demonstration. According to \cite{ravichandar2020recent}, among the demonstration mechanisms, kinesthetic teaching stands out due to its minimal setup requirements and its suitability for ease of demonstration to cobots.
Moreover, to further reduce the time and effort required from humans, our focus is on one-shot demonstration, rather than providing an indefinite number of demonstrations. Among the LfD approaches, Dynamic Movement Primitive (DMP) is a well-established method which is able to learn and generalize from a single demonstration. The choice of DMP is also further motivated by its high explainability and low implementation effort.

%% Remove
There are two primary perspectives when providing task demonstration: allowing humans to demonstrate complete tasks at once, or demonstrating one subtask at a time and then composing the complete task hierarchy through a high-level language that does not require robotic expertise. The subtask approach proves to be more efficient since it simplifies the learning process by focusing on smaller modular components, increasing accuracy and reliability. It also eases the cognitive load on the human teacher, making the demonstration process less challenging. Furthermore, focusing on one subtask at a time allows for easier identification and correction of errors and inefficiencies, resulting in higher overall accuracy and reliability. In terms of flexibility and scalability, Subtasks can be reused and recombined for different tasks. This modular learning strategy accelerates training, reduces the need for demonstrating similar subtask over again. 

%% Remove
More importantly, demonstrating at the subtask level facilitates the integration of LfD into existing robotic setups during the transition from mass production to mass customization. One of the challenges of the deployment of LfD is to ensure a smooth integration of LfD components without completely overhauling the existing setup. Not every traditional functionality can be replaced by LfD-based modules.  For example, gripper functionalities or managing Digital Inputs/Outputs to communicate with PLCs or other components are typically programmed traditionally via the robot's exclusive platform. While the existing works mainly focus on the advancements of LfD itself, there is a need for an architecture that enables the coexistence of traditionally programmed modules and newly implemented LfD modules. This approach not only reduces the downtime during the transition but also allows for a practical and gradual transformation with higher implementation efficiency.

In order to overcome this challenge, we propose a programming framework based on Finite-State Machines (FSM), which allows for modular composition of various behaviors/actions. The FSM architecture enables the integration of subtasks learned via Learning from Demonstration (LfD), traditionally programmed modules, and any other arbitrary behavior modules in a cohesive manner. Composing a high-level task hierarchy in this architecture is also straightforward, as a finite number of building blocks need to be arranged to form the complete task. This ease of composition ensures that non-robot-experts can configure and manage the system effectively, making the process user-friendly.

% \begin{itemize}
%     \item \textbf{Simplified Learning Process.} By breaking complex operations into smaller modular components, LfD algorithm can isolate learning each subtask individually.
%     \item \textbf{Reduced Cognitive Load.} Subtask demonstration eases the cognitive load on the human teacher, making the demonstration process less challenging.
%     \item \textbf{Enhanced Error Correction.} Focusing on one subtask at a time allows for easier identification and correction of errors and inefficiencies, resulting in higher overall accuracy and reliability.
%     \item \textbf{Flexibility and Scalability.} Subtasks can be reused and recombined for different tasks, increasing the flexibility and scalability of the system. This modular learning strategy accelerates training, reduces the need for demonstrating similar subtask over again.
%     \item \textbf{Integration with Existing ecosystem.} Demonstrating at the subtask level facilitates the integration of LfD into existing robotic setups during the transition from mass production to mass customization. Ensuring seamless integration of robotics with existing systems and processes can be complex, and not every traditional functionality can be replaced by LfD-based modules. For example, gripper functionalities or managing Digital Inputs/Outputs to communicate with PLCs or other components are typically programmed traditionally via the robot's exclusive platform.
% \end{itemize}

% A crucial aspect of this modular architecture is composing the task hierarchy in a way that non-robotic experts can seamlessly implement and modify through high-level intuitive modular programming. This ensures that the system remains accessible and manageable for users without specialized robotic expertise.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Efficiency of Operation
The efficiency of operation can be directly evaluated by task success rates and production throughput.  Ideally, a 100\% success rate and maximum possible throughput would yield the highest number of products by the end of the day. However, achieving this ideal is challenging due to several factors encountered in practical settings. When capturing demonstrations, noise is often entangled in the recorded data. This noise can stem from errors in joint sensors as well as hand trembling and shaking during the demonstration. The presence of noise negatively impacts operational efficiency in two significant ways: accuracy and execution time.

\textbf{Accuracy:} Accuracy in LfD is determined by task-specific criteria that ensure the success of the task, similar to optimization-based approaches where constraints and costs guide an algorithm towards a successful solution. In human demonstrations, these constraints and costs are inherently encoded in the motion. For example, in a reaching task, the end-effector must approach the object from a specific direction to avoid collisions and grasp the object at the correct angle. These precise instructions are implicitly conveyed through human demonstration. However, noise can obscure these implicit cues, making them less effective. This degradation affects LfD algorithms' performance, making it challenging for the system to learn and generalize the intended motion, often leading to overfitting the noise and reducing task success rates.

Existing methods often rely on multiple demonstrations to regress noise-free demonstrations while maintaining accuracy. To numerically model the accuracy, they use the local variance of these demonstrations as a measure of significance for each segment: high local variability indicates low accuracy and vice versa. In contrast, we propose a novel approach where the measure of accuracy is represented as local tolerance values for each segment of a single demonstration. Unlike the current methods that depend on the variance profile of multiple demonstrations, our approach extracts these tolerance values from only one demonstration. This not only simplifies the process but also retains the critical information needed to maintain demonstration accuracy when removing noise.

Furthermore, the state-of-the-art learning approaches focus on robustifying against noisy demonstrations, but removing noise beforehand could allow the learning algorithm to better capture the noise-free demonstration.
In this work, we analyze how the learning performance of LfD can be enhanced by tailoring the learning methods towards learning from noise-free demonstrations rather than robustifying against sub-optimal demonstrations.

\textbf{Execution Time:} The execution time of robotic tasks is a crucial factor that directly influences production throughput. For instance, if the current execution time for producing a product is 150 seconds, a 24-hour plant can produce 576 products per day. Reducing the execution time by just 6 seconds increases daily production to 600 products, representing a 4\% increase in throughput. Human demonstrations are naturally slow due to the cognitive complexity of teaching accurate, detailed motions. Therefore, minimizing execution time is essential, requiring the most optimal timing law derived from slow demonstrations.

Achieving optimal demonstration timing law is not straightforward as it present two main issues. Firstly, as elaborated in [ref], demonstrations cannot usually sped up uniformly, hence a simple uniform scaling is not a feasible solution. It is necessary to allow the humans to also teach the correct timing law. Secondly, while existing methods allow humans to improve the timing law by locally speeding up the initial demonstration, the kinematic limits of the robot are often neglected. Noise in the demonstration causes erratic or jerky motion, leading to velocity and acceleration spikes that render the trajectory kinematically infeasible, without achieving an optimal timing. Besides, motion jerk, the rate of change of acceleration over time, is an indication of the smoothness of the motion. Low jerk profiles suggest smooth, human-like motion, reducing stress on mechanical components, while high jerk increases wear and tear, maintenance costs, and energy consumption.



% \begin{itemize}
%     \item As elaborated in [ref], demonstrations cannot usually sped up uniformly, hence a simple uniform scaling is not a feasible solution. It is necessary to allow the humans to also teach the correct timing law
%     \item Noise in the demonstration causes erratic or jerky motion, leading to velocity and acceleration spikes that render the trajectory kinematically infeasible. Motion jerk, the rate of change of acceleration over time, indicates the smoothness of the motion. Low jerk profiles suggest smooth, human-like motion, reducing stress on mechanical components, while high jerk increases wear and tear, maintenance costs, and energy consumption.
% \end{itemize}



Therefore, to optimize efficiency of operation, it is crucial to eliminate noise from demonstrations, maintain the accuracy of the demonstrations, and achieve a minimum-jerk motion to complete tasks successfully in the shortest possible time. To do so, we introduce DFL-TORO, a novel \textbf{D}emonstration \textbf{F}ramework for \textbf{L}earning \textbf{T}ime-\textbf{O}ptimal \textbf{R}obotic tasks via \textbf{O}ne-shot kinesthetic demonstration. DFL-TORO allows humans to intuitively provide demonstrations as well as modifying the timing law and obtaining task tolerances, yielding smooth, jerk-regulated, timely, and noise-free trajectories.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
our overal contributions --> a complete programing framework

- state machine architecture to seamless integration of heterogeneous modules in a high-level manner

- dfl-toro to enhance efficiency of implementation and operation in terms of accuracy and execution time + removing noise

- an alternative learning method for DMP which is tailored to better learn and generlize dmp behavior from noise-free demonstration, rather than being robust against suboptimal demonstration.


==> Sections/methodology-draft.tex <==
\section{DFL-TORO Methodology}
\label{sec:method}

% The effect of noise on demonstration
- show the dmp result with raw demonstrations, show how deviated it is!
- show dmp result with a simple filter (cutting off at the end, filter waypoint distance), show that it's a bit better, but not the best, here focus on the effect of noise in the jerk profile
- then show dmp output with smooth demonstration, highlight the fact that now the bottleneck is LWR/RBFN, contrast it with B-Spline which performs well
- a table to show a similarity metric for different kernel numbers 10, 20, 50, 100, vs B-Spline, for LWR/RBFN












%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{Figures/fig2.pdf}
    \caption{DFL-TORO workflow. Red arrows indicate interactive procedures with the human-robot in the loop.}
    \label{fig:overview}
    \vspace{-6mm}
\end{figure}

The DFL-TORO workflow (Fig. \ref{fig:overview}) is detailed as follows:
\begin{itemize}%[align=right,itemindent=2em,labelsep=2pt,labelwidth=1em,leftmargin=0pt,nosep]
    \item[\textbf{A)}] The human teacher provides an inherently noisy demonstration $q_o(t)$ to a $n$ DoF manipulator via kinesthetic guidance, where the underlying path is extracted and represented as $m$ waypoints, denoted by $w_i$ for $\forall i=1,\cdots,m$. The waypoints encode the joint configuration $Q_{w_i} \in \mathbb{R}^n$, as well as the end-effector's position $p_{w_i}=[x_{w_i}, y_{w_i}, z_{w_i}]^T \in \mathbb{R}^3$ and orientation $\theta_{w_i} \in \mathbb{S}^3$, represented as quaternion. 
    \item[\textbf{B)}] The ``Time Optimization" module computes the ideal timing $\tau_i \in [0,1]$ for  $\forall i=1,\cdots,m$ for each waypoint. 
    \item[\textbf{C)}] The ``Trajectory Generation" module solves a comprehensive optimization problem to minimize the jerk. Given that specific task tolerances are not extracted yet, default tolerance values $\epsilon^d_p \in \mathbb{R}^3$ and $\epsilon^d_\theta \in \mathbb{R}$ are incorporated to generate an initial trajectory. $\epsilon^d_p$ represents the tolerance in Cartesian position, while $\epsilon^d_\theta$  the angular difference tolerance. Consequently, the outcome of this hierarchical optimization procedure is a minimum-time, smooth trajectory $q_f(t)$. 
    \item[\textbf{D)}] The ``Refinement Phase" allows the teacher to interactively slow down and correct the timing law. The robot replays the trajectory, allowing the human teacher to visually assess the execution speed. The teacher can pinpoint areas where the speed is either unreliable or unsafe and determine which segments require slowing down. Since the current trajectory $q_f(t)$ is very rapidly executed, it leaves no time for humans to observe the motion and provide feedback. Therefore, the Refinement Phase operates at a reduced speed $V_0^r \in \mathbb{R}_+$, giving humans enough reaction time to make changes.
    \item[\textbf{E)}] The Refinement Phase provides revised timings for the trajectory, denoted as $\tau_i^r \in [0,1]$, as well as the task tolerances $\epsilon_p^i \in \mathbb{R}^3$ and $\epsilon_{\theta}^i \in \mathbb{R}$ extracted from human feedback. These updated values are subsequently fed to the Trajectory Generation module which leads to a fine-tuned trajectory $q_f^r(t)$ in accordance with the new timings and tolerances.
\end{itemize}

The steps of the proposed demonstration framework is provided in Algorithm \ref{alg:demo_framework}, and elaborated in the following. 

\subsection{Optimization-based Smoothing}
\label{sec:opt}
We employ B-Splines to represent trajectories in our approach. B-Splines are ideal for robot manipulator trajectory optimization due to their smoothness, local control, and efficient computation \cite{de1972calculating}. Their piecewise polynomial nature ensures smooth motion paths, making them highly suitable for complex motion planning. A B-spline curve is defined as a linear combination of control points $P_{i^*}, {i^*}=1,\cdots,\Bar{n}$ and B-spline basis functions $N_{{i^*},k}(s)$. Control points $P_{i^*}$ determine the shape of the curve. A B-Spline $\xi(s)$ of $k^{th}$ order with $\Bar{n}$ control points $P_1, P_2, ..., P_{\Bar{n}}$ is expressed as:
\begin{align}
\xi(s) = \sum_{{i^*}=1}^{\Bar{n}} N_{{i^*},k}(s) P_{i^*}, \label{eq:bspline}
\end{align}
where $s \in [0,1]$ is the normalized time. Let \( u_1 \leq u_2 \leq \ldots \leq u_{\Bar{m}} \) be the knots and \( \Bar{m} = \Bar{n}+k \), with
\begin{align}
N_{{i^*},1}(s) &= \begin{cases} 
1 & \text{if } u_{i^*} \leq s < u_{{i^*}+1} \\
0 & \text{otherwise}
\end{cases}, \nonumber \\
N_{{i^*},k}(s) &= \frac{s - u_{i^*}}{u_{{i^*}+k-1} - u_{i^*}} N_{{i^*},k-1}(s) \nonumber \\
&+ \frac{u_{{i^*+k}} - s}{u_{{i^*+k}} - u_{{i^*+1}}} N_{{i^*+1},k-1}(s). \nonumber
\end{align}
$\xi(s)$ is associated with a duration parameter $T$, which maps the normalized time $s$ into actual time $t$ \cite{de1972calculating}. $P_{i^*}$ and  $T$ are the optimization variables.
In the following, we describe two modules of optimization-based smoothing.

\subsubsection{Time Optimization Module}

The objective of this optimizer is to find the minimum-time trajectory $q_t(t)$ that strictly passes through all the waypoints $Q_{w_i}$. At this stage, we ignore constraints related to acceleration and jerk since the noise is still present in the path. Adding such constraints would prevent the optimizer from finding the ideal timings. B-Spline sub-trajectories $\xi_j$ for $\forall j=1,\cdots,m-1$ are used to represent the trajectory between every two adjacent waypoints $w_j$ and $w_{j+1}$, with control points $P_{{i^*},j}$ and durations $T_j$. Then, the time optimization problem is formulated as: 
\begin{subequations}    
\begin{align}
 (P^*_{{i^*},j},T^*_j) &= \argminx{P_{{i^*},j},T_j} \sum_{j=1}^{m-1} T_j, \label{eq:timeopt0} \\
% &\text{Minimize: } J = \sum_{j=1}^{m-1} T_j, \label{eq:timeopt0} \\\nonumber
% &\text{subject to: }  \\
q_j(t_j)&=\xi_j(\frac{t_j}{T_j}), \label{eq:timeopt1}\\
q_{\text{min}} &\leq q_j(t_j) \leq q_{\text{max}}, \label{eq:timeopt1.5} \\
v_{\text{min}} &\leq \dot{q}_j(t_j) \leq v_{\text{max}}, \label{eq:timeopt2} \\
\xi_j(0) &= Q_{w_{j}}, \label{eq:timeopt2.5} \\
\xi_j(1) &= Q_{w_{j+1}}, \label{eq:timeopt3} \\
\dot{\xi}_1(0) &= \dot{\xi}_{m-1}(1) = 0, \label{eq:timeopt4}
\end{align}
\end{subequations}
for $\forall t_j \in [0, T_j]$. \eqref{eq:timeopt1} relates the normalized and actual trajectories. We set bounds $q_{\text{min}}$, $q_{\text{max}}$, $v_{\text{min}}$ and $v_{\text{max}} \in \mathbb{R}^n$ for joint position and velocity as \eqref{eq:timeopt1.5} and \eqref{eq:timeopt2}, respectively. Note that ``$\leq$" represents element-wise inequality of vectors. Continuity constraints \eqref{eq:timeopt2.5} and \eqref{eq:timeopt3} are applied at the intersection of these sub-trajectories. \eqref{eq:timeopt4} enforces the trajectory to start and rest with zero velocity. The optimization yields an unrealistic trajectory due to the existing noise, with high acceleration and jerk values. \eqref{eq:timeopt0} determines the ideal timings $T^*_j$ to move through all waypoints with highest velocity, which provides normalized time $\tau_i$ defined as
\begin{align} \label{eq:tau_i}
\tau_i &= \begin{cases} 
\frac{\sum_{j=1}^{i-1} T^*_j}{T^*_{m-1}} & i \geq 2 \\
0 & i=1
\end{cases},
\end{align}
which sets the groundwork for the Trajectory Generation module, that addresses the full optimization problem.

\subsubsection{Trajectory Generation Module}
Given $\tau_i$, we fit one B-Spline across all the waypoints, denoted as $\xi_f$ with control points $P_{i,f}$ and duration variable $T_f$. We match the number of control points with the waypoints, i.e., $\Bar{n}=m$, giving flexibility to the optimizer to locally adjust the trajectory around each waypoint. The cost function is formulated as:
\begin{align}
    J_f = \alpha T_f + \beta \int_{0}^{1}||\dddot{\xi}_f||^2ds + \gamma  \sum_{i=1}^{m} ||P_{i,f} -Q_{w_i}||^2, \label{eq:mainopt0}
\end{align}
where $\alpha,\beta$ and $\gamma$ are positive weights. The term $\int_{0}^{1}||\dddot{\xi}_f||^2ds$ attempts to minimize the normalized jerk profile, exploiting the tolerances of waypoints. This strategy is crucial for eliminating noise while respecting the tolerances. The term $\sum_{i=1}^{m} ||P_{i,f} -Q_{w_i}||^2$ ensures that control points align closely with the original joint configurations at the waypoints. Given the robot manipulator's kinematic redundancy, an end-effector pose can correspond to multiple configurations. This term limits the robot's configuration null space, prompting the optimizer to remain near the initial configuration. The trajectory generation problem is formulated as follows: 
\begin{subequations}    
\begin{align}
\hspace{-3cm} (P^*_{i,f},T^*_f) &= \argminx{P_{i,f},T_f} 
\,J_f, \label{eq:mainopt0.5}\\
\hspace{-3cm} q_f(t) &=\xi_f(\frac{t}{T_f}), \label{eq:mainopt0.69} \\
\hspace{-3cm} q_{\text{min}} &\leq q_f(t) \leq q_{\text{max}}, \label{eq:mainopt0.75}\\
\hspace{-3cm} v_{\text{min}} &\leq \dot{q}_f(t) \leq v_{\text{max}}, \label{eq:mainopt1}\\
\hspace{-3cm} a_{\text{min}} &\leq \ddot{q}_f(t) \leq a_{\text{max}}, \label{eq:mainopt1.5} \\
\hspace{-3cm} J_{\text{min}} &\leq \dddot{q}_f(t) \leq J_{\text{max}},  \label{eq:mainopt2}\\
\hspace{-3cm} \xi_f(0) &= Q_{w_{1}}, \label{eq:mainopt3} \\
\hspace{-3cm} \xi_f(1) &= Q_{w_{m}}, \label{eq:mainopt4} \\
\hspace{-3cm}\dot{\xi}_f(0) &= \dot{\xi}_f(1) = 0, \label{eq:mainopt5} \\
\hspace{-3cm} (p_f(t),\theta_f(t)) &=  F_K(q_f(t)), \label{eq:mainopt5.5} \\
\hspace{-3cm} - \epsilon_p^i \leq p_f(&\tau_i T_f) - p_{w_i} \leq \epsilon_p^i, \label{eq:mainopt6} \\
\hspace{-1cm} \mathsf{QuatDiff}&(\theta_f(\tau_i T_f), \theta_{w_i}) \in [0, \epsilon_\theta^i], \label{eq:mainopt7}
\end{align}
\end{subequations}
for $\forall t \in [0, T_f]$.
We have introduced acceleration and jerk bounds  $a_{\text{min}}$, $a_{\text{max}}$, $J_{\text{min}}$ and $J_{\text{max}} \in \mathbb{R}^n$ in \eqref{eq:mainopt1.5} and \eqref{eq:mainopt2}, respectively, to ensure the trajectory's feasibility. Constraints \eqref{eq:mainopt3}-\eqref{eq:mainopt5} enforce the trajectory to start at $Q_{w_1}$ and rest at $Q_{w_m}$ with zero velocity.
\eqref{eq:mainopt5.5} represents the forward kinematic function $F_K$, which is used to assign the tolerance in the end-effector's Cartesian space with $p_f(t) = [x_f(t),y_f(t),z_f(t)] \in \mathbb{R}^3$ and $\theta_f(t) \in \mathbb{S}^3$. The goal is to limit the position and angle deviation of the end-effector at each waypoint $w_i$ to $\epsilon_p^i$ and $\epsilon_\theta^i$, via \eqref{eq:mainopt6} and \eqref{eq:mainopt7}, respectively, at normalized time $\tau_i$.
In \eqref{eq:mainopt6}, ``$\leq$" represents element-wise inequality of vectors. $\mathsf{QuatDiff}(.,.) \in [0,\pi]$ is a conventional function derived based on the dot product of quaternions to compute the absolute angle difference of two quaternions \cite{mccarthy1990introduction}:
\begin{align}
   \mathsf{QuatDiff}(\theta_1,\theta_2) = 2 \cdot \arccos(|\theta_1 \cdot \theta_2|). \label{eq:quatdiff}
\end{align}
Solving \eqref{eq:mainopt0.5} yields $P^*_{i,f}$, with which $q_f(t)$ is computed using \eqref{eq:bspline} and \eqref{eq:mainopt0.69}.

\SetKwInput{KwOutput}{Output}


\begin{algorithm}
% \footnotesize
    \caption{DFL-TORO Architecture}
    \label{alg:demo_framework}
    
    \SetNlSty{textcolor}{rulecolor}{gray!20}
    
    \textbf{\underline{(A): Kinesthetic Guidance}} \\
    \KwIn{Noisy human demonstration $q_o(t)$}
    \KwOutput{Path waypoints $W_i = \left( Q_{w_i}, p_{w_i}, \theta_{w_i} \right)$}
    \BlankLine

    \textbf{\underline{(B): Time Optimization}} \\
    \KwIn{$W_i$}
    Find ideal timings using \eqref{eq:timeopt0}-\eqref{eq:timeopt4} and \eqref{eq:tau_i} \\
    \KwOutput{Initial timings $\tau_i$}
    \BlankLine
    
    \textbf{\underline{(C): Trajectory Generation}} \\
    \KwIn{$W_i$, $\tau_i$, default tolerances $\epsilon_p^d, \epsilon_\theta^d$}
    Solve for smooth trajectory using \eqref{eq:mainopt0.5}-\eqref{eq:mainopt7} \\
    \KwOutput{Trajectory $q_f(t)$}
    \BlankLine

    \textbf{\underline{(D): Refinement Phase}} \\
    \KwIn{$q_f(t)$, human command $C(t), \eta$}
    Initialize $v(0)=V_0^r, s_r(0)=V_0^r \cdot t$ \\
    \While{Replaying Trajectory}{
    Compute $R(t)$ using \eqref{eq:filterC} \\
    % $\dot{v}(t) \gets R(t)$ \\
    % $\dot{s}_r(t) \gets v(t)$ \\
    Compute $s_r(t)$ using \eqref{eq:s_r} \\
    Send $\xi(s_r(t))$ to robot for interactive feedback
    }
    Compute new timings $\tau_i^r$ using \eqref{eq:tau_i_r}\\
    \For{each $w_i$}{
    $\epsilon_p^i \gets \Gamma_p(\tau_i)$ using \eqref{eq:tol}\\
    $\epsilon_\theta^i \gets \Gamma_\theta(\tau_i)$ using \eqref{eq:tol}
    }
    \KwOutput{New timings $\tau_i^r$, new tolerances $\epsilon_p^i, \epsilon_\theta^i$}
    \BlankLine

    \textbf{\underline{(E): Trajectory Fine-Tuning}} \\
    \KwIn{$W_i, \tau_i^r, \epsilon_p^i, \epsilon_\theta^i$}
    Re-optimize $q_f(t)$ via updated timings and tolerances using \eqref{eq:mainopt0.5}-\eqref{eq:mainopt7} \\
    \KwOutput{Optimal Demonstration $q_f^r(t)$}
    % \BlankLine
\end{algorithm}

% \begin{figure}[!htbp]
%     \begin{subfigure}[b]{\columnwidth}
%         \centering
%         \includegraphics[width=0.7\linewidth]{Figures/original.pdf}
%         %\vspace{-5mm}
%         \caption{Original Demonstration $q_o(t)$}
%         \label{fig:org}
%     \end{subfigure}

%     \begin{subfigure}[b]{\columnwidth}
%         \centering
%         \includegraphics[width=0.7\linewidth]{Figures/opt_t.pdf}
%         %\vspace{-5mm}
%         \caption{Time Optimization Output $q_t(t)$}
%         \label{fig:opt1}
%     \end{subfigure}
    
%     \begin{subfigure}[b]{\columnwidth}
%         \centering
%         \includegraphics[width=0.7\linewidth]{Figures/opt_f.pdf}
%         %\vspace{-4mm}
%         \caption{Trajectory Generation Output $q_f(t)$}
%         \label{fig:opt2}
%     \end{subfigure}
%     \caption{Evolution of RT1 from original to smooth time-optimal joint trajectory. Each color represents a distinct DoF.}
%     \label{fig:opt}
%     \vspace{-6mm}
% \end{figure}


\begin{figure*}[!t]
    \centering
    \begin{subfigure}[b]{0.31\textwidth}
        \includegraphics[width=1.04\textwidth]{Figures/original.pdf}
        \caption{Original Demonstration $q_o(t)$}
        \label{fig:org}
    \end{subfigure}
    \hfill % space between subfigures
    \begin{subfigure}[b]{0.31\textwidth}
        \includegraphics[width=\textwidth]{Figures/opt_t.pdf}
        \caption{Time Optimization Output $q_t(t)$}
        \label{fig:opt1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.31\textwidth}
        \includegraphics[width=\textwidth]{Figures/opt_f.pdf}
        \caption{Trajectory Generation Output $q_f(t)$}
        \label{fig:opt2}
    \end{subfigure}
    \caption{Evolution of RT1 from original to smooth time-optimal joint trajectory. Each color represents a distinct DoF.}
    \label{fig:opt}
    \vspace{-3mm}

\end{figure*}

\subsection{Refinement Phase}
\label{sec:refine}
During the Refinement Phase, the teacher can practically slow down the time progression and hence the trajectory velocity. To do so, the trajectory $q_f(t)$ with duration $T_f$ is replayed with a reduced speed $V_0^r = \frac{1}{\eta T_f} $ for $\eta > 1$, letting the human teacher observe and provide interactive feedback in the loop. This is achieved through a teleoperated command, $C(t) \in [-1,0]$, which functions like a brake pedal. It allows the teacher to safely and intuitively interact with the robot in real-time, controlling its velocity during execution. To attenuate noise or abrupt changes in $C(t)$, we pass it as the attractor point of a virtual spring-damper system:
\begin{align}
    \tau \ddot R(t) = K(C(t)-R(t)) - D \dot R(t). \label{eq:filterC}
\end{align}
By carefully setting the values of $\tau$, $K$, and $D$, we can configure \eqref{eq:filterC} to be critically damped, as well as adjust its settling time which, in turn, influences the delay in response to human command. The output $R(t) \in [-1,0]$ is used as a deceleration term to adjust the trajectory velocity, as follows.
\subsubsection{Velocity Adjustment}
\label{sec:vel}
Since $q_f(t)=\xi_f(s(t))$ where $s(t) = V_0^r \cdot t$, by adjusting $s(t)$ we can directly modify the timing law of the trajectory $q_f(t)$. Slowing down specific portions of $\xi_f(s(t))$ locally can be done by incorporating $R(t)$ as a notion of time deceleration, which leads to a modified mapping $s_r(t)$. We compute this new mapping throughout the refinement phase via a straightforward kinematic model:
\begin{align}
    \left\{ \begin{matrix}
        \dot v(t) = R(t) \\
        \dot s_r(t) = v(t)
    \end{matrix} \right., \quad
    \begin{matrix} 
    v(t) \in [V_{min}^r,V^r_0], \\
    s_r(t) \in [0,1]
    \end{matrix} \label{eq:s_r}
\end{align}
To prevent the robot from completely stopping, we bound $v(t)$ to a minimum execution speed $V_{min}^r \in \mathbb{R}_+$.  $s_r(t)$ and $\tau_i$ are used to determine the updated timing $\tau_i^r$ as
\begin{align} \label{eq:tau_i_r}
    \tau_i^r = \frac{s_r^{-1}(\tau_i)}{s_r^{-1}(\tau_m)},
\end{align}
where $s_r^{-1}$ is the inverse of $s_r$ obtained via interpolation. It is worth mentioning that refinement at the reduced speed $V_0^r$ applies the same proportional adjustment on the real speed of execution, as $\tau_i^r$ are in normalized time. 

\subsubsection{Tolerance Extraction}
\label{sec:tol}
To extract the tolerances, we posit a direct correlation between the value of $R(t)$ and the desired level of accuracy at a given point on the trajectory. This means, the more intensively the brake pedal is pressed, the greater the criticality of that trajectory portion, necessitating increased precision. This is captured by introducing the functions  $\Gamma_p(t)$ and $\Gamma_\theta(t)$, defined as:
\begin{align}
    \Gamma_\kappa(t) = (\epsilon_\kappa^{max} - \epsilon_\kappa^{min})(1-(-R(t))^{n+\zeta}) + \epsilon_\kappa^{min}, \label{eq:tol}
\end{align}
where $\kappa \in \{p,\theta\}$. In \eqref{eq:tol}, $R(t) = 0$ is associated with maximum tolerances $\epsilon_p^{max}$ and $\epsilon_\theta^{max}$, whereas a $R(t) = -1$ corresponds to the minimum tolerances $\epsilon_p^{min}$ and $\epsilon_\theta^{min}$. The parameters $\zeta$ and $n$ determine the shape and curve of $\Gamma_\kappa$. By computing $\Gamma_\kappa(\tau_i)$ for each waypoint, we extract the requisite tolerances and pass it along with $\tau_i^r$ for re-optimization. 

==> Sections/nomencl.tex <==
\nomenclature[A]{LfD}{Learning from Demonstration}
\nomenclature[A]{IL}{Imitation Learning}
\nomenclature[A]{DoF}{Degress of Freedom}
\nomenclature[A]{DMP}{Dynamic Movement Primitive}
\nomenclature[A]{GP}{Gaussian Process}
\nomenclature[A]{GMM}{Gaussian Mixture Model}
\nomenclature[A]{RL}{Reinforcement Learning}
\nomenclature[A]{AR}{Augmented Reality}
\nomenclature[A]{MANJ}{Maximum Absolute Normalized Jerk}
\nomenclature[A]{FR3}{Franka Research 3}
\nomenclature[A]{ROS}{Robot Operating System}
\nomenclature[A]{RT}{Reaching Task}
\nomenclature[A]{MT}{Moving Task}
\nomenclature[A]{AI}{Artificial Intelligence}
\nomenclature[A]{sEMG}{surface Electromyography}



\nomenclature[V]{$m$}{Number of waypoints}
\nomenclature[V]{$w_i$}{i-th waypoint}
\nomenclature[V]{$\bm{\mathfrak{q}}_{w_i}$}{Joint configuration of $w_i$}
\nomenclature[V]{$\bm{\mathfrak{p}}_{w_i}$}{End-effector position of $w_i$}
\nomenclature[V]{$x_{w_i}$}{x-coordinate of $w_i$}
\nomenclature[V]{$y_{w_i}$}{y-coordinate of $w_i$}
\nomenclature[V]{$z_{w_i}$}{z-coordinate of $w_i$}
\nomenclature[V]{$\bm{\theta}_{w_i}$}{Orientation quaternion of $w_i$}
\nomenclature[V]{$\bm{q}_o(t)$}{Original joint trajectory}
\nomenclature[V]{$n$}{Number of robot's DoF}


% \nomenclature[V]{$m$}{Number of waypoints}
% \nomenclature[V]{$w_i$}{i-th waypoint of set $\mathcal{W}$}
% \nomenclature[V]{$\bm{\mathfrak{q}}_{w_i}$}{joint configuration vector of $w_i$}
% \nomenclature[V]{$\bm{\mathfrak{p}}_{w_i}$}{end-effector cartesian position of $w_i$}
% \nomenclature[V]{$x_{w_i}$}{x position of $w_i$}
% \nomenclature[V]{$y_{w_i}$}{y position of $w_i$}
% \nomenclature[V]{$z_{w_i}$}{z position of $w_i$}
% \nomenclature[V]{$\bm{\theta}_{w_i}$}{orientation quaternion of $w_i$}
% \nomenclature[V]{$\bm{q}_o(t)$}{The original joint trajectory}
% \nomenclature[V]{$n$}{Robot's number of Degrees of Freedom (DoF)}


\nomenclature[V]{$\bm{\mathfrak{q}}_{min}$}{Lower joint configuration limit}
\nomenclature[V]{$\bm{\mathfrak{q}}_{max}$}{Upper joint configuration limit}
\nomenclature[V]{$\bm{\mathfrak{v}}_{min}$}{Lower joint velocity limit}
\nomenclature[V]{$\bm{\mathfrak{v}}_{max}$}{Upper joint velocity limit}
\nomenclature[V]{$\bm{\mathfrak{a}}_{min}$}{Lower joint acceleration limit}
\nomenclature[V]{$\bm{\mathfrak{a}}_{max}$}{Upper joint acceleration limit}
\nomenclature[V]{$\bm{\mathfrak{j}}_{min}$}{Lower joint jerk limit}
\nomenclature[V]{$\bm{\mathfrak{j}}_{max}$}{Upper joint jerk limit}

% \nomenclature[V]{$\bm{\mathfrak{q}}_{min}$}{lower bound on joint configuration limit}
% \nomenclature[V]{$\bm{\mathfrak{q}}_{max}$}{upper bound on joint configuration limit}
% \nomenclature[V]{$\bm{\mathfrak{v}}_{min}$}{lower bound on joint velocity limit}
% \nomenclature[V]{$\bm{\mathfrak{v}}_{max}$}{upper bound on joint velocity limit}
% \nomenclature[V]{$\bm{\mathfrak{a}}_{min}$}{lower bound on joint acceleration limit}
% \nomenclature[V]{$\bm{\mathfrak{a}}_{max}$}{upper bound on joint acceleration limit}
% \nomenclature[V]{$\bm{\mathfrak{j}}_{min}$}{lower bound on joint jerk limit}
% \nomenclature[V]{$\bm{\mathfrak{j}}_{max}$}{upper bound on joint jerk limit}


\nomenclature[V]{$\bm{q}_f(t)$}{Optimized joint trajectory}
\nomenclature[V]{$\bm{\epsilon}_p^i$}{Position tolerance for $w_i$}
\nomenclature[V]{$\epsilon_{\theta}^i$}{Orientation tolerance for $w_i$}
\nomenclature[V]{$\bm{q}_f^r(t)$}{Fine-tuned joint trajectory}

\nomenclature[V]{$\mathsf{QuatDiff}$}{Function to compute angular difference}
\nomenclature[V]{$\mathsf{F_K}$}{Forward kinematic function}

\nomenclature[V]{$\bm{p}_f(t)$}{Optimized position trajectory}
\nomenclature[V]{$\bm{\theta}_f(t)$}{Optimized orientation trajectory}


% \nomenclature[V]{$\bm{q}_f(t)$}{The optimized joint trajectory}
% \nomenclature[V]{$\bm{\epsilon}_p^i$}{tolerance bounds on the cartesian position of $w_i$}
% \nomenclature[V]{$\epsilon_{\theta}^i$}{tolerance bounds on the orientation angle of $w_i$}
% \nomenclature[V]{$\bm{q}_f^r(t)$}{The fine-tuned joint trajectory}

% \nomenclature[V]{$\mathsf{QuatDiff}(.,.)$}{function to compute absolute angular difference}
% \nomenclature[V]{$\mathsf{F_K}$}{forward kinematic function}

% \nomenclature[V]{$\bm{p}_f(t)$}{The optimized cartesian position trajectory}
% \nomenclature[V]{$\bm{\theta}_f(t)$}{The optimized orientation quaternion trajectory}

\nomenclature[V]{$x_f(t)$}{Optimized x-coordinate trajectory}
\nomenclature[V]{$y_f(t)$}{Optimized y-coordinate trajectory}
\nomenclature[V]{$z_f(t)$}{Optimized z-coordinate trajectory}

\nomenclature[V]{$\bm{p}_f^r(t)$}{Refined position trajectory}
\nomenclature[V]{$x_f^r(t)$}{Refined x-coordinate trajectory}
\nomenclature[V]{$y_f^r(t)$}{Refined y-coordinate trajectory}
\nomenclature[V]{$z_f^r(t)$}{Refined z-coordinate trajectory}

\nomenclature[V]{$\mathrm{v}_0^r$}{Reduced speed factor}

\nomenclature[V]{$\bm{\xi}_f(s)$}{Optimized joint trajectory in normalized time}
\nomenclature[V]{$T_f$}{Execution time of $\bm{\xi}_f(s)$}
\nomenclature[V]{$\tau_i$}{Normalized time at $w_i$}
\nomenclature[V]{$t_i$}{Actual time at $w_i$}
\nomenclature[V]{$\bm{P}_{\hat{i},f}$}{Control points for $\bm{\xi}_f(s)$}


% \nomenclature[V]{$x_f(t)$}{The optimized cartesian position trajectory}
% \nomenclature[V]{$y_f(t)$}{The optimized cartesian position trajectory}
% \nomenclature[V]{$z_f(t)$}{The optimized cartesian position trajectory}

% \nomenclature[V]{$\bm{p}_f^r(t)$}{The refined cartesian position trajectory}
% \nomenclature[V]{$x_f^r(t)$}{The refined cartesian position trajectory}
% \nomenclature[V]{$y_f^r(t)$}{The refined cartesian position trajectory}
% \nomenclature[V]{$z_f(^rt)$}{The refined cartesian position trajectory}

% \nomenclature[V]{$\mathrm{v}_0^r$}{Reduced speed factor in refinement phase}

% \nomenclature[V]{$\bm{\xi}_f(s)$}{The optimized joint trajectory in normalized time}
% \nomenclature[V]{$T_f$}{The decision variable for the execution time of $\bm{\xi}_f(s)$}
% \nomenclature[V]{$\tau_i$}{Decision variable for the normalized time when $\bm{\xi}_f(s)$ passes through $w_i$}
% \nomenclature[V]{$t_i$}{Decision variable for the actual time when $\bm{q}_f(t)$ passes through $w_i$}
% \nomenclature[V]{$P_{\hat{i},f}$}{Decision variable for the control points underlying $\bm{\xi}_f(s)$}

% % u_i, N_{i,k}, n bar, m bar
% % What is i^*


\nomenclature[V]{$\bm{q}_t(t)$}{Output trajectory from time optimization}
\nomenclature[V]{$\bm{\xi}_j(s)$}{B-spline for $\bm{q}_j(t)$}
\nomenclature[V]{$\bm{q}_j(t)$}{Sub-trajectories of $\bm{q}_t(t)$} 
\nomenclature[V]{$t_j$}{Actual time at $w_i$ for $\bm{q}_t(t)$}
\nomenclature[V]{$T_j$}{Execution time of $\bm{\xi}_j(s)$}
\nomenclature[V]{$T_j^*$}{Optimized $T_j$}
\nomenclature[V]{$\tau_i^*$}{Optimized $\tau_i$}

\nomenclature[V]{$J_f$}{Cost function for trajectory generation}
\nomenclature[V]{$\alpha$}{Weight parameter in $J_f$}
\nomenclature[V]{$\beta$}{Weight parameter in $J_f$}
\nomenclature[V]{$\gamma$}{Weight parameter in $J_f$}

\nomenclature[V]{$t$}{Actual time}
\nomenclature[V]{$s$}{Normalized time}

\nomenclature[V]{$\bm{P}^*_{\hat{i},f}$}{Optimized control points for $\bm{\xi}_f(s)$}
\nomenclature[V]{$T^*_f$}{Optimized execution time}

\nomenclature[V]{$\bm{\epsilon}_p^d$}{Default position tolerance}
\nomenclature[V]{$\epsilon_{\theta}^d$}{Default orientation tolerance}


% \nomenclature[V]{$\bm{q}_t(t)$}{The output trajectory from the time optimization module}
% \nomenclature[V]{$\bm{\xi}_j(s)$}{B-spline representing $\bm{q}_j(t)$}
% \nomenclature[V]{$\bm{q}_j(t)$}{The sub-trajectories making $\bm{q}_t(t)$}

% \nomenclature[V]{$t_j$}{Decision variable for the actual time when $\bm{q}_t(t)$ passes through $w_i$}
% \nomenclature[V]{$T_j$}{The decision variable for the execution time of $\bm{\xi}_j(s)$}
% \nomenclature[V]{$T_j^*$}{The optimized value of $T_j$}
% \nomenclature[V]{$\tau_i^*$}{The optimized value of $\tau_i$}

% \nomenclature[V]{$J_f$}{Cost function of the trajectory generation module}
% \nomenclature[V]{$\alpha$}{Weight parameter in $J_f$}
% \nomenclature[V]{$\beta$}{Weight parameter in $J_f$}
% \nomenclature[V]{$\gamma$}{Weight parameter in $J_f$}

% \nomenclature[V]{$t$}{actual/real time}
% \nomenclature[V]{$s$}{normalized time}

% \nomenclature[V]{$P^*_{\hat{i},f}$}{Optimized value of $P_{\hat{i},f}$}
% \nomenclature[V]{$T^*_f$}{Optimized value of $T_f$}

% \nomenclature[V]{$\bm{\epsilon}_p^d$}{default tolerance bounds on the cartesian position}
% \nomenclature[V]{$\epsilon_{\theta}^d$}{default tolerance bounds on the orientation angle}

\nomenclature[V]{$C(t)$}{Teleoperated brake command}
\nomenclature[V]{$s(t)$}{Time mapping function}
\nomenclature[V]{$\eta$}{Speed reduction factor}

\nomenclature[V]{$s_r(t)$}{Refined time mapping}

\nomenclature[V]{$\mathrm{v}_{min}^r$}{Minimum speed during refinement}
\nomenclature[V]{$v_r(t)$}{Derivative of $s_r(t)$}
\nomenclature[V]{$\Gamma_\kappa(t)$}{Tolerance function}
\nomenclature[V]{$\Bar{n}$}{Shape parameter of $\Gamma_\kappa(t)$}
\nomenclature[V]{$\zeta$}{Shape parameter of $\Gamma_\kappa(t)$}

\nomenclature[V]{$\bm{\epsilon}_p^{min}$}{Min position tolerance}
\nomenclature[V]{$\epsilon_{\theta}^{min}$}{Min orientation tolerance}
\nomenclature[V]{$\bm{\epsilon}_p^{max}$}{Max position tolerance}
\nomenclature[V]{$\epsilon_{\theta}^{max}$}{Max orientation tolerance}

\nomenclature[V]{$\tau_i^r$}{Refined timing law}


% \nomenclature[V]{$C(t)$}{Teleoperated brake command}
% \nomenclature[V]{$s(t)$}{Mapping function of the actual time to normalized time}
% \nomenclature[V]{$\eta$}{Execution speed reduction factor}

% \nomenclature[V]{$s_r(t)$}{Modified mapping of $s(t)$ after refinement}

% \nomenclature[V]{$\mathrm{v}_{min}^r$}{Minimum execution speed during refinement}
% \nomenclature[V]{$v_r(t)$}{First time derivative of $s_r(t)$}
% \nomenclature[V]{$\Gamma_\kappa(t)$}{Tolerance extraction function}
% \nomenclature[V]{$\Bar{n}$}{shape parameter of $\Gamma_\kappa(t)$}
% \nomenclature[V]{$\zeta$}{shape parameter of $\Gamma_\kappa(t)$}

% \nomenclature[V]{$bm{\epsilon}_p^{min}$}{Minimum tolerance bound on cartesian position}
% \nomenclature[V]{$\epsilon_{\theta}^{min}$}{Minimum tolerance bound on orientation angle}
% \nomenclature[V]{$bm{\epsilon}_p^{max}$}{Maximum tolerance bound on cartesian position}
% \nomenclature[V]{$\epsilon_{\theta}^{max}$}{Maximum tolerance bound on orientation angle}

% \nomenclature[V]{$\tau_i^r$}{Refined timing law}


\nomenclature[V]{$y$}{DMP position}
\nomenclature[V]{$\alpha_z$}{DMP constant}
\nomenclature[V]{$\beta_z$}{DMP constant}
\nomenclature[V]{$g$}{DMP goal state}
\nomenclature[V]{$f(x)$}{DMP nonlinear forcing term}
\nomenclature[V]{$x$}{DMP phase variable}
\nomenclature[V]{$\psi_\mathfrak{i}$}{DMP Gaussian basis functions}
\nomenclature[V]{$\mathrm{w}_\mathfrak{i}$}{DMP weight parameters}
\nomenclature[V]{$c_\mathfrak{i}$}{Center of $\psi_\mathfrak{i}$}
\nomenclature[V]{$h_\mathfrak{i}$}{Width of $\psi_\mathfrak{i}$}
\nomenclature[V]{$\alpha_x$}{DMP phase constant}

\nomenclature[V]{$N_{{\hat{i}},k}(s)$}{B-Spline basis functions}
\nomenclature[V]{$k$}{B-Spline degree}
\nomenclature[V]{$U$}{B-Spline knot set}
\nomenclature[V]{$u_{\hat{i}}$}{B-Spline knot values}
\nomenclature[V]{$\hat{n}$}{Number of B-Spline control points}


% \nomenclature[V]{$y$}{DMP system's position}
% \nomenclature[V]{$\alpha_z$}{DMP system's constant}
% \nomenclature[V]{$\beta_z$}{DMP system's position}
% \nomenclature[V]{$g$}{DMP system's goal state}
% \nomenclature[V]{$f(x)$}{DMP system's nonlinear forcing term}
% \nomenclature[V]{$x$}{DMP system's phase variable}
% \nomenclature[V]{$\psi_\mathfrak{i}$}{Gaussian basis functions for DMP training}
% \nomenclature[V]{$\mathrm{w}_\mathfrak{i}$}{DMP system's weight parameters}
% \nomenclature[V]{$c_\mathfrak{i}$}{center of $\psi_\mathfrak{i}$}
% \nomenclature[V]{$h_\mathfrak{i}$}{width of $\psi_\mathfrak{i}$}
% \nomenclature[V]{$\alpha_x$}{DMP phase system's position}


% \nomenclature[V]{$N_{{\hat{i}},k}(s)$}{B-Spline basis functions}
% \nomenclature[V]{$k$}{B-Spline degree}
% \nomenclature[V]{$U$}{Set of knot values of B-Spline}
% \nomenclature[V]{$u_{\hat{i}}$}{B-Spline knot values}
% \nomenclature[V]{$\hat{n}$}{number of B-Spline control points}

\nomenclature[V]{$t^*$}{Start time of teleoperated brake}

\nomenclature[V]{${\mathrm{DMP}}_o$}{DMP trained via $\bm{q}_o(t)$}
\nomenclature[V]{${\mathrm{DMP}}_f$}{DMP trained via $\bm{q}_f(t)$}
\nomenclature[V]{$\bm{q}_{o,dmp}(t)$}{Generalized trajectory via ${\mathrm{DMP}}_o$}
\nomenclature[V]{$\bm{q}_{f,dmp}(t)$}{Generalized trajectory via ${\mathrm{DMP}}_f$}
\nomenclature[V]{$\bm{q}_{s,dmp}(t)$}{Scaled trajectory via ${\mathrm{DMP}}_o$}

\nomenclature[V]{$\bm{p}_{o,dmp}(t)$}{Position trajectory of $\bm{q}_{o,dmp}(t)$}
\nomenclature[V]{$\bm{p}_{f,dmp}(t)$}{Position trajectory of $\bm{q}_{f,dmp}(t)$}
\nomenclature[V]{$\bm{p}_{s,dmp}(t)$}{Position trajectory of $\bm{q}_{s,dmp}(t)$}


% \nomenclature[V]{$t^*$}{The time human starts applying teleoperated brake}


% \nomenclature[V]{${\mathrm{DMP}}_o$}{The DMP trained via $\bm{q}_o(t)$}
% \nomenclature[V]{${\mathrm{DMP}}_f$}{The DMP trained via $\bm{q}_f(t)$}
% \nomenclature[V]{$\bm{q}_{o,dmp}(t)$}{Generalized trajectory via ${\mathrm{DMP}}_o$}
% \nomenclature[V]{$\bm{q}_{f,dmp}(t)$}{Generalized trajectory via ${\mathrm{DMP}}_f$}
% \nomenclature[V]{$\bm{q}_{s,dmp}(t)$}{Scaled trajectory generalized via ${\mathrm{DMP}}_o$}

% \nomenclature[V]{$\bm{p}_{o,dmp}(t)$}{Cartesian position trajectory of $\bm{q}_{o,dmp}(t)$}
% \nomenclature[V]{$\bm{p}_{f,dmp}(t)$}{Cartesian position trajectory of $\bm{q}_{f,dmp}(t)$}
% \nomenclature[V]{$\bm{p}_{s,dmp}(t)$}{Cartesian position trajectory of $\bm{q}_{s,dmp}(t)$}













==> Sections/related_work-draft.tex <==
\section{Background and Related Work}
\label{sec:works}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LfD for manufacturing

% LfD for suboptimal demonstrations
% lfd and suboptimal demonstrations
% lfd and optimizing lfd outcome with respect to smoothness, generalizability
according to \cite{li2024learning}, suboptimal demonstrations can reduce the performance of LfD and cause overfitting or underfitting on the non-optimal demonstrations.

One approach is to focus on augmenting the demonstrations in order to fine tune their data efficiency \cite{ma2022efficient, qian2020hierarchical}, which aims at compensating the suboptimal demonstrations via various methods such as data augmentation, self-exploration, etc. to improve the performance of learning.
Also another approach is feature extraction from demonstrations in order to extract the key information implicitly encoded \cite{he2021imitation}. It has a similar concept to the accuracy tolerances which also determines the key information in the demonstration. However, the feature extraction methods require multiple demonstrations.
the work in \cite{wu2021framework} focused on assessing the effectiveness of the newly added demonstrations, a way of quantifying how informative are the demonstrations in order to enhance the efficiency of data in the demonstration process.
To deal with the flaws and noises in LfD, \cite{wang2021optimised} attempted to deal with jerky demonstrations by introducing a Gaussian noise. However, this approach works when working with multiple demonstrations, not one-shot demonstrations

Several works have focused on improving the LfD output trajectory with respect to smoothness and generalizability (?)
the work in \cite{el2021itp},  the LfD outcome is optimized via RL by eliminating suboptimal demonstrations from the demonstration data, and keeping the more useful demonstrations. 
The work in \cite{ye2022bagging} utilized GMM to increase the robustness of LfD to suboptimal training data, and ensure that the reproduced trajectory maintains the required precision.

Recent literature in LfD for collaborative robots has shifted from focusing on robustness against sub-optimal demonstrations \cite{cao2022learning} towards assessing the information gain and quality of demonstrations \cite{wu2021framework,kalinowska2021ergodic}.

% DMP
among LfD learning methods such as GMM, GP, ProMP, etc, DMP has special attention mainly due to its explainability, ease of use, and its capability to learn from one-shot demonstration.
for DMP, there has been focus on obstacle avoidance\cite{zhai2022motion}, 
Although learning the forcing term via DMP is possible through GMMs, Deep neural networks, etc. they required multiple demonstrations, which is against the objective of this paper.
hence, our focus is on learning approaches that work with one-shot demonstration, which are

\cite{wang2016dynamic} --> modified kernels in the modeling of forcing term and used LWR to learn. they still use rbfs, which was originally good for noisy demonstrations. they also test it on a minimum jerk trajectory already.
plus, their metric for improvement is MSE!

\cite{liu2023cauchy} --> replaced gaussian distribution with Cauchy distribution.

\cite{lu2021constrained} --> mostly an effort for dmp with constraints, targetted for obstacle avoidance.

\cite{ginesi2021overcoming} --> they propose truncated gaussian basis functions - they use L2-Norm for numerical comparison - \bl{mollifier-like basis functions to be good approximators for the forcing term, while providing a faster and more stable learning phase. Moreover, being compactly supported, this new set of basis functions allows to update a DMP when only a portion of the trajectory has to be modified.}

idea --> you can also include the computation time - we can also argue on the parameters that need to be learned in different approaches (?!)
plus, you can show that with rbfs there is no guarantee that you get to the goal precisely in $\tau$ time. it might take longer, but we don't know the exact time. therefore, to get precisely to the point, we need to allow dmp to continue for an unknown amount of time, to get to the goal. this compromises the time efficiency --> you can also show it on yumi grasping, where a bit above the object means failed grasping.

also, you can fundamentally and conceptually argue that other approaches require discretization, but B-Spline from DFL-TORO is directly used with DMP (if you can work out the formulation!!)




% State Machines
In \cite{mitrevski2019reusable}, \bl{When developing robot functionalities, finite state machines are commonly used due to their straightforward semantics and simple implementation.} --> they implemented a python library 
in \cite{conner2018flexible} --> they also implemented a fsm program with ros and moveit

the use of FSM and lfd together was initially proposed in \cite{grollman2010can}.
\cite{sauer2019towards} --> create FSM from kinesthestic demonstrations and provide a user interface to allow non-experts to intuitively program robots. 

\cite{willibald2020collaborative} --> allowing non-experts to intuitively program conditional tasks via a task-representing graph. 
% they also allow for programming when an anomaly is detected (fault recovery behavior)
they continued their work in \cite{eiband2023collaborative}, where they allow users to also program recovery behaviors

in \cite{niekum2015learning} --> they take multiple demonstrations and extract the finite-state representation.





% DFL-TORO

\cite{ostanin2018programming} --> optimize trajectories for time and energy consumption, using multiple demonstrations

\cite{maeda2008easy} --> the non-expert moves the manipulator around the free space of the working environment, and then the robot records all that space as available space for optimizing the demonstration with respect to time


NURBS = Non-Uniform Rational B-Splines
\cite{aleotti2006robust} --> used NURBS for smoothing trajectories from demonstrations, one-shot, or multiple --> no objective on time or jerk

\cite{marino2016fast} --> filtered and reduced the points in the demonstration trajectory to fit a spline --> no optimization, no time, no jerk

\cite{muller2020one} --> use the points from demonstration to fit a piecewise trajectory with a tolerance initially set by user

\cite{lee2011incremental} --> there is a nominal demonstration averaged from multiple demonstrations. around the nominal demonstration, the user can refine the demonstration within a tube around the demonstration. the radius of the tube at each part is automatically determined based on the variance of the training data. 

\cite{biagiotti2023robot} --> one shot kinesthetic demonstration + EMG signal to determine the tolerance in one shot. the feeding all into a B-Spline (using b-spline is their attempt to eliminate noise)





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Related work expansion ideas
- LfD in general, with focus on learning from suboptimal demonstrations
- DMP in general, with a focus on one-shot + motivating LWR/RBFN
- LfD in manufacturing/assembly, with focus on remaining challenges (refers to the 2024 surveys below)
- The stuff you already wrote
- (Optimization approaches used in any stage of LfD)
- B-Splines


% 2024 - Obstacles and Opportunities for Learning from Demonstration in Practical Industrial Assembly: A Systematic Literature Review
this work mentions that literature focous is way too much on peg in hole, and there should be focus on other manufacturing stuff as well
this work mentions the challenge of execution time
this work says that many works don't take it into real practical robot manufacturing (we take it to yumi in production)
this work also mentions the challenges of integration and how smooth and seamless integration is still a challenege (related to state machine)


% Optimised Learning from Demonstrations for Collaborative Robots - wang2021optimised
mentions jerky demonstrations, but addressed with multiple demos not one-shot
to show the effect of noise, it plots the 3d path and marks the unsmooth parts.

% A robot learning from demonstration framework to perform force-based manipulation tasks
referenced for Root mean squared error as a metric of demonstration similarity

% Bagging for Gaussian mixture regression in robot learning from demonstration
referenced for euclidean distance as a metric of demonstration similarity

% Learning from demonstration for autonomous generation of robotic trajectory: Status quo and forward-looking overview
quote from ref "while jerk, as a derivative of acceleration, reflects the presence of unfavored points in the demonstrations to be removed or further optimized"
it also highlights that collecting demonstration is expensive, point for one-shot demonstration
it has also explicitly called for the optimization of DMP to address errors between demonstration goal and executed goal

% biagiotti2023robot
\bl{a common characteristic of almost all the proposed approaches is the need for suppressing noise and unwanted/unnecessary motions that inevitably affect human demonstrations. To cope with these issues, the basic solution consists in recording multiple demonstrations, which are performed by an expert user, and then applying some kind of averaging or optimization method.}
\bl{n the context of probabilistic approaches, the differences among the input trajectories are translated into different variance levels of the stochastic processes used to model the task\cite{schneider2010robot,calinon2007learning}}
\bl{In \cite{delson1994robot}, variations between multiple demonstrations performed by a human operator are exploited to define the boundaries of a region free from obstacles. Then, a piecewise linear segment trajectory, fully contained in this admissible region, is built up to minimize the geometric path of the robot. In this approach, the human inconsistency in repeating the same desired trajectory is not treated as a noise to be canceled but is considered a measure of accuracy required by the task.}
\bl{As abovementioned, the generality of the PbD methods relies on multiple demonstrations of the same task, while only a few cases are based on a one-shot demonstration despite the clear advantages in terms of required effort and time for programming.}








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Integrating LfD into existing setups
In recent years, Learning from Demonstration (LfD) has evolved significantly, reaching a level of maturity suitable for real-world applications. Coupled with the emergence of mass customization, this advancement presents both opportunities and challenges for deploying LfD in robot manufacturing. There has been a significant focus on developing LfD methodologies and algorithms to enhance learning and generalization performance, precision and accuracy, as well as robustness and safety. However, a critical practical aspect of integrating LfD into existing robotic setups in the manufacturing sector has been overlooked.

Robots in manufacturing environments are surrounded by other equipment, such as Programmable Logic Controllers (PLCs), which are traditionally programmed by robot experts. It is impractical to completely and suddenly eliminate the need for these experts, as many functionalities are still only natively supported by the robot's exclusive traditional programming frameworks, such as RAPID for ABB robots. To address this, we need a modular architecture that enables robot experts to develop essential modules using traditional programming while allowing other modules to be replaced by LfD. 


While some modules are implemented by robot experts, the final high-level programming should be accessible to non-expert users, allowing them to easily arrange building blocks to create the complete robot program. To meet these requirements, we propose a Finite State Machine (FSM) architecture. This architecture facilitates the implementation of various self-contained independent modules, which can be developed either traditionally by robot experts or through LfD by human teachers. We ensure structured communication between these modules without the need for additional programming, allowing for high-level, easy programming by simply arranging the building blocks. Additionally, we propose a pool of common knowledge, accessible to all modules, to enable automated data transfer among them. This approach simplifies the integration of LfD into existing robotic manufacturing setups, leveraging the strengths of both traditional programming and LfD.


% Execution Time
To address the issue of slow demonstration, several studies focused on the isolation of demonstrating path and timing, allowing humans to teach the path and the timing law of demonstrations separately. Authors in \cite{nemec2018efficient} explore methods based on incremental learning to let human teacher adjust the speed of their initial demonstrations, integrating human feedback into velocity scaling factors within the DMP formulation. The work in \cite{simonivc2021analysis} further investigates the refinement of both path and speed through kinesthetic guidance, enabling teachers to fine-tune their demonstrations in real-time, thereby enhancing the quality of the learned trajectories. Moreover, the study of \cite{meszaros2022learning} utilizes teleoperated feedback to locally speed up the task execution. Their work clearly signifies the importance of a well demonstrated timing law in achieving high task success rates. Building upon these works, our approach incorporates the robot's kinematic limits into an optimization problem, solving for the best feasible timing law for the demonstrated path. Then, instead of merely speeding up, we permit users to ``slow down" demonstrations until reliable execution is achieved, and hence ensure the optimal timing. As opposed to other works, optimizing for the timing law provides guarantee that the best achievable execution time is calculated, while the ability to slow down the demonstration provides direct control to the human teacher in order to make the task execution reliable and successful while maintaining fast performance.

% Accuracy
In the process of removing noise from demonstrations, it is essential to highlight the importance of maintaining the integrity and accuracy of the demonstration, while giving freedom to the noise removal algorithm to slightly deviate from the original demonstration. To achieve this, a robust measure of tolerance must be established to represent the accuracy of the demonstration and state how much deviation is acceptable. Studies such as \cite{tsai2020constrained} and \cite{calinon2016tutorial} emphasize using task variability tolerances to adjust a robot's compliance, with low impedance settings employed when high variability is measured, thereby allowing for more deviations in human demonstrations. The main idea is to align multiple demonstrations of a task and use the variance of each segment of demonstration as a measure of significance or required accuracy. For example, the part of the motion that was highly similar in all demonstrations indicate that an accurate behavior is expected to perform, while the part where motion is variant among the demonstration shows that the motion can deviate more while maintaining the accuracy of the task. The same concept can also be utilized to extract tolerance values for noise removal. However, while existing approaches often rely on multiple demonstrations to statistically extract these tolerances \cite{hu2022robot,roveda2020assembly}, we propose a novel approach to discern tolerances from a single demonstration. Grounded in the psychological observation that humans naturally slow down when aiming for precision \cite{fitts1954information}, our method captures tolerances during periods where the demonstrator slows down. Although demonstrations are presented in joint space, we extract tolerances in the Cartesian space, emphasizing the end-effector pose as the task's crucial point.


% Dealing with noise in LfD
Recent literature in LfD for collaborative robots has shifted from focusing on robustness against sub-optimal demonstrations \cite{cao2022learning} towards assessing the information gain and quality of demonstrations \cite{wu2021framework,kalinowska2021ergodic}. However, there were not a significant focus on how demonstration noise is affecting LfD performance, as well as how this noise can be removed. The study in \cite{chen2018playback} offers a detailed comparison of various smoothing algorithms, and the noise-removing effect of RBF-based methods like DMPs. However, without careful hyperparameter tuning, they risk overfitting and noise replication. The study concludes that optimization-based smoothing is more effective in preserving demonstration features and improving information gain. Given that demonstrations do not have a set ground truth, distinguishing signals from noise is not trivial. Therefore, we bound the demonstration trajectory to the extracted tolerance values to ensure that the authenticity of the demonstration is preserved. Within this context, some works have omitted tolerances \cite{shyam2019improving} or used fixed user-defined tolerances \cite{muller2020one}. However, our approach extracts these tolerances directly from human demonstrations and incorporates them into the optimization.

To address the smoothing problem and deal with high jerk values, the simultaneous optimization of timing and jerk poses a challenge as it might lead to an infeasible problem. This stems from the fact that applying path constraints requires knowledge of the relative time when each part of the path is reached. On the other hand, such timings cannot be considered as decision variables, since the underlying trajectory representation is a piece-wise polynomial \cite{yang2018new}. Also, the original timing of the demonstration is not optimal. We address these challenges by solving the problem in two steps, where first the timing is optimized and then the jerk profile is regulated by removing the noise. To the best of our knowledge, the impact of optimizing the original demonstration on LfD performance has not been explored in previous research. Our study is the first attempt to showcase the performance of optimization-based smoothing as an additional layer with respect to the LfD output.

By adding optimization-based smoothing to the LfD process, we can always guarantee a noise-free demonstration. This raises questions about the effectiveness of common learning approaches used in LfD methods, which are designed to be robust to noise to some extent. The question is, with the noise eliminated from demonstrations, how can we improve the learning methodologies so that they learn and generalize the noise-free demonstration, compared to attempting to robustly learn from noisy demonstrations. To address this question, we use DMP as a case study and provide an alternative learning method which can be trained from optimal demonstrations, and compare its performance to the well-established Locally-Weighted-Regression (LWR) method which is commonly used as a baseline to learn from noisy demonstration. The RBF nature of LWR automatically deals with noisy demonstrations. However, its performance is affected when it comes to replication and generalization. In contrast, we propose an approach based on B-Splines. While B-Splines are not inherently robust against noise, they outperform LWR when having noise-free demonstrations. We show that our LfD framework based on noise-free demonstrations can provide a better learning and generalization compared to conventional LfD approaches where the effect of noise is partially or completely neglected.










%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% % Recent literature has shifted from focusing on robustness against sub-optimal demonstrations \cite{cao2021learning,cao2022learning} towards assessing the information gain and quality of demonstrations \cite{wu2021framework,kalinowska2021ergodic}. Specifically, in \cite{wu2021framework}, the authors underscore that poor demonstrations significantly impact learning outcomes.

% % Several studies have used incremental learning to improve the quality of human demonstrations. In \cite{nemec2018efficient}, the authors introduced a method for humans to adjust the speed of their initial demonstration, integrating human feedback into a velocity scaling factor within the Dynamic Movement Primitive (DMP) formulation. \cite{simonivc2021analysis} focused on allowing humans to refine both path and speed through kinesthetic guidance. Meanwhile, \cite{meszaros2022learning} employed teleoperated feedback for a grocery pick-and-place task to ensure faster and reliable task execution. This work was expanded in \cite{montero2022solving} for a precise assembly task. However, none of these studies factored in the robot's kinematic limits to ensure the most optimal task timing.

% % Several studies have used multiple demonstrations to smooth trajectories from kinesthetic demonstrations \cite{hu2022robot} \cite{paxton2015incremental} \cite{roveda2020assembly} \cite{tsai2020constrained} \cite{wu2021framework}. The study in \cite{shyam2019improving} used the demonstration as an initial guide for trajectory optimization, focusing on smoothness and jerk reduction but without strict task constraints. \cite{tsai2020constrained} used data from multiple demonstrations to determine task tolerances for their optimization. Aiming to improve implementation efficiency, \cite{muller2020one} employed a single demonstration with a fixed user-defined tolerance to generate a smooth trajectory. Our method advances beyond existing research by using just one demonstration and offering an intuitive interface for users to specify variability tolerance, rather than manually defining or statistically extracting from multiple demos.

% % Numerous methods like Low-pass Filters and Kalman Filters are used for noise filtering in trajectories, but they typically only address high-frequency noise and don't allow for the inclusion of variability tolerances or prevent excessive deviation from the original demonstration. \cite{chen2018playback} offers a detailed comparison of various smoothing algorithms and notes that while RBF-based learning methods like DMPs can naturally smooth demonstrations, they risk overfitting and noise replication without precise hyperparameter tuning. The study concludes that optimization-based smoothing is more effective in preserving demonstration features and improving information gain.

% Recent literature in LfD for collaborative robots has shifted from focusing on robustness against sub-optimal demonstrations \cite{cao2022learning} towards assessing the information gain and quality of demonstrations \cite{wu2021framework,kalinowska2021ergodic}. To do so, several studies have employed incremental learning to simplify the demonstration process, enabling humans to teach task components in phases. Authors in \cite{nemec2018efficient} let humans demonstrate path and timing separately, by allowing them to adjust the speed of their initial demonstration. The proposed framework in \cite{simonivc2021analysis} enables path and speed refinement through kinesthetic guidance, while the one in \cite{meszaros2022learning} uses teleoperated feedback for efficient task execution. Building on these, our approach incorporates the robot's kinematic limits into an optimization problem, solving for the best feasible timing law for the demonstrated path. Then, instead of merely speeding up, we permit users to ``slow down" demonstrations until reliable execution is achieved, and hence ensure the optimal timing.

% % In order to make the demonstration process more intuitive, natural, and effortless, several studies have used incremental learning to have the human teach different aspects of the task at different phases. In \cite{nemec2018efficient}, authors introduced a method for humans to demonstrate path and timing separately, by allowing them to adjust the speed of their initial demonstration. \cite{simonivc2021analysis} focused on allowing humans to refine both path and speed through kinesthetic guidance. Meanwhile, \cite{meszaros2022learning} employed teleoperated feedback for a grocery pick-and-place task to ensure faster and more reliable task execution. Building upon these works, we take the kinematic limits of the robot into an optimization problem and solve for the most optimal timing law for the provided demonstration path. Then, instead of speeding up, we allow the user to locally "slow down" the demonstration until reliable execution is ensured. In this way, we can guarantee that the most efficient timing law is adopted for the demonstration.

% Task variability tolerances are primarily used to adjust a robot's impedance, e.g., low impedance when there is high variability \cite{calinon2016tutorial}, but they are also pivotal for noise removal. Given that demonstrations do not have a set ground truth, distinguishing signals from noise is challenging. Using tolerances as trajectory guidelines ensures the trajectory is with the desired accuracy, preserving the demonstration's authenticity \cite{tsai2020constrained}. The study in \cite{chen2018playback} offers a detailed comparison of various smoothing algorithms, and the noise-removing effect of RBF-based methods like DMPs. However, without careful hyperparameter tuning, they risk overfitting and noise replication. The study concludes that optimization-based smoothing is more effective in preserving demonstration features and improving information gain. Within this context, some works have omitted tolerances \cite{shyam2019improving} or used fixed user-defined tolerances \cite{muller2020one}. However, our approach extracts these tolerances directly from human demonstrations and incorporates them into the optimization.

% To deduce tolerances from human demonstrations, it is common to consider the variance of multiple demonstrations, as an indicator of variability tolerance \cite{hu2022robot,roveda2020assembly,tsai2020constrained}. To enhance implementation efficiency, we propose a novel approach to discern tolerances from a single demonstration. Grounded in the psychological observation that humans naturally slow down when aiming for precision \cite{fitts1954information}, our method captures tolerances during periods where the demonstrator slows down. Although demonstrations are presented in joint space, we extract tolerances in the Cartesian space, emphasizing the end-effector pose as the task's crucial point.

% The simultaneous optimization of timing and jerk remains a challenge as it might lead to an infeasible problem. This stems from the fact that applying path constraints requires knowledge of the relative time when each part of the path is reached. On the other hand, such timings cannot be considered as decision variables, since the underlying trajectory representation is a piece-wise polynomial \cite{yang2018new}. Also, the original timing of the demonstration is not optimal. We address these challenges by solving the problem in two steps, where first the timing is optimized and then the jerk profile is regulated by removing the noise. To the best of our knowledge, the impact of optimizing the original demonstration on LfD performance has not been explored in previous research. Our study is the first attempt to showcase the performance of optimization-based smoothing as an additional layer (Fig. \ref{fig:intro}) with respect to the LfD output.
% % The notion of task variability tolerances has been employed in several works, mostly to locally adapt the impedance of the robot \cite{calinon2016tutorial}. But they can also be used to solve the challenge of noise removal from demonstrations. Eliminating trajectory noise requires a baseline signal or "truth." Since demonstrations lack a consistent ground truth, discerning signal from noise is challenging. It can be addressed by using tolerances as trajectory boundaries, ensuring that the trajectory does not deviate from the desired accuracy range, and hence maintaining the demonstration's integrity \cite{tsai2020constrained}. For example, authors in \cite{muller2020one} employed a fixed user-defined tolerance in their optimization problem to generate a smooth trajectory. In our work, task tolerances are extracted from human demonstration instead of being hand-designed.

% % To acquire the tolerances from humans, it is common to utilize the variance of multiple demonstrations as the notion of variability tolerance \cite{hu2022robot,paxton2015incremental,roveda2020assembly,tsai2020constrained,wu2021framework}. To enhance the implementation efficiency, we propose a novel way to obtain such tolerances through one single demonstration. In our work, we leverage the psychological fact that humans slow down when they want to be precise \cite{fitts1954information} and simultaneously extract tolerances during the stage where the human is slowing down the demonstration in our proposed framework. While the demonstration is in joint space, we extract the tolerances in the cartesian space, as the end-effector pose is the final important factor in the task.




==> Sections/related_work-draft2.tex <==
\section{Background and Related Work}
\label{sec:works}

% Execution Time
To address the issue of slow demonstrations and execution time, several studies focused on the isolation of demonstrating path and timing, allowing humans to teach the path and the timing law of demonstrations separately. Authors in \cite{nemec2018efficient} explore methods based on incremental learning to let human teacher adjust the speed of their initial demonstrations, integrating human feedback into velocity scaling factors within the DMP formulation. The work in \cite{simonivc2021analysis} further investigates the refinement of both path and speed through kinesthetic guidance, enabling teachers to fine-tune their demonstrations in real-time, thereby enhancing the quality of the learned trajectories. Moreover, the study of \cite{meszaros2022learning} utilizes teleoperated feedback to locally speed up the task execution. Their work clearly signifies the importance of a well-demonstrated timing law in achieving high task success rates. Building upon these works, our approach incorporates the robot's kinematic limits into an optimization problem, solving for the best feasible timing law for the demonstrated path. Then, we allow the human teacher to refine the new timing law in one pass. Instead of merely speeding up, we permit users to ``slow down" demonstrations to achieve reliable execution, and hence ensure the optimal timing. As opposed to other works, optimizing for the timing law provides guarantee that the best achievable execution time is calculated, while the ability to slow down the demonstration provides direct control to the human teacher in order to make the task execution reliable and successful while maintaining fast performance.

% Jerk
In the context of LfD, there are a limited number of works focusing on regulating the motion jerk. In \cite{wang2021optimised}, authors attempted to deal with jerky demonstrations by introducing a Gaussian noise.  In \cite{aleotti2006robust}, the smoothing nature of B-Splines was leveraged by fitting the demonstration trajectories via B-SPlines. A similar approach has been adopted by \cite{biagiotti2023robot} and \cite{shyam2019improving}. B-splines are a suitable choice for trajectory optimization due to their smoothness, local control, and efficient computation. Their piecewise polynomial nature ensures smooth motion paths, making them highly suitable for complex motion optimization \cite{de1972calculating}. However, the simultaneous optimization of timing and jerk poses a challenge as it might lead to an infeasible problem. This stems from the fact that applying path constraints requires knowledge of the relative time when each part of the path is reached. On the other hand, such timings cannot be considered as decision variables, since the underlying trajectory representation in B-Splines is a piece-wise polynomial \cite{yang2018new}. Also, the original timing of the demonstration is not optimal. We address these challenges by solving the problem in two steps, where first the timing is optimized and then the jerk profile is regulated by removing the noise.


When it comes to eliminating noise and unwanted behaviors/motions that naturally occur in human demonstrations, the focus of the existing studies is to turn suboptimal demonstrations into optimal demonstrations and enhance the learning and execution performance of LfD algorithms such as DMPs, GPs, GMMs, etc., which are directly affected through encoding and generalizing the demonstration data. suboptimal demonstrations can reduce the performance of LfD and cause overfitting or underfitting on the non-optimal demonstrations \cite{li2024learning}.
One approach is to focus on augmenting the demonstrations in order to fine-tune their data efficiency \cite{ma2022efficient, qian2020hierarchical}, which aims at compensating the suboptimal demonstrations via various methods such as data augmentation or self-exploration to improve the performance of learning. Another approach is to extract key information from demonstrations to capture the essential implicit features \cite{he2021imitation}. The work in \cite{wu2021framework} focused on assessing the effectiveness of the newly added demonstrations, a way of quantifying how informative are the demonstrations in order to enhance the efficiency of data in the demonstration process. In the work in \cite{el2021itp},  the LfD outcome is optimized via RL by eliminating suboptimal demonstrations from the demonstration data, and keeping the more useful demonstrations. 
The authors in \cite{ye2022bagging} utilized GMM to increase the robustness of LfD to suboptimal training data, and ensure that the reproduced trajectory maintains the required precision.

However, the common point in the mentioned works is that they used multiple demonstrations to optimize the demonstration process. This choice is motivated by the fact that human demonstrations do not have a set ground truth, which is a necessary requirement to distinguish between accurate demonstration data and noise or unwanted motion.The research question is how to develop a metric of accuracy to bind the demonstrations to and act as ground truth, while providing some level of freedom to modify or optimize the demonstration trajectories.
Studies such as \cite{tsai2020constrained} and \cite{calinon2016tutorial} emphasize using task variability tolerances to adjust a robot's compliance, with low impedance settings employed when high variability is measured, thereby allowing for more deviations in human demonstrations. The main idea is to align multiple demonstrations of a task and use the variance of each segment of demonstration as a measure of significance or required accuracy. For example, the part of the motion that was highly similar in all demonstrations indicates that an accurate behavior is expected to be performed, while the part where motion is variant among the demonstration shows that the motion can deviate more while maintaining the accuracy of the task.
In several works, authors have leveraged the statistical distribution of multiple demonstration trajectories and used the variance to extract tolerance values to represent accuracy \cite{hu2022robot,paxton2015incremental,roveda2020assembly,wu2021framework}. Additionally, in \cite{delson1994robot}, tolerance bounds are extracted from multiple demonstrations to serve as an obstacle-free region. In this way, the optimization approach has some degree of flexibility to regress a noise-free trajectory, while being confined to the tolerance bounds, ensuring that the demonstration remains accurate, obstacle-free, and successful at achieving the goal of the task. In \cite{maeda2008easy}, the human first is required to move the manipulator around the free space of the working environment. Next, the swept volume is used as tolerance bounds to constrain the optimization method in order to successfully optimize based on the desired objective.

The aim of all of these studies is to develop a tolerance bound as a numerical representation of accuracy, so that they can safely constrain the optimization method and apply their desired objective to optimize the demonstrations. However, since all of the mentioned works rely on multiple demonstrations, they sacrifice the clear advantages of one-shot demonstration. There are only a limited number of works that have attempted to address this challenge via one-shot demonstration. In \cite{muller2020one}, the authors have used the points recorded from the demonstration to fit a piece-wise polynomial trajectory, within a predefined and fixed tolerance bound. Building upon this, authors in \cite{biagiotti2023robot} proposed a novel approach to adaptively extract tolerance bounds via one-shot kinesthetic demonstration. They proposed a demonstration approach based on surface Electromyography (sEMG) signals. Throughout kinesthetic demonstration, the stiffness of the hand of the human teacher is recorded through sEMG measurements and serves as a measure of accuracy level, i.e. tolerance bounds. However, the proposed method requires an expensive setup which increases the cost and efforts of implementation. 

In this work, we propose a novel approach to the acquisition of tolerance values, without the need for an expensive extension of demonstration setup. Grounded in the psychological observation that humans naturally slow down when aiming for precision \cite{fitts1954information}, our method captures tolerance bounds during the refinement phase when the human teacher slows down the timing law of the demonstration. The tolerance acquisition logic is that when the human teacher slows down a segment of the demonstration, it implies that the particular section is more critical and has to be more accurate. For example, in a task involving picking and inserting a peg, while the picking and moving part can be performed fast, the insertion part should be performed slower. This is because this part of the motion requires a higher accuracy to ensure success. During the refinement phase, the human teacher not only has the opportunity to locally slow down the optimized demonstration trajectory, but they simultaneously imply the tolerance bounds required by the task at each part of the demonstration. In our work, although demonstrations are represented in the joint space, we extract tolerance bounds in the Cartesian space, due to the fact that the end-effector pose is the task's ultimate point of accuracy.

Overall, and to the best of our knowledge, the impact of optimizing the original demonstration on LfD performance has not been explored in previous research. Our study is the first attempt to showcase the performance of optimization-based smoothing as an additional layer with respect to the LfD output. Moreover, it is noteworthy to mention that our approach works with one-shot demonstration, with an additional one-shot refinement. This makes the whole approach one-shot since all the teachings from the human teacher is provided in one pass only.


==> Sections/shortcuts.tex <==
% Shortcuts
\newcommand{\hide}[1]{}
\newcommand{\Figure}{Fig.~}
\newcommand{\Equation}{Eq.~}
% \newcommand{\ie}{\emph{ie.~}}
% \newcommand{\eg}{\emph{eg.~}}
\newcommand{\cf}{\emph{cf.~}}
\newcommand{\bdmath}{\begin{dmath}}
\newcommand{\edmath}{\end{dmath}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bdm}{\begin{displaymath}}
\newcommand{\edm}{\end{displaymath}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\beal}{\beq \begin{array}{ll}}
\newcommand{\eeal}{\end{array} \eeq}
\newcommand{\beas}{\begin{eqnarray*}}
\newcommand{\eeas}{\end{eqnarray*}}
\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}

% Groups, Domains, Sets
\newcommand{\SO}{\mathrm{SO}}
\newcommand{\so}{\mathfrak{so}}
\newcommand{\SE}{\mathrm{SE}}
\newcommand{\se}{\mathfrak{se}}
\newcommand{\Real}{\mathbb{R}}
\newcommand{\Int}{\mathbb{Z}}
\newcommand{\ImageDomain}{\Omega}
\newcommand{\Surface}{\mathcal{S}}
\newcommand{\SEtwo}{\ensuremath{\mathrm{SE}(2)}\xspace}
\newcommand{\SEthree}{\ensuremath{\mathrm{SE}(3)}\xspace}
\newcommand{\SOtwo}{\ensuremath{\mathrm{SO}(2)}\xspace}
\newcommand{\RPE}{\ensuremath{\mathrm{RPE}}\xspace}
\newcommand{\ATE}{\ensuremath{\mathrm{ATE}}\xspace}
\newcommand{\RMSE}{\ensuremath{\mathrm{RMSE}}\xspace}
\newcommand{\Ed}{\ensuremath{\mathrm{E}}\xspace}
\newcommand{\SOthree}{\ensuremath{\SO(3)}\xspace}
\newcommand{\sothree}{\ensuremath{\so(3)}\xspace}
\newcommand{\setdef}[2]{ \{#1 \; {:} \; #2 \} }

% Calligraphic fonts
\newcommand{\calA}{{\cal A}}
\newcommand{\calB}{{\cal B}}
\newcommand{\calC}{{\cal C}}
\newcommand{\calD}{{\cal D}}
\newcommand{\calE}{{\cal E}}
\newcommand{\calF}{{\cal F}}
\newcommand{\calG}{{\cal G}}
\newcommand{\calH}{{\cal H}}
\newcommand{\calI}{{\cal I}}
\newcommand{\calJ}{{\cal J}}
\newcommand{\calK}{{\cal K}}
\newcommand{\calL}{{\cal L}}
\newcommand{\calM}{{\cal M}}
\newcommand{\calN}{{\cal N}}
\newcommand{\calO}{{\cal O}}
\newcommand{\calP}{{\cal P}}
\newcommand{\calQ}{{\cal Q}}
\newcommand{\calR}{{\cal R}}
\newcommand{\calS}{{\cal S}}
\newcommand{\calT}{{\cal T}}
\newcommand{\calU}{{\cal U}}
\newcommand{\calV}{{\cal V}}
\newcommand{\calW}{{\cal W}}
\newcommand{\calX}{{\cal X}}
\newcommand{\calZ}{{\cal Z}}

% Image
\newcommand{\Image}{\mathtt{I}}
\newcommand{\Depth}{\mathtt{D}}
\newcommand{\bearingvec}{\mathbf{f}}
\newcommand{\px}{\mathbf{u}} % Pixel
\newcommand{\pt}{\mathbf{p}} % 3D point
\newcommand{\depth}{d}
\newcommand{\proj}{\pi}

% Transformation
\newcommand{\T}{\mathtt{T}}
\newcommand{\R}{\mathtt{R}}
\renewcommand{\S}{\mathtt{S}}
\newcommand{\Identity}{\mathbf{I}}
% \newcommand{\inv}{^{-1}}

% Matrices
\newcommand{\trace}[1]{\mathrm{tr}\left(#1\right)}

% Other
\newcommand{\residual}{\mathbf{r}}
\newcommand{\trnsp}{\mathsf{T}}
\newcommand{\Zero}{\mathbf{0}}
% \newcommand{\eye}{{\mathbf I}}
\renewcommand{\skew}{{\mathbf S}}
\newcommand{\Jac}{\mathtt{J}}
\newcommand{\Zthree}{\Zero_{3 \times 3}}
\newcommand{\Ithree}{\eye_{3 \times 3}}

% Imu
\newcommand{\rotvel}{\boldsymbol\omega}
\newcommand{\acc}{\mathbf{a}}
\newcommand{\rotvec}{\boldsymbol\phi}
\newcommand{\rotvecpert}{\delta\rotvec}
\newcommand{\rotvecang}{\varphi}	% rotation vector angle
\newcommand{\rotvecdir}{\mathbf{a}} % rotation vector direction
\newcommand{\tran}{\mathbf{p}}
\newcommand{\tranpert}{\delta\tran}
\newcommand{\vel}{\mathbf{v}}
\newcommand{\velpert}{\delta\vel}
\newcommand{\bias}{\mathbf{b}}
\newcommand{\biaspert}{\delta\bias}
\newcommand{\gravity}{\mathbf{g}}
\newcommand{\noise}{\boldsymbol\eta}
\newcommand{\VIO}{VIO\xspace}
\newcommand{\odometry}{navigation\xspace}
\newcommand{\tango}{{\rm Tango}\xspace}

%Kalman Filter
\newcommand{\F}{\mathbf{F}}
\newcommand{\G}{\mathbf{G}}
\newcommand{\Pcov}{\mathbf{P}}
\newcommand{\Kgain}{\mathbf{K}}




% Paper Specific
\newcommand{\hl}[1]{ {\color{red} #1} }
\newcommand{\cut}[1]{\hl{cut? $\rightarrow$ #1}}
\newcommand{\Cov}{\mathbf{\Sigma}}
\newcommand{\at}[1]{^{(#1)}}
\newcommand{\expmap}{\mathrm{Exp}}
\newcommand{\logmap}{\mathrm{Log}}
\newcommand{\normsq}[2]{\left\|#1\right\|^2_{#2}}
\renewcommand{\d}{\text{d}}
\newcommand{\Rmean}{\R}
\newcommand{\Rrand}{\tilde\R}
\newcommand{\eq}{Eq.}
\newcommand{\eqs}{Eqs.}

\newcommand{\iSAMtwo}{iSAM2\xspace}
% \newcommand{\MAP}{MAP\xspace}
% \newcommand{\SVO}{SVO\xspace}
% \newcommand{\GN}{GN\xspace}
% \newcommand{\BS}{BS\xspace}
\newcommand{\States}{\mathcal{X}}
% \newcommand{\meascam}{\mathcal{C}}
% \newcommand{\measimu}{\mathcal{I}}
% \newcommand{\cov}{\mathbf{\Sigma}}
\newcommand{\covprior}{\mathbf{\Sigma}}
% \newcommand{\covimu}{\mathbf{\Sigma}}
% \newcommand{\covcam}{\mathbf{\Sigma}_{\meascam}}
\newcommand{\World}{\text{W}}
\newcommand{\Imu}{\text{B}}
% \newcommand{\Camera}{\text{C}}
\newcommand{\world}{\text{\tiny{W}}}
\newcommand{\imu}{\text{\tiny{B}}}
\newcommand{\camera}{\text{\tiny{C}}}
\newcommand{\cam}{{\scriptsize \text{c}}}
% \newcommand{\accshort}{\tilde\acc(t)\!-\! \bias^a(t) \!-\! \noise^{ad}(t)}
\newcommand{\preintVar}{increments\xspace} 
\newcommand{\biasFixedPreintVar}{bias-fixed increments\xspace} 
% \newcommand{\biasFixed}{\bar{\bias}}
% \newcommand{\biasFixedDelta}{\Delta}
% \newcommand{\biasHat}{\hat{\bias}}
% \newcommand{\meters}{\rm{m}}
\newcommand{\preintRmeas}{\Delta\bar\R}
\newcommand{\preintVmeas}{\Delta\bar\vel}
\newcommand{\preintPmeas}{\Delta\bar\tran}

% % smart factors
% \newcommand{\pixel}{\mathbf{z}}
% \newcommand{\pixelnoise}{\noise_{cam}}
% \newcommand{\landmark}{\mathbf{\rho}}
% \newcommand{\landpert}{\delta\landmark}
% \newcommand{\posepert}{\delta\mathbf{X}}
% \newcommand{\bvec}{\mathbf{b}}
% \newcommand{\Amat}{\mathbf{A}}
% \newcommand{\Bmat}{\mathbf{B}}
% \newcommand{\Fmat}{\mathbf{F}}
% \newcommand{\Emat}{\mathbf{E}}
% \newcommand{\Qmat}{\mathbf{Q}}
% %
% \newcommand{\appendixRef}{Appendix\xspace}
% \newcommand{\subimu}{{ij}} 
% \newcommand{\indmeas}{(i,j)} 


% % Jacobians
% \newcommand{\DLog}{\mathtt{J}_{r}^{-1}} 
% \newcommand{\DExp}{\mathtt{J}_{r}} 
% \newcommand{\DExpk}{\mathtt{J}^k_{r}} 
% \newcommand{\jacobian}[2]{\frac{\partial #1}{\partial #2}}

% % updates
% \newcommand{\rup}{\rotvecpert} 
% \newcommand{\tup}{\tranpert} 
% \newcommand{\vup}{\velpert} 
% \newcommand{\bupa}{\tilde\delta{\bias^a_i}} 
% \newcommand{\bupg}{\tilde\delta{\bias^g_i}}

%% Preintegrated measurements
% \newcommand{\pRot}{\Delta\bar\R_{ij} } % integration value
% \newcommand{\pRotk}{\Delta\bar\R_{ik} } % integration value
% \newcommand{\pTran}{\Delta\bar\tran_{ij}}
% \newcommand{\pVel}{\Delta\bar\vel_{ij}}
% \newcommand{\pVelk}{\Delta\bar\vel_{ik}}
% \newcommand{\mRot}{\Delta\tilde\R_{ij}} % measured
% \newcommand{\mTran}{\Delta\tilde\tran_{ij}}
% \newcommand{\mVel}{\Delta\tilde\vel_{ij}}
% \newcommand{\Adjoint}{\mathtt{Ad}}

% \newcommand{\biasCorrectedGyroMeas}{\tilde\rotvel(t) \!-\! \bias^g(t)}
% \newcommand{\biasCorrectedAccMeas}{\tilde\acc(t) \!-\! \bias^a(t)}
% \newcommand{\Rmeas}{\tilde\R}
% \newcommand{\vmeas}{\tilde\vel}
% \newcommand{\tmeas}{\tilde\tran}

\newcommand{\toa}{ToA\xspace}
\newcommand{\aoa}{AoA\xspace}
\newcommand{\aod}{AoD\xspace}
\newcommand{\quadriga}{QuaDRiGa\xspace}


==> Sections/temp/introduction-temp.tex <==

\gpt{The manufacturing industry has witnessed a remarkable transformation due to the advent of robot manipulation. With its ability to perform precise and repetitive tasks, robots have become indispensable in modern manufacturing processes. Evaluating the performance of industrial robotic tasks revolves around three essential metrics: time, accuracy, and energy efficiency. Time refers to the speed and efficiency with which a robot completes a task, directly influencing production rates. Accuracy measures the precision and consistency of a robot's movements and actions, ensuring the quality and reliability of the manufactured products. Lastly, energy efficiency evaluates the robotic system's ability to optimize power consumption, reducing operational costs and environmental impact.}

\gpt{In the current manufacturing landscape, there has been a noticeable shift from mass production to mass customization, compelling companies to swiftly respond to market demands while maintaining economic feasibility.} As a result, robotized plants need to tune into a small-bath production scheme, where frequent reconfiguration and reprogramming becomes a recurring and essential process. However, traditional programming methods present challenges, including prolonged programming time and the necessity of having an on-site robot expert, which incurs significant effort, production off time, and financial resources.



\textbf{Why robot manipulation for the industry?}

  - Save costs in the long-term by replacing human labor
  - Increase production capacity as robots can work 24/7
  - Ergonomics and safety of humans
  - better consistency and quality as the robots excel at repetitive tasks and don't make mistakes

The introduction of robots, and especially robotic manipulator, has pushed the industry to another level in terms of performance efficiency, production quality and consistency, flexibility and adaptability, production capacity, as well as saving costs in the long-term, particularly labor costs! [find a ref]

\textbf{What are the challenges of integrating robots into the industry?}

  - \bl{Despite recent changes in the manufacturing paradigm, robots are still predominantly used in large-scale and large batch production manufacturing plants such as the automotive and electronics industry} 
  - In a large-batch production setting, the robot task is fixed to one task and is supposed to repeat that. In this case, a robot expert needs teach the task to the robot by putting effort into the modeling and programming in a traditional way. In such scenarios, the robot's environment is static and structured.
  - On the contrary, as modern industries are moving towards a more customized production scheme, the concept of mass customization is replacing mass production [find ref]
  - \bl{The global competitive arena forces companies to react quickly to the demands of the market while maintaining economic feasibility. Consequently, the robotized production plants should adapt to handle a wide variety of products by frequent reconfiguration of both hardware sub-components and robot programs} 
  - In this new paradigm, robot learning becomes a frequent process, as the robot task is no longer static and is required to change over the course of production.



\textbf{How can the robot learn the industrial task?}
There are three different approaches to robot learning

  - \bl{Traditional robot programming requires profound knowledge in computer science and understanding issues arising from robot kinematics and dynamics} 
  - Motion Planning / RL. This approach requires a great amount of modeling, i.e. modeling robot environment, task model, etc. Therefore, it requires a robot expert to be on-site for implementation and modification.
  - Learning From Demonstration (LFD). LFD is the approach that enables humans to teach robot in a similar manner they teach each other, by demonstrating the task. The robot learns not only the movements demonstrated by the teacher, but the concept of motion, which makes it possible to generalize to new situations. Learning from demonstration doesn't require a robotic expert to model the problem, but it enables the non-experts in robotics to interact and collaborate with the robot.

\bl{Nowadays, robots are still dominating in large-scale automotive and electronic industries, characterized by largevolume, large-batches productions. One of the issues of contemporary robotics is the introduction of flexible and collaborative robots in craft and small-scale SME production. These production plants are characterized by a wide variety of different assembly tasks, where it is essential to shorten the programming time and to reduce the required skill level of the operators } \cite{nemec2019incremental}

\bl{The efficiency of the human–robot collaboration system has a direct and significant impact on the assembly task quality. However, most of the collaborative robots in manufacturing are traditionally programmed and controlled by some offline coding devices such as teaching pendants and workstations. Afterward, the robot collaborates with its human partner via the predefined workflows to perform repetitive tasks. The human–robot collaboration system will become confused and even shut down if the task is changed. It will cost a lot of human efforts and time to recode the corresponding new task, which decreases the collaboration efficiency and task quality. Modern manufacturing is seeing quick product updates with shorter life cycles and more customizations to meet the market needs.}

\bl{Traditional robot programming is often not feasible in small-batch production, as it is time-consuming, inefficient, and expensive.} 

\bl{Another issue is to shorten the robot programming time and reduce the required skill level of the operators} 

\bl{Learning from Demonstration (LfD), often referred to as Imitation Learning, is a promising and powerful technology that can among others solve the issues mentioned above 

\bl{Within this framework, the robot tasks are demonstrated naturally rather than coding in a robot-oriented programming language or using expensive and complex robot simulation systems. It is important to emphasize that LfD concept goes beyond the simple showing and copying of a policy performed by a demonstrator. It includes many aspects such as generalization of the robot policy to different contexts, the ability to adapt to changes in the environment, or refinement of the captured policy} 

\textbf{What are the challenges of LFD in industry?}

The performance of robot manipulation in industry is essentially measured via the following metrics:

  - Time. The most important factor in industrial and production settings is the factor of time. the less cycle time for each cycle of robot manipulation (e.g. for assembling a product) the more output at the end of the day (e.g. more products assembled). However, it is necessary to maintain the quality of the process as well as minimizing the number of errors while increasing the speed of task execution and hence reducing the cycle time.
  - Accuracy. depending on the scale of the manipulation objects, accuracy would play an important role in the successful execution of the task and avoid faulty cycles.
  - Energy Consumption. In order to move towards a more economic and efficient production, it is beneficial to consider finding the most optimal way of performing a task in order to consume the least energy and also improve the lifespan of the machinery (structural load). In kinematic terms, the value of the Jerk of a trajectory is the key indicator to quantify this metric.


In this regard, it is crucial to ensure the mentioned metrics are taken into consideration through the learning loop.

Another challenging aspect of LFD is the interface through which humans interact with the robot and teach the task (Demonstration). Kinesthetic teaching is shown to be one of the most intuitive ways of demonstration [find ref]. However, the demonstration contains noise, due to jerky/shaky human movements and unwanted vibrations. The presence of noise in the demonstration hinders the core algorithm to learn the essential aspects of the task and the learning resources are wasted on fitting to the noisy parts. Moreover, the means of providing the demonstration directly impact the quality of the demonstration and the amount of pure information it contains about the task.




What is important in the case of industrial robot manipulation?

Why Learning from demonstration instead of traditional programming?

What are the benefits, requirements, and challenges of LFD?

How to make demonstration in LFD easier and more intuitive? and why is



==> Sections/temp/introduction-temp2.tex <==
\section{Introduction}
\label{sec:intro}

In recent years, the manufacturing industry has experienced a paradigm shift from mass production to mass customization. This transformation necessitates a small-batch production scheme, challenging robotized production lines to frequently reconfigure and reprogram robotic tasks based on market demand \cite{cohen2019assembly} \cite{pedersen2016robot} \cite{qu2019smart}. The performance of these  tasks is evaluated primarily based on three critical metrics: time, accuracy, and energy efficiency, which directly affect the production rate, product reliability, and operational costs, respectively.

Within this new paradigm, traditional programming methods present several drawbacks. These include the necessity of an on-site robot expert, prolonged programming time, and a significant investment of resources, which in turn increase production downtime and financial costs \cite{sloth2020towards} \cite{dean2016robotic}. In contrast, Learning from Demonstration (LfD) \cite{ravichandar2020recent} offers a promising alternative to resolve these issues in small-batch productions with frequent task changes. \bl{The choice of LfD over other robot learning methods is compelling when ideal behavior can neither be easily scripted, as done in traditional robot programming, nor be easily defined as an optimization problem, but can be demonstrated.} \cite{ravichandar2020recent}. It enables robots to learn tasks through human demonstrations \cite{pastor2011skill}. However, in existing LfD approaches, the quality of the demonstration presents significant challenges to learning efficiency, often failing to meet the essential metrics of time, accuracy, and energy.



Human-provided demonstrations typically manifest at slower speeds, as demonstrating at high speed is challenging for the human teacher and even unsafe. A uniform speed-up to the entire movement is also suboptimal as different phases of a task may require varying speeds. Additionally, the noise prevalent in the demonstrations, when sped up, can result in extreme jerks or non-ideal trajectories. The inherent noise is intertwined with the path information, in which the required accuracy for a given task is encapsulated. It is nontrivial to effectively filter this noise while preserving accuracy, primarily due to the non-uniform accuracy requirements across different sections of the task. For instance, the accuracy at the beginning and the end of a Pick and Place task is higher than other parts. While the profile of required accuracy should ideally be provided by the human demonstrator, many LfD approaches fail to incorporate this crucial information directly, leading to suboptimal assumptions that may trade off accuracy for time. 

\bl{However, to fully capture a demonstrator’s motion characteristics, an approximator (like DMP, etc.) would have to rely heavily on multiple critical demonstrations, which in practice, are hard to obtain.} \cite{tsai2020constrained}

\bl{Therefore, a sufficient number of demonstrations is needed, from which the important features can be extracted e.g. via Gaussian Mixture Models. In ...,  demonstrated trajectories are encoded with Hidden Markov Models and obtained by a spline interpolation through key points, which are identified by significant changes in position and velocity. In ..., the focus lies on clustering, selecting and approximating a set of demonstrated, often noisy, trajectories. Though this method yields impressive robotics results, demonstrating the same task over and over again is inefficient and impractical for industrial applications.,}\cite{muller2020one}

[The quality and the outcome of the learning are highly affected by a poor demonstration \cite{wu2021framework}. In \cite{wu2021framework} authors have looked into how to eveluate and measure the quality of demonstrations. They have highlighted how existing LfD approaches mainly focus on the learning part of LfD and rarely paid attention to the quality of demonstration]

[Approaches that require multiple demonstrations such as GMM/GMR, ProMP, GP, etc. have two main drawbacks: 1)task information is passed indirectly and spread through several demonstrations 2) it is complicated to modulate the trajectories in order to alter the timing or optimizing for objectives and constraints (?!)]

[In \cite{muller2020one}, They have proposed a trajectory generation approach, where the resulting trajectory will not deviate more than a user-defined threshold from the original demonstrated path. However, they have not incorporated time, and the customized tolerance, as the threshold is defined explicitly by the user.]

[In \cite{tsai2020constrained} authors have leveraged the statistical distribution of multiple human demonstrations to extract tolerance values (safety margin) for optimization, i.e. Low variance demands high precision and vice versa. The optimization problem is tackled through RL to improve learning efficiency, i.e. complete the task minimum \textbf{path length} and without collision while satisfying trajectory smoothness]

[In \cite{shyam2019improving}, Kinesthetic-based human demonstrations have been used to form the initial guess for the trajectory planning problem, in order to avoid falling into local optima while solving for smoothness and minimum jerk. The trajectory planning problem is also targeted for obstacle avoidance.]

[In \cite{cao2021learning}, authors considered the problem of learning from suboptimal demonstration. They have proposed a scoring function that measures how informative a demonstration is. In their work, they have again focused on the robustness of the learning algorithm instead of increasing the information gain of the demonstrations]

[In \cite{cao2022learning} they continued the work from \cite{cao2021learning} to develop a confidence-based demonstration ranking. Both works focus on the robustness of the learning algorithm by assuming there is sub-optimality among the demonstrations. ]

\bl{Due to the complexity of the task, these demonstrations are often slow and even slightly flawed, particularly at moments when multiple aspects (i.e., end-effector movement, orientation, and gripper width) have to be demonstrated at once.}\cite{meszaros2022learning}

[In \cite{meszaros2022learning}, authors have proposed a demonstration + correction approach that reduces the effort of demonstrating all the aspects of the task at once and enables non-expert users to enhance their initial demonstration through teleoperated feedback. Their motivation was to reduce the execution time while ensuring the reliability of execution (e.g. picking a bottle fast enough not to topple it over)]

[In \cite{montero2022solving}, similar incremental learning as \cite{meszaros2022learning} is used to reshape the trajectory in order to satisfy precision requirements while speeding up the original demonstration]

[In \cite{simonivc2021analysis} they have for the first time considered the separate refinement of path and velocity]

[In \cite{nemec2018efficient}, they have used incremental learning to refine the robot’s path and velocity. The final refinement step is the velocity correction where human demonstration leads to a velocity scaling factor, in this way, they have contributed to the time optimality of the learning --> but they have nowhere considered the kinematic limits of the robot and if the achieved velocity is the maximum limit of the robot!]

[It is noteworthy to mention that human demonstration encodes some implicit constraints required for the task, which are not directly included in the optimization problem. However, by constraining the path to adhere to the demonstration, we can assume that those constraints are also taken into consideration]

[In \cite{kalinowska2021ergodic} authors have focused on the learning algorithm to cope with suboptimal demonstration (instead of focusing on demonstration quality). They have leveraged negative demonstration to teach the robot what not to do. In this work, the demonstrations are used to formulate an objective for MPC function, which is in some aspect similar to what we do. However, we use the demonstration to formulate the constraints of an optimization problem, which in turn allows us to define our objective with respect to the task's key performance metrics. This approach is capable of converting a suboptimal demonstration into an optimal one while ensuring that the required constraints are not violated]

[In order to remove noise from demonstration, one common approach is to record multiple demonstrations and use GMM/GMR to approximate and generate a smooth trajectory \cite{hu2022robot} \cite{paxton2015incremental} \cite{roveda2020assembly} \cite{tsai2020constrained} \cite{wu2021framework}]

[In \cite{chen2018playback}, they targeted the noises and jumps from hand trembling and sensor noises that appear in the demonstration. When replaying the demonstration trajectory, these noises cause vibrations and shocks and could be damaging the robot, especially if sped up! In order to smooth a trajectory, several approaches based on low-pass filters exist \cite{bearee2013dissociated} \cite{jin2014improving} \cite{biagiotti2013online}. However, they can only eliminate high-frequency noises, while the jumps caused by hand trembling would remain \cite{chen2018playback}. The other approach is to filter noise through multiple trajectory samples and use GP or GMM, which is inefficient in terms of demonstration workload and how the information is conveyed through multiple demonstrations. 
The RBF-based learning process of DMPs and ProMPs can naturally smoothen the demonstration, but without careful tuning of the hyperparameters for each demonstration, the model can overfit easily and replicate the noise \cite{chen2018playback} (the reference is not very good, should I find a better one? also should I look more for similar works that are not really LfD for my literature review?)
Finally, this work uses CHOMP in order to find the optimized trajectory, but it does not solve for time optimization (or even jerk I guess). But they compare the smoothing performance of their optimization-based smoothing with respect to Kalman Filter, RBFNN, and Sliding average. They have mentioned the drawback of each approach and proved that the optimization-based approach is the best in terms of retaining the main features of the demonstrations.]

[In \cite{hu2022robot}, in order to capture the skillful aspects of the task, the authors divided it into phases to deal with the variability of multiple demonstrations. again here, multiple demonstrations poses challenges to directly convey the precision information required.]

[The positive effects induced by a jerk minimization are: errors during trajectory tracking are reduced. 
stresses to the actuators and to the structure of the manipulator are reduced.  excitation of resonance frequencies of the robot is limited. a very coordinated and natural robot motion is yielded. \cite{piazzi2000global} \cite{gasparetto2007new}]

Finally, using the jerk profile of a trajectory as a metric for energy consumption reveals that noisy demonstrations often result in high-jerk spikes. 
Although learning algorithms can act as filters to smooth out these spikes, it comes at the expense of learning efficiency. This is because the noise inhibits the algorithms' capacity to distill the fundamental features of the demonstration, and some trajectory irregularities may nonetheless endure. Notably, there exists an inherent trade-off between minimizing jerk and maintaining close adherence to the original demonstration path. Achieving the right balance is a nontrivial task that current LfD approaches struggle to tackle.

[The effect of noise can be more severe when performing LfD on joint space compared to end-effector space, as the noise on joint values can translate to high end-effector variations depending on the configuration. The choice of joint state over end effector state for industrial tasks is due to advantages in kinematic redundancy management, singularities avoidance, and correspondence problem \cite{fabisch2020comparison} Moreover, efficiency is increased by eliminating the need for inverse kinematics as well as complex encodings of end effector orientation which can lead to more errors]
\bl{for the final trajectory generation this implies the solution of the inverse kinematics problem which is in the case of redundant manipulators difficult to solve due to joint constraints and the infinite solution possibilities \cite{chiaverini2016redundant}}\cite{muller2020one}

% Good one
[In our approach, instead of focusing on how the learning algorithm can benefit the most from demonstration (especially the suboptimal ones) to become robust, we focus on how much information about the target task is encoded in the demonstration (e.g. how time optimality and precision can be best encoded in a demonstration to be directly leverageable by the learning algorithm. The nature of this information highly depends on the targetted task. Here, we focus on maximizing information gain for an industrial task]

[In our work, the notion of efficiency is associated with minimizing task execution time along with energy consumption (jerk), constrained to adhering to the human-provided demonstration feedback (precision), while satisfying trajectory smoothness]

[The demonstration suboptimality stems from two main sources, 1) the noise inherent in human demonstration which obscures the original underlying information. 2) How the task-related information is encoded in the demonstration and how the learning algorithm can leverage it]
% Good one
[The significance of our approach is that it attempts to reduce the implementation time/effort by eliminating the need to have multiple demonstrations/corrections. Instead of using multiple demonstrations and indirectly extracting information (e.g. via statistics). we attempt to provide the user with a hierarchical demonstration procedure, where the task is learned one feature at a time. With this approach, the information gain is concentrated in one single demonstration (at each stage of the hierarchy), instead of being spread across different demos.]

[inspired by incremental learning, we incrementally allow the human demonstrator to provide different aspects of the task, while keeping the learning phases isolated. Moreover, as opposed to other works, we initially optimize for the best key performance parameters, before user modification (find the best timing law and allow the user to slow it down until reaching reliable execution).]

[incremental learning can refer to learning different aspects of the motion incrementally. In this framework, the path is initially demonstrated, isolated from other aspects of the task. Then, the optimization framework finds the optimal demonstration trajectory with respect to the time and jerk, with a default precision profile. Then, the user can adjust the velocity profile of the demonstration trajectory, which at the same time, will be taken into account as the precision profile.So the learning incrementally completes in three step: path, time, precision, energy!]


Motivated by the above-mentioned considerations, in this paper, we introduce a novel approach to enhance the quality of demonstration in an LfD pipeline: an optimization-based smoothing algorithm that refines noisy demonstrations in terms of time, accuracy, and energy efficiency. By adjusting the demonstration path within user-specified tolerances, our method achieves minimal cycle time and jerk, while preserving task-specific accuracy requirements through an innovative velocity correction procedure. The main contributions of the paper are as follows:

\begin{itemize}
    \item A new smoothing approach is proposed to mitigate the noise in demonstrations while optimizing for key performance metrics.
    \item An intuitive velocity feedback procedure is introduced to let human demonstrators provide meaningful velocity inputs. This leverages the inverse relationship between speed and accuracy.
    \item A novel method for associating velocities and tolerances is incorporated within the smoothing algorithm, to make a trade-off between accuracy and time.
\end{itemize}



[In this work, we discuss how jerk as a metric is also directly associated with the efficiency of learning as well. We take Dynamic Movement Primitives (DMPs) as our learning approach and showcase how DMP's learning efficiency is improved via a smooth demonstration trajectory compared to its original form.

minimum jerk is associated with better joint position tracking (accuracy).

% General

The original demonstration implicitly encodes some constraints required for the reliable execution of the task (e.g. the structure around the robot, where demonstration makes sure that robot won't hit itself (self-collision) as well as the environment.) by constraining the path to adhere to the demonstration, we can assume that those constraints are also taken into consideration
]

[% Time
demonstration time is slow because usually humans need to demonstrate different aspects of the task at the same time, e.g. robot configuration, end effector position, gripper, etc., which makes it cognitively challenging.
A uniform speed-up is not ideal because 1) various velocity profiles across the demonstration, and high velocities at some sections of the task lead to unreliable task execution (for example, peg in hole!) 2) There are noises and jumps in the demonstrations due to hand trembling and sensor noises. Speeding up will amplify these noises which leads to infeasible trajectories.

% Accuracy
Accuracy is the underlying factor for the reliability of a task. The accuracy of the task is encoded in two aspects 1) The accuracy of the path which the robot needs to follow and 2) The allowed variability at each segment of that path, i.e. how much deviation is allowed for the robot in order to still reliably accomplish the task. For example, in a Pick and Place task, the motion has to be accurate at the picking and the placing segment of the task, but can be more variable (lenient) in the rest of the motion without violating task reliability. [related works: GMMs to capture the variability instead]
demonstrating the task multiple times is inefficient and impractical
delivering the variability information indirectly through multiple demonstrations is informationally inefficient, while leaving the user with less control over what they are teaching (e.g. for a high-precision manufacturing task, user needs to repeat the high-precision part of the task, while teaching variability in other parts, while robot might also capture some unwanted variability in the accurate part. Moreover, There appears the problem of matching different demonstrations and extracting the variabilty will become dependent on the quality of matching.
while multiple demonstration makes it easier to generalize, it is inefficient in terms of information delivery as well as teaching time and effort]

==> Sections/temp/introduction-temp3.tex <==
\section{Introduction}
\label{sec:intro}
[First figure: the robot actual picture, a noisy path in red, and a smooth path in green. showing that the noise is removed]
[traditional programming is where robot is hand-coded (most common in industry now). One level more advanced is opt-based planning, which requires defining constraints: path constraints e.g. how to approach, how to pick, how to insert; as well as timing constraints: where should be slow, where can be fast. For some complicated tasks, it is not easy to formulate in this way, so LFD comes to save us.
Demonstration in LFD can be seen as an implicit way of representing such constraints. an optimal information-rich demonstration can be measured by how well it encodes the task constraints in order for any LfD algorithm to learn and generalize them. Although such optimality is at its cores similar for all robotic tasks, there are certain preferences based on the context on which LFD is applied. Here in this work, our focus is the application of LFD in manufacturing tasks. In this context, robot tasks are expected to be reliable and cost-efficient. reliability comes from the fact that ]

[In the realm of LFD for robotic manufacturing tasks, it is paramount to strike a balance between speed and reliability in task execution. Not only should the robot operate at optimal speeds, but the execution should consistently result in successful outcomes. Furthermore, cost efficiency plays a pivotal role. This encompasses both the initial investment of time and resources in teaching the robot the task and the ongoing operational costs of task execution. For instance, jerky or erratic movements can accelerate wear and tear on the robot, inevitably leading to increased maintenance costs. Thus, smooth and precise task execution is not only a matter of operational efficiency but also a determinant of long-term economic viability.]

[In the context of manufacturing, the cycle time of execution of robot tasks becomes a key factor in the performance of the robot. Human demonstrations are often presented at a slow speed]






[demonstrations are actually the implicit constraints requried for successful performance of a task. Compared to the classic optimization-based trajectory planning approach, instead of explicitly defining the constraints needed to find an optimal path, demonstrations will encode this information implicitly. However, there is noise in the demonstration which obscures this information. As there is no objective truth (ground truth) to use for filtering the noise without destroying the information gain, this becomes a challenge to increase information efficiency. That is why we need to get this information from humans!]
[So overall, we can formulate the structure as follows; 1) traditional ways and optimization-based trajectory planning vs LFD 2) how Lfd can be related to opt based, constraints no longer need to be defined by an expert (sometimes it is even impossible to explicitly program it), but there is noise. opt-based solves for the fastest time while lfd is normally not fast, and due to noise, cannot be sped up. local speed-up is also possible in opt programmed by an expert, we need to find a way that nonexpert can do the same too. In this way we maximize the information gain]
In recent years, the manufacturing industry has witnessed a paradigm shift from mass production to mass customization. This transformation requires a more flexible and adaptive approach to robot programming, as production lines need to frequently reconfigure and reprogram tasks based on market demand\cite{cohen2019assembly} \cite{pedersen2016robot} \cite{qu2019smart}. This shift has created a demand for programming methods that can efficiently handle small-batch productions with frequent task changes. In this context, Traditional programming methods present several drawbacks, including the need for on-site robot experts and extended programming time. These limitations increase production downtime and financial costs, hindering the ability to meet the dynamic demands of mass customization\cite{sloth2020towards} \cite{dean2016robotic}.  As a solution, Learning from Demonstration (LfD) \cite{ravichandar2020recent} has emerged as a promising alternative. Unlike traditional methods, LfD enables robots to learn tasks through human demonstrations\cite{pastor2011skill}. This approach allows for the transfer of human skills and expertise to machines, providing a more flexible and adaptable solution. LfD is compelling when ideal behavior cannot be easily scripted or defined as an optimization problem but can be demonstrated\cite{ravichandar2020recent}.

[Kinesthetic teaching and why it is good: \cite{wu2021framework} --> direct transfer of skills
\cite{simonivc2021analysis}]

In the context of manufacturing tasks, the performance of robots is evaluated based on three "Key Performance Metrics": time, accuracy, and energy efficiency. These metrics hold direct influence over production rates, product reliability, and operational costs, making them vital indicators of success in manufacturing tasks. Despite the conceptual advantages of LfD, existing approaches often struggle to meet the key performance metrics. The quality of demonstrations plays a significant role in the learning efficiency of LfD approaches \cite{tsai2020constrained}. In many cases, the demonstrations fall short of the desired standards, resulting in suboptimal performance. These limitations highlight the need for an improved approach that can address these challenges and optimize the learning process in manufacturing tasks \cite{liu2022robot}.

%Time
in terms of time efficiency, humans often demonstrate at a low speed, as it is cognitively challenging to demonstrate different aspects of a task at once \cite{meszaros2022learning}. A simple uniform speed-up is not possible, as the dynamics of the task require a variable velocity profile across different segments in order to ensure reliable execution \cite{meszaros2022learning}. In the case of Kinesthetic teaching, hand trembling and sensor noises cause jumps and non-regularities in the recorded demonstration. A plain speed-up will amplify the existing noise and often lead to infeasible trajectories [Show it with a figure here]. Existing LfD approaches attempt to provide a corrective procedure, namely incremental learning \cite{simonivc2021analysis}, through which human can non-uniformly speed up and enhance their initial demonstration. However, the resulting velocity profile has no guarantee to be the most time-optimal one. Therefore, here in this work, we take the kinematic limits of the robot into an optimization problem, and solve for the most optimal timing law for the provided demonstration path. Then, we allow the user to locally "slow down" the demonstration until reliable execution is ensured. In this way, we can guarantee that the most efficient timing law is adopted for the demonstration.

% Accuracy
In order to solve for the optimal timing law, it is necessary to eliminate the aforementioned demonstration noise from the demonstration path, since the noise can rapidly surpass the kinematic limits and prevent the optimization problem to converge to the solution (also it will provide high-jerk trajectories that damages the robot). Removing this noise, without compromising the path's accuracy, becomes a nontrivial problem. In the state of the art, the accuracy of demonstrations has been best represented by the notion of permitted path variability across the motion, i.e. how much deviation is allowed for the robot in order to still reliably accomplish the task. For example, in a Pick and Place task, the motion has to be accurate at the picking and the placing segment, but can be more variable in the rest of the motion without violating task reliability. Existing LfD approaches rely on the statistics of multiple demonstrations to extract this variability, which leads to longer programming time and more human effort \cite{muller2020one}. Delivering the variability information indirectly through multiple demonstrations is informationally inefficient as it leaves the user with less control over what they are teaching (e.g. for a high-precision manufacturing task, the user needs to repeat the high-precision part of the task while teaching variability in other parts, while the robot might also capture some unwanted variability in the accurate part) \cite{hu2022robot}. In our work, we leverage the psychological fact that humans slow down when they want to be precise and propose a novel method through which humans can demonstrate the variability, and hence the accuracy, of the motion in one single step. We propose a velocity correction procedure, through which proper variability tolerance values are extracted from human velocity feedback. We incorporate these tolerances in our optimization approach as constraints in order to smoothen the demonstration while maintaining accuracy!

% Energy Efficiency
The energy efficiency of a robot executing a task has been overlooked in the existing LfD approaches. This becomes of special importance when it comes to manufacturing and industrial task. Reducing the energy consumption of an execution cycle by even a small amount could lead to significant savings in energy at the end of the day, as numerous cycles accumulate. A suitable metric for the energy efficiency of a trajectory on the kinematic level is the jerk \cite{soori2023optimization}, as it indicates how robot torque commands are fluctuating. This is directly related to mechanical vibration, and wear-and-tear of the robot in the long run \cite{piazzi2000global} \cite{gasparetto2007new}. Moreover, the jerk profile shows the irregularities of the motion, reflecting the demonstration noise as well as unnecessary changes in the motion. By minimizing jerk in our optimization problem, we can take advantage of the variability tolerances in order to converge to a smooth path in position, velocity, and acceleration level. With the new smoothed demonstration, We use Dynamic Movement Primitives (DMPs) as our learning approach to show how the reproduced motion is more energy-optimal compared to the original demonstration. The choice of DMP over other LfD approaches is simply due to the fact that DMP provides satisfactory generalizability by requiring only one demonstration.

% Overall wrap up
Considering the mentioned key performance metrics, our work proposes an optimization-based smoothing algorithm that creates accurate time-and-jerk optimal trajectories while filtering the demonstration noise. We show how the learning efficiency of DMPs in trajectory reproduction improves with our smoothing approach %, especially in the joint space, as a minor noise on joint values can translate to high end-effector variations. The choice of the joint state over the end effector state for industrial tasks is due to advantages in kinematic redundancy management and singularities avoidance\cite{fabisch2020comparison}.
We also present an incremental learning approach, where the human first only demonstrates the path, then the timing, and as a byproduct, the accuracy of the task [Figure here]

[Performing the computations in joint space instead of Cartesian space allowed the operator to determine the entire configuration of the 7 DOF robot arm \cite{karlsson2017autonomous}]

[The mean and variance of the trajectory are adopted to construct the constrained space for the optimization problem. Motion primitives with larger variance imply multiple possible trajectories and therefore the policy will aim to find the optimal path within the bounded space. On the other hand, the ones with smaller variance imply movement with higher precision, hence the policy should deviate less from the mean trajectory. By constraining the search area within the variance and applying a teacher’s understanding of the subtrajectory to the learning policy, it can avoid the exploration of sub-optimal region and action and thus improving the learning efficiency. \cite{tsai2020constrained}]


Considering the mentioned key performance metrics, our work proposes a human-in-the-loop demonstration framework, that guarantees optimal and information-rich demonstration at the output. The main contributions of our work is as follows:
\begin{itemize}
    \item an optimization-based smoothing algorithm that creates accurate time-and-jerk optimal trajectories while filtering the demonstration noise. We show how the learning efficiency of DMPs in trajectory reproduction improves with our smoothing approach
    \item A novel way of acquiring task variability as a notion of accuracy, in order to avoid providing multiple demonstrations
    \item compiling our approach into an incremental learning approach, where the human first only demonstrates the path, then the timing, and as a byproduct, the accuracy of the task.
\end{itemize}


==> Sections/temp/introduction-temp4.tex <==
\section{Introduction}
\label{sec:intro}

% -- demonstrations can be seen as a way to implicitly provide the required task constraints for reliable execution. These constraints comprise of 1) path constraints, which e.g. encodes the information on how to approach and pick an object, how to insert a peg in hole, etc. 2) timing constraints: e.g. which part of the task should be executed slowly, which part can be executed faster without compromising the successful execution.

% -- Regarding path constraints, current demonstrations are inefficient in two ways 1) The demonstrations are noisy due to hand trembling, sensor noise, etc. which in turn leads to the unwanted fitting of the learning algorithm on the noise, instead of the underlying task constraints. 2) What is the importance of each portion of the demonstration? how different parts of a task might have different tolerances for variability?

% --regarding timing constraints, demonstrations are normally provided at a slow speed, as it is cognitively demanding to accurately demonstrate at a high speed. So the demonstration is not representative of the actual timing law with which the task should be executed. while the requirements

% -- Here in this work, we focus on the quality of the demonstration as a major bottleneck to the performance of the overall LfD system. We aim to enhance the quality of the human demonstration with respect to the most important metrics of manufacturing tasks.



In recent years, the manufacturing industry has witnessed a paradigm shift from mass production to mass customization. This transformation requires a more flexible and adaptive approach to robot programming, as production lines need to frequently reconfigure and reprogram tasks based on market demand\cite{cohen2019assembly} \cite{pedersen2016robot} \cite{qu2019smart}. This shift has created a demand for programming methods that can efficiently handle small-batch productions with frequent task changes. In this context, Traditional programming methods present several drawbacks, including the need for on-site robot experts and extended programming time. These limitations increase production downtime and financial costs, hindering the ability to meet the dynamic demands of mass customization\cite{sloth2020towards} \cite{dean2016robotic}.  As a solution, Learning from Demonstration (LfD) \cite{ravichandar2020recent} has emerged as a promising alternative. Unlike traditional methods, LfD enables robots to learn tasks through human demonstrations\cite{pastor2011skill}. This approach allows for the transfer of human skills and expertise to machines, providing a more flexible and adaptable solution. LfD is compelling when ideal behavior cannot be easily scripted or defined as an optimization problem but can be demonstrated\cite{ravichandar2020recent}.

In the context of robot manufacturing, the performance of a robotized plant can be evaluated based on its implementation costs and operational efficiency. implementation costs are directly related to the resources and efforts required to successfully teach a robotic task, while operational efficiency can be evaluated based on the production speed vs the ongoing costs like maintenance and wear-and-tear of the robot. Despite the conceptual advantages of LfD, state-of-the-art approaches are not fully tailored for such a context. In this paper, we argue that the quality of demonstrations is a major bottleneck causing LfD approaches to struggle to meet the demands of the manufacturing industry. In many cases, the demonstrations fall short of the desired standards, resulting in suboptimal performance. \cite{liu2022robot}.

Human demonstrations can be seen as an intuitive way to implicitly represent the task constraints required for reliable execution of the task. an optimal information-rich demonstration can be measured by how well it contains the task constraints with respect to the application, in order for any LfD algorithm to learn and generalize. Such constraints encode the temporal and spatial laws. Temporal laws provide information on the dynamics of the task at each segment, e.g. which segments should be executed slower in order to ensure successful task completion. Spatial laws encode the robot's desired way of executing the task, e.g. how to approach and pick an object, how to insert a peg in hole, etc.

Regarding the temporal laws, humans often demonstrate at a low speed, as it is cognitively challenging to demonstrate different aspects of a task at once \cite{meszaros2022learning}. As reducing the cycle time of execution is a crucial factor in manufacturing, it is necessary to obtain the most optimal temporal laws. Existing LfD approaches attempt to provide a corrective procedure, namely incremental learning \cite{simonivc2021analysis}, through which humans can non-uniformly speed up and enhance their initial demonstration. However, the resulting velocity profile has no guarantee to be the most time-optimal one, as no kinematic limits are taken into account. Moreover, the process of recording human demonstrations introduces noise in the demonstration, e.g. hand trembling, and sensor noise, which causes jumps and non-regularities in the recorded demonstration. Speeding up can amplify the noise and can rapidly surpass the limits of the robot, without actually reaching the optimal timing law. The noise will also lead to a highly jerky movement, leading to more wear-and-tear, lower robot lifespan, higher maintenance cost, and inefficient energy usage. Therefore, in order to optimize the information gain of the demonstrations with respect to operational efficiency, it is necessary to provide smooth demonstrations with the lowest possible cycle time.

Regarding spatial laws, When humans demonstrate a task, they are inherently defining the "correct" or "desired" way of executing that task. This is similar to defining the constraints in an optimization problem. Since the goal of LfD is not to exactly replicate the motion, but to learn the underlying recipe of the task, it is necessary to define a factor of precision for each portion of the demonstration, i.e. how much tolerance is allowed for the robot in order to still reliably accomplish the task. For example, in a Pick and Place task, the motion has to be precise at the picking and the placing segment, but can be more variable in the rest of the motion without violating task reliability. Encoding these tolerances in the demonstration can be leveraged to find an optimum solution. Existing LfD approaches rely on the statistics of multiple demonstrations to extract the tolerances, we aim at developing a demonstration framework where humans can intuitively demonstrate the spatial and temporal laws of the task, as well as the underlying tolerances.

Considering the mentioned drawbacks, we propose a 2-stage optimal demonstration framework for teaching manufacturing tasks (Fig ...). The guiding stage is where humans only teach the

% Learning from Demonstration (LfD) represents a paradigm shift in the field of robotics where robots are trained by observing and replicating human demonstrations. As opposed to traditional methods of programming, there is no need for a robotic expert to program the robot and non-experts can directly teach the robots how a task is done in an intuitive way. Human demonstrations in LfD can be seen as an intuitive way to provide required task constraints to ensure reliable execution of the task, directly by a task expert, not a robot expert. Traditionally, precise robot tasks would need to be formulated as on optimization problem with explicit constraints. Human demonstrations can be a means of providing these constraints in an implicit way, without a robot expert hand-designing them. LfD is particularly compelling when ideal behavior cannot be easily scripted or formulated as an optimization problem with hand-designed task constraints but can be demonstrated\cite{ravichandar2020recent}.

% In the context of robot manufacturing, the efficiency of a robotized plant can be measured by implementation and operational efficiency. The implementation efficiency is directly related to the resources required to introduce/program a new robot task, while the operational efficiency is about the cycle time of execution, maintenance, and wear-and-tear of the robot. The recent paradigm shift from mass production to mass customization, calls for a more flexible and adaptive approach to robot programming, as production lines need to frequently reconfigure and reprogram tasks based on market demand\cite{cohen2019assembly} \cite{pedersen2016robot} \cite{qu2019smart}. Conceptually, LfD is a promising alternative as it significantly reduces the implementation costs by eliminating the need for an on-site robot expert and shortens the implementation time by having the process expert directly interact with the robot.



==> Sections/temp/methodology-temp.tex <==
\section{Methodology}
\label{sec:method}

In this section, we first explain in detail, how our optimization-based smoothing algorithm works. Then, we elaborate on the variability-velocity relationship and finally illustrate our optimal demonstration framework.

\subsection{Optimization-based Smoothing}

We begin by recording a noisy demonstration of the robot's trajectory and prefiltering it based on the end-effector's position and orientation, in the sense that robot must move beyond a certain threshold in order to consider a new waypoint. This process allows us to extract meaningful waypoints from the path, denoted as $w_i$ for  $\forall i=1,\cdots,m$. $q_{w_i} \in \mathbb{R}^n$ refers to the joint configuration of the waypoint, while $p_{w_i} \in \mathbb{R}^3$ and $\theta_{w_i} \in \mathbb{S}^3$ refer to the position and orientation of the end-effector, respectively. We want to formulate an optimization problem that minimizes the timing and jerk of a trajectory passing through these waypoints with a specific tolerance. Defining the tolerance in the joint space becomes unintuitive and non-uniform, since depending on the joint configuration, a fixed tolerance value for joint space can lead to different values in the end-effector space. As the end-effector pose is the final important factor in the task, it makes more sense to define the tolerance for each waypoint in the end-effector space. Let's denote $\epsilon_p^i \in \mathbf{R}^3$ as the tolerance in the position, and $\epsilon_\theta^i \in \mathbf{R}$ as the tolerance in the difference of angle for $i^th$ waypoint. there are two challenges when attempting to solve this problem: 1) Simultaneously minimizing time and jerk is conflicting. As the total time is unknown, the optimizer will attempt to conversely increase the time to make the jerk values drop. Since our goal is to keep the optimal timing while regulating the jerk profile, this approach which will not converge to a desired solution. 2) In order to apply the path waypoints constraints, we need to know the time step when the trajectory reaches each waypoint. Since the original timing of the demonstration is suboptimal, we do not have the information necessary to formulate our optimization problem.

To handle the mentioned challenges, we propose a two-stage optimization problem. The first stage solves an optimization to find the optimal timing of each waypoint as well as the minimum overall execution time of the trajectory, denoted as $\tau_i$ for  $\forall i=1,\cdots,m$. We leverage this information in the second stage, where we solve the full optimization problem with all the tolerance constraints with the main objective of minimizing jerk. This hierarchical approach will output a time-optimal smooth trajectory $q_f(t)$ which satisfies the accuracy requirements. The underlying representation of all the trajectories in this work is B-Spline. Mathematically, a B-spline curve is defined as a linear combination of control points $P_i$ and B-spline basis functions $N_{i,k}(s)$. If the order of the B-spline is $k$ and there are $n$ control points, $P_1, P_2, ..., P_n$, then the B-spline curve can be expressed as:

\begin{align}
\xi(s) = \sum_{i=1}^{n} N_{i,k}(s) P_i
\end{align}

where $s$ is the parameter that ranges over the interval [0,1]. The control points $P_i$ determine the shape of the curve. These are typically the parameters we want to adjust in optimization problems. To represent a trajectory, $\xi(s)$ is associated with a duration parameter $T$, which scales the normalized value of $s$ into actual time.

\begin{figure}
    \centering
    
    \begin{subfigure}{0.47\textwidth}
        \includesvg[width=\linewidth]{Figures/opt_stage1}
        \caption{}
        \label{fig:opt1}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.47\textwidth}
        \includesvg[width=\linewidth]{Figures/opt_stage2}
        \caption{}
        \label{fig:opt2}
    \end{subfigure}
    
    \caption{Trajectory Representation at each stage}
    \label{fig:opt}
    \vspace{-5mm}
\end{figure}

\subsubsection{Stage 1: Finding the ideal timings}
The objective of this optimizer is to ensure that trajectory $q(t)$ strictly passes through all the waypoints $q_{w_i}$ in the minimum possible time. At this stage, we disregard kinematic acceleration and jerk limit, as the noise is still present in the path, and constraining the acceleration or jerk would prevent the optimizer to find the ideal timing. We fit a B-Spline sub-trajectory between every two consecutive waypoints, denoted as $\xi_j$ for $\forall j=1,\cdots,m-1$ (Fig here). The duration of the sub-trajectories, denoted as $T_j$, is a decision variable, along with the control points of all the sub-trajectories. The order of all the sub-trajectories is chosen to be $k=4$, to ensure smoothness. Moreover, we apply smoothness constraints at the joining point of sub-trajectories. By introducing the position and velocity bounds, denoted respectively by $q_{\text{min}}$, $q_{\text{max}}$, $v_{\text{min}}$ and $v_{\text{max}}$ the optimization problem becomes:

\begin{align}
&\text{Minimize: } J = \sum_{j=1}^{m-1} T_j, \\\nonumber
&\text{subject to: } \quad (\forall j = 1,\cdots,m-1, \quad \forall t \in [0, T_j]) \\
&1. \quad q_j(t) \in [q_{\text{min}},q_{\text{max}}], \quad \dot{q}_j(t) \in [v_{\text{min}},v_{\text{max}}] \\
&2. \quad \xi_j(0) = q_{w_{j}}, \quad \xi_j(1) = q_{w_{j+1}}, \\
&4. \quad \dot{\xi}_1(0) = \dot{\xi}_{m-1}(1) = 0
\end{align}

It is important to note that the result of this optimization is typically an infeasible trajectory, as the present noise causes large acceleration and jerk values. The purpose of this stage is to assume an ideal trajectory and find the ideal timing if the robot passes through all the points with the maximum possible velocity. The outcome of this stage is the time steps of each waypoint, denoted as $\tau_i$ for $\forall i=1,\cdots,m$ with $\tau_m$ being the execution time of the whole trajectory. This forms the basis for the next stage, where the full optimization problem is solved.

\subsubsection{Stage 2}

In order to formulate the full optimization problem, we represent the whole trajectory $q_f(t)$ as one single B-Spline $\xi_f$ with its associated duration variable $T_f$. The number of control points is chosen as the same as the waypoints, in order to give the optimizer enough freedom to locally tweak the trajectory around each waypoint. The order of the trajectory is again chosen as $k=4$ to enable smoothness. The objective of this stage is formulated as:

\begin{align}
    J_f = \alpha T_f + \beta \int_{0}^{1}||\dddot{\xi}_f||^2ds + \gamma  \sum_{i=1}^{m} ||P_i -q_{w_i}||^2
\end{align}

with the full optimization formulated as follows: 

\begin{align}
&\text{Minimize: } J_f, \\\nonumber
&\text{subject to: } \quad (\forall i=1,\cdots,m, \quad  \forall t \in [0, T_f]) \\
&1. \quad q_f(t) \in [q_{\text{min}},q_{\text{max}}], \quad \dot{q}_f(t) \in [v_{\text{min}},v_{\text{max}}],\\
&3. \quad \ddot{q}_f(t) \in [a_{\text{min}},a_{\text{max}}], \quad \dddot{q}_f(t) \in [j_{\text{min}},j_{\text{max}}], \\
&5. \quad ||T_f - \tau_m|| \in [-\epsilon_t,\epsilon_t], \\
&6. \quad \xi_f(0) = q_{w_{1}}, \quad \xi_f(1) = q_{w_{m}} \\
&7. \quad \dot{\xi}_f(0) = \dot{\xi}_f(1) = 0, \\
&8. \quad ||p_f(\tau_i) - p_{w_i}|| \in [- \epsilon_p^i, \epsilon_p^i], \\
&9. \quad ||\theta_f(\tau_i) - \theta_{w_i}|| \in [- \epsilon_\theta^i, \epsilon_\theta^i]
\end{align}

In this formulation, the acceleration and jerk bounds, denoted respectively by $a_{\text{min}}$, $a_{\text{max}}$, $j_{\text{min}}$ and $j_{\text{max}}$ have been introduced as well, to make the output a feasible trajectory. The timing of the trajectory $T_f$ is bounded to $\tau_m$, by a user-defined value $\epsilon_t$. This constraint uses the output of the previous stage to give the optimizer limited freedom to change $T_f$, while mostly forcing the optimizer to regulate the jerk profile. Constraints 55 and 66 enforce the trajectory to start at $q_{w_i}$ and finish at $q_{w_m}$ with zero velocity. The equations 77 and 88 enforce the path to stay close to $w_i$ at the time $\tau_i$ which is derived from the previous stage. The tolerances are applied on the end-effector space with the help of a forward kinematic function in the loop of optimization, $F_K: q_f(t) \mapsto (p_f(t),\theta_f(t))$. The aim is to keep the deviation of the position $p_f(\tau_i)$ and the angle $||\theta_f(\tau_i)||$ of the end-effector at each waypoint limited to $\epsilon_p^i$ and $\epsilon_\theta^i$, respectively.

In the objective function, $\int_{0}^{1}||\dddot{\xi_f}||^2ds$ attempts to minimize the normalized jerk profile. This will force the optimizer to leverage the waypoints' tolerances to modify the path in order to minimize the jerk profile. This process is the key step that eliminates the path noise while adhering to the tolerances representing task accuracy. Finally, the term $\sum_{i=1}^{m} ||P_i -q_{w_i}||^2$ makes sure that the control points are close to the original joint configuration of the waypoints. Since most of the robot arms used in manufacturing are kinematically redundant, multiple joint configurations exist for an end-effector pose. This term limits the null space of the robot configuration, encouraging the optimizer to stay close to the original joint configuration. Solving this optimization problem leads to a smooth trajectory, free of noise, and with an optimal timing law and a minimal jerk profile.



\subsection{Velocity Adjustment}

The smoothing process refines the demonstrated path by applying the fastest timing law, which effectively eliminates noise. However, this optimal timing may not ensure reliable task execution. Thus, it becomes imperative to allow human intervention to moderate the speed across different parts of the trajectory to enhance reliability. This is achieved by adjusting the mapping from normalized time, $s$, to actual time, $t$, on the normalized smooth trajectory, $\xi_f(s)$.

Our B-Spline trajectory is denoted by a normalized trajectory $\xi_f(s)$ and duration $T_f$. The mapping between actual time $t$ and normalized time $s$ is given as:

\begin{align}
s(t) = V_0 \cdot t
\end{align}

Here, $V_0 = \frac{1}{T_f}$ is the full speed at which the trajectory is executed. Nonetheless, during the adjustment phase, we replay the trajectory at a reduced speed, $V_0^c = \eta V_0$, to facilitate more reaction time for human observers. This moderated speed purely serves to accommodate human feedback and has no bearing on the ultimate execution speed, given the normalization at the conclusion of this stage.

Slowing down specific segments of $\xi_f(s)$ locally can be accomplished by modifying this mapping through user feedback. In this study, human feedback is used to compute an acceleration term $A(t) \in [0,-1]$, analogous to the function of a brake pedal, indicating the extent to which the trajectory speed should be reduced. The acceleration $A(t)$ is integrated into the mapping $s(t)$ using a straightforward kinematic model:

\begin{align}
    \left\{ \begin{matrix}
        \dot s_c(t) = v(t) \\
        \dot v(t) = A(t) 
    \end{matrix} \right., \quad
    \begin{matrix} 
    v(t) \in [V^c_0, V_{min}^c], \\
    s_c(t) \in [0,1]
    \end{matrix}
\end{align}

This model generates a new mapping, $s_c(t)$, modifying the timing law of the trajectory as per user preference. Upon replaying the trajectory and establishing the new mapping, $s_c(t)$ and $\tau_i$ can be used to determine the updated timing of each waypoint, $\tau_i^c$. These values are subsequently input into the second optimizer to derive the optimal trajectory given the new timings.


\subsubsection{Human Correction Interface}
To ensure intuitive and safe receipt of human feedback, we employ teleoperation. An axis button on a joystick serves as the brake button, supplying the command $C(t) \in [0,-1]$. In order to remove noise and prevent abrupt changes in this command, it is introduced as the attractor point of a spring-damper system:

\begin{align}
    \tau \ddot A(t) = K(C(t)-A(t)) - D \dot A(t) 
\end{align}

By carefully setting the values of $\tau$, $K$, and $D$, we can configure the system to be critically damped, as well as adjusting its settling time which, in turn, influences the delay in response to human command. The system output, $A(t)$, is used as an acceleration term during the adjustment phase.

\subsubsection{Tolerance Extraction}
Leveraging the psychological insight that individuals tend to slow down when precision is required, we posit a direct correlation between the absolute value of $C(t)$ and the desired level of accuracy at a given point on the trajectory. This means, the more intensively the brake button is pressed, the greater the significance of that trajectory section, necessitating increased precision. Consider the function $\Gamma(t)$:

\begin{align}
    \Gamma(t) = (\epsilon^{max} - \epsilon^{min})(1-(-C(t))^{n+\zeta}) + \epsilon^{min}
\end{align}

In this formulation, a $C(t) = 0$ is associated with maximum tolerances $\epsilon_p^{max}$ and $\epsilon_\theta^{max}$, whereas a $C(t) = -1$ corresponds to the minimum tolerances $\epsilon_p^{min}$ and $\epsilon_\theta^{min}$. By computing $\Gamma(\tau_i)$ for each waypoint, we extract the requisite tolerances and reapply the second optimization process.







==> Sections/temp/related_work-temp2.tex <==
\section{Related Work}
\label{sec:works}

Recently in the literature, there has been a shift from focusing on learning robustness against demonstration sub-optimality \cite{cao2021learning} \cite{cao2022learning}, towards evaluating the information gain and the quality of demonstrations \cite{wu2021framework} \cite{kalinowska2021ergodic}. In \cite{wu2021framework}, authors are motivated by the fact that the outcome of learning is highly affected by a poor demonstration, and have looked into how to measure the information gain from demonstrations. In \cite{kalinowska2021ergodic}, authors proposed the concept of negative demonstration, as a notion of what not to do, in order to enhance demonstrations efficiency. However, In this work, the focus is to provide a demonstration framework carefully designed to meet the key performance metrics of manufacturing tasks.

Several approaches leveraged incremental learning to enhance the optimality of human demonstrations. Authors in \cite{nemec2018efficient} proposed a velocity correction stage through which humans can locally adjust the speed of their initial demonstration. Human feedback was incorporated in a velocity scaling factor in the formulation of DMP. \cite{simonivc2021analysis} is one of the main works on incremental learning that allowed humans to enhance their initial demonstrations through corrective refinement of path and velocity via kinesthetic guidance. In \cite{meszaros2022learning}, teleoperated corrective feedback was used in a pick-and-place grocery task in order to speed up the execution while ensuring reliable execution. They continued their work in \cite{montero2022solving} by applying their framework to a precise assembly task. However, none of these works consider the kinematic limits of the robot in order to achieve the most optimal timing of the task. Moreover, Filtering demonstration noise and capturing the required variability of the task as a measure of accuracy is not directly considered in their incremental learning framework.

In order to smooth a trajectory obtained by kinesthetic demonstration, numerous works relied on obtaining multiple demonstrations \cite{hu2022robot} \cite{paxton2015incremental} \cite{roveda2020assembly} \cite{tsai2020constrained} \cite{wu2021framework}. Authors in \cite{shyam2019improving} utilized the demonstration to form the initial guess for their trajectory optimization problem, where they solve for smoothness and jerk minimization, although there are no constraints on the allowed variability and deviation from the demonstrations. In \cite{tsai2020constrained}, the statistics from multiple demonstrations were used in order to extract motion tolerances, which they use for their smoothing optimization. The information inefficiency of learning variability through multiple demonstrations is visible in the work of \cite{hu2022robot}. In order to capture the skillful aspects of a precise manufacturing task, the authors divided it into phases to be able to extract the precision requirements out of multiple demonstrations. Motivated by this inefficiency in industrial tasks, authors in \cite{muller2020one} proposed to use a single demonstration along with a fixed user-defined variability threshold. They leveraged this information to create a smooth noise-free trajectory. Our work surpasses the existing works by relying on a single demonstration while providing an interface for the humans to intuitively provide the variability tolerance, instead of hand designing or extracting statistically from multiple demos.

Several established methods exist for the purpose of noise filtering in a trajectory, e.g. Low-pass Filters, Kalman Filters, etc. However, they often manage to only eliminate high-frequency noise. Also, there is no possibility to incorporate the variability tolerances and constrain the smoothing process from deviating too much from the original demonstration. A comprehensive comparison of different smoothing algorithms is carried out in \cite{chen2018playback}. The authors have also mentioned the fact that RBF-based learning processes like DMPs can naturally smoothen the demonstration, but without careful tuning of the hyperparameters, the model can overfit easily and replicate the noise. It is finally shown that an optimization-based smoothing approach is advantageous in terms of retaining the main features of demonstration, and hence, enhancing information gain.

Therefore, we offer an incremental learning approach to capture the task's velocity and accuracy requirement, while leveraging the tolerances to minimize time and jerk. To the best of our knowledge, no previous work has considered all these factors. Hereby, we compile our proposed methods into an optimal demonstration framework tailored for manufacturing tasks [Figure here?]



==> Sections/temp/related_work_temp.tex <==
\cite{tsai2020constrained} --> multiple demos --> statistics (low variance ~ high precision) --> tolerances for variability in optimization problem -- optimization for smoothness, path length, and collision avoidance
accuracy (tolerance) + optimization (smoothing)

\cite{muller2020one} --> from multiple demo to single demo for industrial tasks -- use tolerances in optimization for trajectory generation -- tolerance is hand-designed -- time and jerk is not considered
accuracy(tolerance) + optimization

\cite{wu2021framework} --> Evaluate/Measure quality of demonstration -- Existing LFD approaches mostly focus on the learning part of LfD, rather than demonstration quality
from learning robustness to demonstration quality

\cite{shyam2019improving} --> Kinesthetic demonstration as initial guess for trajectory optimization --> avoid local optima -- optimization for smoothness and jerk + obstable avoidance -- multiple demos
optimization (smoothing)

\cite{cao2021learning} \cite{cao2022learning} --> Learning from suboptimal demonstration --> focus on learning robustness instead of demonstration quality.
from learning robustness to demonstration quality

\cite{meszaros2022learning} --> incremental learning --> reduce demonstration effort + reduce execution time while keeping reliability
incremental learning + time

\cite{montero2022solving} --> incremental learning same as \cite{meszaros2022learning} --> focus on precision while speeding up
incremental learning + time and precision

\cite{simonivc2021analysis} --> incremental learning -- first time to consider separate refinement of path and velocity
incremental learning +  time 

\cite{nemec2018efficient} --> incremental learning -- velocity correction in a form of velocity scaling factor -- contribute to time optimality -- no kinematic limit
incremental learning + time

\cite{kalinowska2021ergodic} --> multiple demos -- evaluate demonstrations information gain -- negative demonstration to increase information gain of demos -- formulate demonstration info as the objective of an MPC
from learning robustness to demonstration quality + information gain

Remove noise from trajectory and smoothen via multiple demos and GMM/GMR --> \cite{hu2022robot} \cite{paxton2015incremental} \cite{roveda2020assembly} \cite{tsai2020constrained} \cite{wu2021framework}

\cite{chen2018playback} --> remove noise from trajectory -- solve CHOMP, no time or jerk optimization, only smoothin for removing the noise -- 
smoothing based on optimization-based trajectory generation is better than low-pass filter, RBFNN, Kalman Filter -- learning processes can filter noise, but they can overfit easily and replicate the noise

\cite{hu2022robot} -> information inefficiency of teaching variability through multiple demos in manufacturing precise scenarios -- to capture the task, they divided it into phases
accuracy(multiple demos)

\cite{bearee2013dissociated} \cite{jin2014improving} \cite{biagiotti2013online} --> low pass filter approach













in meszaros the default is the demonstration speed and then user can speed it up, but here we default to the maximum speed and user can slow it down!

In \cite{meszaros2022learning}, authors have proposed an approach to iteratively correct a demonstration through teleoperated feedback. Their argument is on the complexity and the effort required by the human to teach multiple aspects of the task at the same time. Hence in this way, they facilitate the modification of the intial demonstration in terms of path and velocity. However, 
\begin{itemize}
    \item Their learning approach operates on the end-effector state. It means that the null space of the joint space is not captured by the LfD approach.
    \item As their target task is related to groceries (not industrial anyway), they have not incorporated the limits of the robot to achieve the highest possible execution cycle time. It is noteworthy to mention that in their approach, the LfD algorithm is in the loop of control, which reduces the achievable control frequency, and hence the achievable tracking velocity. The fact that they learn in the task space but execute in the joint space puts extra latency on the control process.
    \item They have not
\end{itemize}




%%%%%%%%%%%%%%%%%%%%%

One can say that with multiple demos there is the problem of association due to different durations and sample points

==> Sections/temp/result-temp.tex <==
\section{Validation Experiments}
\label{sec:result}


Experiments were conducted to evaluate the efficiency of our proposed framework, as well as to highlight the usability of our method. In Sec. \ref{sec:res_opt}, the performance of our optimization-based smoothing was analyzed for Reaching Task \#1. In Sec. \ref{sec:res_refine}, we evaluate the functionality of our refinement phase, showcasing how velocity adjustment and tolerance extraction works in action. We further discuss the role of tolerance values in finding optimal demonstrations. In Sec. \ref{sec:res_dmp}, a baseline comparison is made with respect to the original demonstration resulting from kinesthetic guidance. We compare the resulting DMP policy from both original and optimal demonstrations and show that our approach enhances efficiency by reducing the execution time and jerk profile.

We have used the 7 DoF Franka Emika Research 3 (FR3) with 1KHz control frequency. The recording of the demonstration happens through a ROS interface and with a frequency of 10 Hz. For teleoperation, we used a wireless F710 Logitech Gamepad which provides ergonomic convenience as well as ensuring that humans remain at a safe distance from the robot. The continuous input of the R2 axis is used as the brake button.

\subsection{Performance of Optimization-based Smoothing}
\label{sec:res_opt}
This experiment encompasses stages (A), (B), and (C) of the demonstration framework (refer to Algorithm \ref{alg:demo_framework}). Reaching Task \#1 was recorded via kinesthetic guidance and the corresponding waypoints $w_i$ were extracted. The criteria for extracting the waypoints was based on the movement of the end-effector, resulting in 49 waypoints. A new waypoint was extracted if the end-effector was moved at least 1 cm in position or 0.1 radian in angle. Kinematic limits $q_{\text{min}}$, $q_{\text{max}}$, $v_{\text{min}}$, $v_{\text{max}}$, $a_{\text{min}}$, $a_{\text{max}}$, $J_{\text{min}}$ and $J_{\text{max}}$ of FR3 for each joint are obtained through the robot's datasheet \cite{franka}. The goal of optimization-based smoothing is to take the path of the original demonstration and find the most optimal timing with respect to FR3's kinematic limits while regulating the jerk profile by eliminating path noise. The joint trajectory, along with velocity, acceleration, and jerk profile of each stage is shown in Fig. \ref{fig:opt}. Each color corresponds to a joint trajectory, representing all 7 DoFs. Fig. \ref{fig:org} shows the original demonstration, where velocity, acceleration, and jerk values are differentiated in a non-casual manner \cite{stulp2019dmpbbo}. The present noise particularly reflects itself on the jerk profile, with the maximum absolute normalized jerk value being 15358 $rad/s^3$. Moreover, the demonstration trajectory is slow, taking 8.88 seconds to accomplish the task. As explained in Sec. \ref{sec:opt}, The original demonstration is fed to the Time Optimization module for finding $\tau_i$. The output of this stage is shown in Fig. \ref{fig:opt1}. As mentioned, this is an unrealistic trajectory due to the exclusion of acceleration and jerk constraints. Nevertheless, for each $w_i$, the associated $\tau_i$ is extracted from this trajectory and fed to the Trajectory Generation module. Moreover, the default tolerance values are chosen to be $\epsilon^d_p = 2 cm$ and $\epsilon^d_\theta = 0.1 radian$. The output of this module is shown in Fig. \ref{fig:opt2}. It represents $q_f(t)$, a noise-free trajectory with a maximum absolute normalized jerk value of 78.3 $rad/s^3$ which only takes 1.2 seconds to execute.

Regarding the optimization process, $k=4$ is chosen as the order of B-Spline, ensuring smoothness up until the velocity level. The knots $u_1, \cdots, u_{\Bar{m}}$ were distributed in a clamped uniform manner \cite{de1972calculating}, forming the basis functions in \eqref{eq:bspline}. For the Time optimization module, the decision variables sum up to $4 \times 48=192$ control points and 48 duration variables, solved via SNOPT solver\cite{gill2005snopt}. The Trajectory Generation has 49 control points and one duration variable as decision variables, solved via IPOPT solver \cite{wachter2006implementation} as it offered more stability compared to SNOPT. The objective weights in \eqref{eq:mainopt0} are designed as $\alpha=1, \beta=0.04$, and $\gamma=1$ through trial and error. $\epsilon_t=0.5 s$ is chosen for the duration bound in \eqref{eq:mainopt3}. The optimization was performed on a system equipped with an Intel Core i9-10885H CPU running at 2.40 GHz, with 8 cores and 32 GB of DDR4 RAM. The Time Optimization took less than 5 seconds, while the Trajectory Generation took approximately 2 minutes to converge. All the optimization implementations are developed via Drake toolbox \cite{drake}.


\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.31\textwidth}
        \includegraphics[width=1.12\textwidth]{Figures/original.pdf}
        \caption{Original Demonstration}
        \label{fig:org}
    \end{subfigure}
    \hfill % space between subfigures
    \begin{subfigure}[b]{0.31\textwidth}
        \includegraphics[width=1.1\textwidth]{Figures/opt_t.pdf}
        \caption{Time Optimization}
        \label{fig:opt1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.31\textwidth}
        \includegraphics[width=1.1\textwidth]{Figures/opt_f.pdf}
        \caption{Trajectory Generation}
        \label{fig:opt2}
    \end{subfigure}
    \caption{Overall caption for all subfigures}
    \label{fig:opt}
\end{figure*}


\subsection{Demonstration Refinement}
\label{sec:res_refine}
It is possible that $q_f(t)$ is too fast for reliable or safe execution. For a reaching task, it is generally the case where the robot needs to carefully approach a target with fine precision and more stability. It is also very important in the context of human-robot collaboration. In the Refinement Phase (stage (D) in Algorithm \ref{alg:demo_framework}), the robot replays $q_f(t)$, while the teacher interactively slows down the motion at the end, hence implying higher precision towards the end of reaching. As discussed in Sec. \ref{sec:refine}, we have chosen $\eta=5$ and $V_min^r=0.2V_0^r$ to reduce the task execution speed, solely for the sake of giving enough reaction time to the teacher through the loop of interaction. Without the teacher's command, the robot will continue to execute $\xi(s(t))$ with $s(t)=V_0^r(t)$. The teacher's filtered command $R(t)$ will decelerate the progression of time, leading to a modified mapping $s_r(t)$, immediately affecting the robot's motion. The progression of $s(t)$ and $s_r(t)$ during the refinement phase is shown in Fig. \ref{fig:srt}. Before providing any command, $s(t)$ and $s_r(t)$ overlap, leaving the timing law unchanged. As the teacher's command is received at $t^*$, $s_r(t)$ progression changes to slow down the motion accordingly, hence taking longer to execute the task. From this new mapping, the waypoints' modified timing law $\tau_i^r$ is extracted according to \ref{sec:vel}. Since the new timing law is extracted with respect to the normalized time $s$, the value of reduced refinement speed $V_0^r$ will not have any effect on the outcome.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{Figures/fig_replay.pdf}
    \caption{The progression of $s(t)$ and $s_r(t)$ during the refinement phase. The vertical green line shows the moment the teacher started giving command $R(t)$}
    \label{fig:srt}
    \vspace{-6mm}
\end{figure}

For tolerance extraction (Sec. \ref{sec:tol}, we have chosen $\epsilon_p^{max} = 5cm$, $\epsilon_p^{min}=1cm$, $\epsilon_\theta^{max}=0.3rad$, and $\epsilon_\theta^{min} = 0.1 rad$. By having $\epsilon_p^i$ and $\epsilon_\theta^i$ along with $\tau_i^r$, the Trajectory Fine-Tuning stage solves for $q_f^r(t)$ shown in \ref{fig:refined}, where the inverse relationship between the intensity of the brake command and extracted tolerances is illustrated via a colormap. The plot shows the Cartesian position trajectory of the end-effector and its associated tolerances derived from \eqref{eq:tol}. The fine-tuned trajectory is adjusted to be more precise towards the end of reaching, where slow speed was commanded. The tolerances in rotation angles were also applied in a similar way but omitted in the plotting for simplicity.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{Figures/fig_refined.pdf}
    \caption{Refined trajectory $q_f^r(t)$ after re-optimization via new timing law and tolerance values. Fig. (subfigure waypoint) shows the updated timing distribution of waypoints according to the provided command $R(t)$. Fig. (subfigure traj) highlights the extracted tolerance range in the end-effector's cartesian position X, Y, and Z. $T^*=...$ marks the duration of $q_f(t)$ before entering the refinement phase. }
    \label{fig:refined}
    \vspace{-6mm}
\end{figure}

Moreover, Fig. \ref{fig:wps} showcases the comparison between $tau_i$ and $\tau_i^r$, by showing the Y distribution of the waypoints $w_i$ before and after refinement. Towards the end of the task, the waypoints are stretched according to the received teacher's command, leading to a longer execution time. It is also noticeable that while the timing law of the beginning of the trajectory is left unchanged during refinement, the waypoint distribution does not overlap. This is due to the fact that since the tolerance values are increased from $\epsilon_p^d=2cm$ to $\epsilon_p^max=5cm$, the optimizer has managed to find a faster trajectory to traverse these waypoints. While low tolerances are necessary for the critical portions of the task, high tolerances elsewhere can be leveraged by optimization-based smoothing to find a trajectory with a better timing law and a lower jerk profile. This is best shown via Reaching Task \#2, where higher tolerances allow the optimizer to find better solutions. Fig. \ref{fig:tols} shows that increasing the value of the tolerances from 2 cm to 5 cm reduced the duration from 1.87 to 1.6, while regulating the jerk profile at the beginning of the motion, reducing the maximum jerk value from 73.6 $m/s^3$ to 36.56 $m/s^3$. We include this advantage in our refinement phase by assigning maximum tolerance where the teacher is not pressing the brake button, giving the optimizer more freedom to adapt the motion.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{Figures/fig_wps_t.pdf}
    \caption{Waypoints timing}
    \label{fig:wps}
    \vspace{-6mm}
\end{figure}



\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{Figures/fig_tols.pdf}
    \caption{The role of tolerances in finding the optimal demonstration. The high-tolerance trajectory executes with a lower duration and a lower initial jerk compared to the low-tolerance trajectory}
    \label{fig:tols}
    \vspace{-6mm}
\end{figure}


\subsection{Baseline Comparison}
\label{sec:res_dmp}

Compared to state-of-the-art kinesthetic teaching, we show the effectiveness of our demonstration framework via DMPs as an LFD approach. The choice of DMP as our designated method is due to the fact that it requires only one demonstration to train. Nevertheless, our proposed method is generic and can be applied to any LFD method. We train ${\mathrm{DMP}}_o$ with the original kinesthetic demonstration recorded for Reaching Task \#1, and ${\mathrm{DMP}}_s$ with $q_f(t)$, the resulting smooth demonstration out of our demonstration framework. Reproducing for the same start and goal, Fig. \ref{fig:dmp_path} shows the planned path of ${\mathrm{DMP}}_o$ with respect to ${\mathrm{DMP}}_s$. As shown, ${\mathrm{DMP}}_o$ has produced unnecessary curves at the beginning of the motion, replicating the existing noise. The effect of this noise is better shown in terms of the underlying joint trajectory generated by the ${\mathrm{DMP}}_o$, as well as the end-effector's jerk profile.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{Figures/fig_dmp_3d.pdf}
    \caption{An overview of the workflow in our proposed demonstration framework}
    \label{fig:dmp_path}
    \vspace{-6mm}
\end{figure}

For the sake of comparison, we also include a scaled version of ${\mathrm{DMP}}_o$, denoted as ${\mathrm{DMP}}_{os}$. Since the original demonstration is slower than the smooth one, we leverage the inherent scaling capability of DMPs \cite{ijspeert2013dynamical} to scale down ${\mathrm{DMP}}_{os}$ to have the same execution time as ${\mathrm{DMP}}_{s}$. For the optimal execution time calculated via our demonstration framework, ${\mathrm{DMP}}_{os}$ leads to an infeasible trajectory, caused by the existing noise. The planned velocity, acceleration, and jerk profile of ${\mathrm{DMP}}_{os}$ and ${\mathrm{DMP}}_{s}$ is shown in Fig. \ref{fig:dmp_kin}, along with the portions where kinematic limits are violated. The marked portions in Fig. \ref{fig:org_kin} highlight that several joint trajectories violate the kinematic limits in ${\mathrm{DMP}}_{os}$, while ${\mathrm{DMP}}_{s}$ trajectory in Fig. \ref{fig:smooth_kin} achieves the same timing while remaining feasible. Moreover, while the maximum jerk value for ${\mathrm{DMP}}_{os}$ is 999.27 $rad/s^3$, ${\mathrm{DMP}}_{s}$ creates jerks of maximum 57.4 $rad/s^3$ . This proof of concept shows that our demonstration framework has improved the efficiency of DMP output.

\begin{figure}[!htb]
    \centering
    \begin{subfigure}[b]{\columnwidth}
        \includegraphics[width=\linewidth]{Figures/fig_org_kin.pdf}
        \caption{First subfigure}
        \label{fig:org_kin}
    \end{subfigure}
    
    % \vspace{-5mm} % Optional vertical space
    
    \begin{subfigure}[b]{\columnwidth}
        \includegraphics[width=\linewidth]{Figures/fig_smooth_kin.pdf}
        \caption{Second subfigure}
        \label{fig:smooth_kin}
    \end{subfigure}
    \caption{Caption for the whole figure}
    \label{fig:dmp_kin}
\end{figure}

Fig. \ref{fig:dmp_jerk}, shows a comparison of the end-effector's jerk profile between ${\mathrm{DMP}}_o$, ${\mathrm{DMP}}_{os}$, and ${\mathrm{DMP}}_{s}$, plotted in normalized time for the sake of consistency. It is clear that ${\mathrm{DMP}}_{s}$ creates the minimum overall jerk, highlighting the effect of the demonstration's jerk in DMP output. Overall, we have successfully proved that our proposed method effectively finds optimal timing law while removing noise and regulating jerk. Table \ref{tab:comparison} summarizes the comparisons made between the original and smooth demonstration, as well as among ${\mathrm{DMP}}_o$, ${\mathrm{DMP}}_{os}$, and ${\mathrm{DMP}}_{s}$ with respect to their cycle time and maximum absolute jerk value computed in normalized time s (for the sake of consistency).


\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{Figures/fig_dmp_jerk.pdf}
    \caption{An overview of the workflow in our proposed demonstration framework}
    \label{fig:dmp_jerk}
    \vspace{-6mm}
\end{figure}


\begin{table}[h!]
  \centering
  \caption{Comparison of Time and Jerk for Different Trajectories}
  \label{tab:comparison}
  \begin{tabular}{l S[table-format=2.2] S[table-format=5.1]}
    \toprule
    \multicolumn{1}{l}{\textbf{Trajectory Source}} & 
    \multicolumn{1}{c}{\textbf{Time [$s$]}} & 
    \multicolumn{1}{c}{\textbf{\parbox{3cm}{\centering Max. abs.\\ normalized jerk [$rad/s^3$]}}} \\
    \midrule
    Original Demonstration & 8.88 & 15358 \\
    Smooth Demonstration   & \textbf{1.2} & \textbf{78.3} \\
    \cmidrule{1-3}
    $\mathrm{DMP}_{o}$   & 8.88  & 2305.9 \\
    $\mathrm{DMP}_{so}$  & \textbf{1.2} & 1837 \\
    $\mathrm{DMP}_{s}$   & \textbf{1.2} & \textbf{101.5} \\
    \bottomrule
  \end{tabular}
\end{table}



% \begin{figure}[!htb]
%     \centering
%     \begin{minipage}{0.3\columnwidth} % Left side: one large image
%         \begin{subfigure}[t]{\textwidth}
%             \includegraphics[width=\textwidth,height=0.6\columnwidth,keepaspectratio]{Figures/fig_dmp_3d.pdf}
%             \caption{Subfigure 1}
%         \end{subfigure}
%     \end{minipage}%
%     \begin{minipage}{0.7\columnwidth} % Right side: two stacked images
%         \begin{subfigure}[t]{\textwidth}
%             \includegraphics[width=\textwidth,height=0.3\columnwidth,keepaspectratio]{Figures/fig_org_kin.pdf}
%             \caption{Subfigure 2}
%         \end{subfigure}
        
%         \vfill
        
%         \begin{subfigure}[b]{\textwidth}
%             \includegraphics[width=\textwidth,height=0.3\columnwidth,keepaspectratio]{Figures/fig_smooth_kin.pdf}
%             \caption{Subfigure 3}
%         \end{subfigure}
%     \end{minipage}
%     \caption{Main figure caption}
%     \label{fig:main}
% \end{figure}




==> Sections/temp/result_temp.tex <==
\textbf{Time Optimality}

compare the duration of the original demonstration to the smoothed demonstration

\textbf{Noise and Jerk}

For all 7DOF: compute the mean and standard deviation of acceleration and jerk profile of the original vs smoothed trajectory.

Comparison of energy consumption: scale the original demonstration to have the same time as the smooth one, execute them both on Gazebo and calculate the energy consumption of both based on the effort profile. (original demonstration is infeasible, so we have to execute it in Gazebo)

\textbf{accuracy}

create plots for x, y, z, and $\theta$, show the original demonstration, and show a colored area around that to show the tolerance region, and then show that the optimized trajectory is in that region.

\textbf{velocity adjustment}

remember one of the demos that couldn't optimize properly for a low tolerance in the middle.

Create a 2x2 Plot, the first row shows the default tolerances, with the optimized velocity profile, which sucks (we can also show the high jerks and stuff later in a table)
the second row shows the new tolerance region which is narrower at the beginning and end, and wider in the middle, with the optimized velocity profile in this case: this velocity profile is faster and better than the one with default tolerance, it is also accurate in the beginning and end, which is very nice:
The timing, velocity, acceleration, and jerk can also be compared in a table!

